CheckedCBox: Type Directed Program Partitioning with Checked C for Incremental Spatial Memory Safety

Spatial memory safety violation is still a major issue for C programs. Checked-C is a safe dialect of C and extends it with Checked pointer types and annotations that guarantee spatial memory safety in a backward-compatible manner, allowing the mix of checked pointers and regular (unchecked) pointer types. However, unchecked code vulnerabilities can violate the checked code's spatial safety guarantees. We present CheckedCBox, which adds a flexible, type-directed program partitioning mechanism to Checked-C, by enhancing the Checked-C type system with tainted types that enable flexible partitioning of the program into checked and unchecked regions, in a manner such that unchecked region code does not affect the spatial safety in the checked region. We formalize our type system and prove the non-crashing and non-exposure properties of a well-typed CheckedCBox program. We implemented CheckedCBox in a configurable manner, which enables us to use existing sandbox mechanisms (eg WebAssembly) to execute programs. Consequently, in doing so, CheckedCBox has prevented four known vulnerabilities by efficiently partitioning the program.

==> compilation.tex <==
\section{Compilation}
\label{sec:compilation}

% \review{
% The first reviewer said:
% \begin{itemize}
% \item I had a really hard time understanding precisely the "formalized" compilation
%   from CoreChkC to CoreC. Specifically: is CoreC intended to model LLVM-IR, or
%   is it a subset of C? Is CheckedC compiling to C or is it a new frontend like
%   `clang`? See remark about undefined behavior (UB) below which got me even more
%   confused. \mwh{CoreC is meant to model CoreChkC but with
%   annotations, and checks removed; it is not meant to model C or LLVM-IR.}
% \item Is the compilation scheme from CoreChkC to CoreC is faithful to the actual
%   compilation scheme of the checkedc-clang compiler to ...? I feel like the
%   paper is missing an actual description of what happens in the compiler to
%   allow us to connect the dots and understand how the formalization illuminates
%   the implementation. \mwh{We did not model compilation on the real
%   implementation; our purpose was to show that annotations in CoreChkC
%   do not necessitate fat pointers in an implementation; that said,
%   our formalization does show how a real implementation can be
%   carried out}
% \item The paper doesn't seem upfront about what is *shown* (theorem in Coq) and what
%   is *tested* (via PLT-Redex), and thus remains a
%   conjecture. \mwh{Updated the intro and the individual sections}
% \item  Missing discussion of why Coq vs. PLT-Redex, effort involved, any plans to
%   formally prove compilation from CoreChkC to CoreC, any hopes of integrating
%   that in the official implementation, etc. \mwh{Added note at the
%   start of section 3.}
% \end{itemize} }

% \review{IV: ghost variables in other contexts (e.g. Why3, Dafny) are used for things
%   that do not exist at run-time, but this doesn't seem to be the case here.}
% \yiyun{Agreed: We changed the name to ``shadow variables'' to avoid confusion}
% \review{Do your bug report and github links break anonymity?}


% \review{From reviewer C:
% \begin{itemize}
% \item I'd like to have seen a bit more motivation for using PLT redex:
%   what aspects made the use of this tool preferable to formulating the
%   compilation in Coq and using Quickchick to do random testing of the
%   simulation result.
%   \mwh{Added some text to the end of III.A and IV.C}
% \yiyun{Some reasons I can think of:\begin{itemize}
%     \item Redex is highly optimized for specifying judgments that are algorithmic. By writing down a typing relation, we can immediately obtain a typechecker
%     that is executable. Same applies for the small-step evaluation relation. Translating the relations into functions in Coq is definitely doable but time-consuming, especially since compilation is embedded as part of the typing rules. It is also hard to see whether the function we define really corresponds to the relation unless we formally prove it. This issue is particularly relevant at the early stage of the development when the compilation rules were buggy and the simulation property was violated often as we added new generator cases.
%     In Redex, we don't have any formal guarantee either, but at least we can more easily see the correspondence because Redex is able to convert the relation into an executable version so we can specify the relation literally. This feature of Redex helped us speed up our development significantly when our compilation rules were constantly changing.
% \end{itemize} }
% \item there's a funny change of line spacing in column 2 of page 6, about 2/3 down.
% \end{itemize}
% }

The main subtlety of compiling \checkedc to Clang/LLVM is to capture the annotations on pointer literals
that track array bound information, which is used in premises
of rules like \textsc{S-DefArray} and
  \textsc{S-AssignArr} to prevent spatial safety violations.
The \checkedc compiler \cite{li22checkedc} inserted additional pointer checks 
for verifying pointers are not null and the bounds are within their limits. \lc{what does it mean by bounds within limits?}
The latter is done by introducing additional shadow variables for storing (NT-)array pointer bound information.

\begin{figure}[t!]
{\small
\hspace*{-0.5em}
\begin{tabular}{|c|c|c|c|}
\hline
& \cmode & \tmode & \umode \\
\hline
& \textsc{CBox} / \textsc{Core} & \textsc{CBox} / \textsc{Core} & \textsc{CBox} / \textsc{Core} \\
\hline
\cmode & $\estar{x}$ / $\getstar{\cmode}{x}$ 
 & $\texttt{sand\_get}(x)$ / $\getstar{\umode}{x}$ &  $\times$ \\
\hline
\umode & $\times$
 & $\estar{x}$ / $\getstar{\umode}{x}$ &  $\estar{x}$ / $\getstar{\umode}{x}$ \\
\hline
\end{tabular}

}
\caption{Compiled Targets for Dereference}
\label{fig:flagtable}
\end{figure}

In \systemname, context and pointer modes determine the particular heap/function store that a pointer points to,
i.e., $\cmode$ pointers point to checked regions, while $\tmode$ and $\umode$ pointers point to unchecked regions. \lc{context mode doesn't determine where pointer points to but check if it is valid to point to that region?}
Unchecked regions are associated with a sandbox mechanism that permits exception handling of potential memory failures.
In the compiled LLVM code, pointer access operations have different syntaxes when the modes are different. \lc{should we explain why we use different syntax instead of compiling the corresponding heap to llvm}
\Cref{fig:flagtable} lists the different compiled syntaxes of a deference operation ($\estar{x}$) for the compiler implementation (\textsc{CBox}, stands for \systemname) and formalism (\textsc{Core}, stands for \lang). The columns represent different pointer modes and the rows represent context modes.
For example, when we have a $\tmode$-mode pointer in a $\cmode$-mode region, we compile a deference operation to the sandbox pointer access function ($\texttt{sand\_get}(x)$) accessing the data in the \systemname implementation. In \lang, we create a new deference data-structure on top of the existing $\estar{x}$ operation (in LLVM): $\getstar{m}{x}$. If the mode is $\cmode$, it accesses the checked heap/function store; otherwise, it accesses the unchecked one.

This section shows how \lang deals with pointer modes, mode switching and function pointer compilations, 
with no loss of expressiveness
as the \checkedc contains the erase of annotations in \cite{li22checkedc} and \Cref{appx:comp1}.
For the compiler formalism, 
we present a compilation algorithm that converts from
\lang to \elang, an untyped language without metadata
annotations, which represents an intermediate layer we build on LLVM for simplifying compilation. 
In \elang, the syntax for deference, assignment, malloc, function calls are: $\getstar{m}{e}$, $\elassign{m}{e}{e}$, 
$\emalloc{m}{\omega}$, and $\elcall{m}{e}{\overline{e}}$. \lc{strlen?}
The algorithm sheds
  light on how compilation can be implemented in the real Checked C
  compiler, while eschewing many vital details (\elang has many 
  differences with LLVM IR).


%This section shows how \systemname deals with 
%annotations can be safely erased: using static information a compiler
%can insert code to manage and check bounds metadata, with no loss of
%expressiveness. We present a compilation algorithm that converts from
%\lang to \elang, an untyped language without metadata
%annotations. The syntax and semantics \elang
  %closely mirrors that of \lang; it differs only in that literals lack
  %type annotations and its operational rules perform no
  %bounds and null checks, which are instead inserted during
  %compilation. Our compilation algorithm is evidence that \lang's
  %semantics, despite its apparent use of fat pointers, faithfully
  %represents Checked C's intended behavior. The algorithm also sheds
  %light on how compilation can be implemented in the real Checked C
  %compiler, while eschewing many important details (\elang has many 
  %differences with LLVM IR).

Compilation is defined by extending \lang's
typing judgment as follows:
\[\Gamma;\Theta;\rho \vdash_m e \gg \dot e:\tau\]
There is now a \elang output $\dot e$ and an input $\rho$, which maps
each (NT-)array pointer variable to its mode and
each variable \code{p} to a pair of \emph{shadow
  variables} that keep \code{p}'s up-to-date upper and lower bounds. 
These may differ from the bounds in \code{p}'s type due to bounds
widening.\footnote{Since lower bounds are never widened, the
  lower-bound shadow variable is unnecessary; we include it for uniformity.} 
\lc{These two sentences are confusing. }

% When $\Gamma$,$\Theta$ and $\rho$ are all empty, we write $e \gg \dot e$ rather than the
% complete judgment, implicitly assuming that $e$ is a well-typed and closed
% term.

We formalize rules for this judgment in PLT Redex~\cite{pltredex},
following and extending our Coq development for \lang. To give
confidence that compilation is correct, we use Redex's property-based
random testing support to show that compiled-to $\dot e $ simulates
$e$, for all $e$.

% We developed a \checkedc compiler to compile a \checkedc program to a C program.
% \mwh{We formalized compilation from CoreChkC to a version of CoreChkC
%   but with the metadata removed, right? This is not a Checked C
%   compiler. You go on to see stuff about CompCert, CLight,
%   etc. This is confusing. We should be talking about how this relates
%   to what was just presented. Pick definitive names for things. }
% Given a \checkedc program $e$, we build a compilation process ($\gg$), such that $e \gg \dot e$, where $\dot e$ is the corresponding C program for $e$ in A-normal form (ANF). 
% The compilation process ($\gg$) relies on the type checking step $\Gamma;\Theta\vdash_m e:\tau$. 
% Especially, it relies on $\Gamma$ to provide the type information for variables in $e$. 
% We utilize CompCert/CLight syntax and semantics \cite{Leroy:2009:FVC:1666192.1666216,Blazy2009} as our translation target language.
%  Besides, we defined two data structures in the CompCert format for representing $\enull$ and $\ebounds$ states.
% We write $\xrightarrow{c}$ for the semantics of CLight. \mwh{Of our
%   target language, which I presume does not have all the features that
%   CLight has. Should mention up front that we did all of this in PLT Redex.}

\subsection{Approach}

Due to space constraints, we explain the rules for compilation by
examples, using a C-like syntax; the complete rules are given in
\iftr
Appendix~\ref{appx:comp1}.
\else
the supplemental report~\cite{checkedc-tech-report}.
\fi
Each rule performs up to three tasks: (a) conversion of $e$ to
A-normal form; (b) insertion of dynamic checks and bound widening expressions; 
and (c) generate right pointer accessing expressions based on modes.
%
A-normal form conversion is straightforward: compound expressions are managed by storing results of subexpressions into temporary variables,
as in the following example.

{\vspace*{-0.5em}
{\small
\begin{center}
$
\begin{array}{l}
$\code{let y=(x+1)+(6+1)}$
\;
\begin{frame}

\tikz\draw[-Latex,line width=2pt,color=orange] (0,0) -- (1,0);

\end{frame}
\;
\begin{array}{l}
$\code{let a=x+1;}$\\
$\code{let b=6+1;}$\\
$\code{let y=a+b}$\\
\end{array}
\end{array}
$
\end{center}
}
}

This simplifies the management of effects from subexpressions. The
next two steps of compilation are more interesting.
We state them based on different \lang operations.

\begin{figure}[t!]
  \begin{small}
\begin{lstlisting}[mathescape,xleftmargin=4 mm]
int deref_array(n : int,
     p :  $\color{green!40!black}\tntarrayptr{0}{n}{\tint}{\cmode}$,
     q : $\color{green!40!black}\tntarrayptr{0}{n}{\tint}{\tmode}$) {
  /* $\color{purple!40!black}\rho$(p) = p_lo,p_hi,p_m */
  /* $\color{purple!40!black}\rho$(q) = q_lo,q_hi,q_m */
    * p;
    * q = 1;
}
...
/* p0 : $\color{purple!40!black}\tntarrayptr{0}{5}{\tint}{\cmode}$ */
/* q0 : $\color{purple!40!black}\tntarrayptr{0}{5}{\tint}{\tmode}$ */
deref_array(5, p0, q0);
    \end{lstlisting}
\begin{frame}

\tikz\draw[-Latex,line width=2pt,color=orange] (0,0) -- (1,0);

\end{frame}
\begin{lstlisting}[mathescape,xleftmargin=4 mm]
deref_array(int n, int* p, int * q) {
  //m is the current context mode
  let p_lo = 0; let p_hi = n; 
  let q_lo = 0; let q_hi = n; 
  /* runtime checks */
  assert(p_lo <= 0 && 0 <= p_hi);
  assert(p != 0);
  *(mode(p) $\wedge$ m,p);
  verify(q, not_null(m, q_lo, q_hi) 
             && q_lo <= 0 && 0 <= q_hi);
  *(mode(q) $\wedge$ m,q)=1;
}
...
deref_array(5, p0, q0);
    \end{lstlisting}
\end{small}
    \caption{Compilation Example for Dependent Functions}
\label{fig:compilationexample1}
\end{figure}

% \review{Fig 9: if this is actual C code, then your null-check at line 6 will be
%   eliminated by the compiler. At line 3, you performed a pointer addition, which
%   is only defined when `p` is non-null. So, either `p` is non-null, and the
%   NULL-check can be eliminated; or, `p` is NULL, but line 3 was undefined
%   behavior, meaning the compiler is allowed to do anything, notably eliminate
%   the NULL-check. This is where I am super confused, and either:
%   - CoreC is not really the C language, and has different semantics...? but is
%     this well-defined in the context of LLVM?
%   - there is a problem that was not caught by the PLT-Redex-based testing.
% \yiyun{We have clarified at the start of IV that CoreC is an untyped
%   variant of CoreChkC, and does not aim to represent C per se, or LLVM
%   IR. We aimed to avoid confusion by rewriting the examples in a way that is more closely
%     related to the syntax presented in Fig 3. Pointer arithmetic between 0 and a non-zero
%     index is always valid because CoreC there is technically only
%     integer arithmetic.}}

\myparagraph{Pointer Accesses and Modes}
%
In every declaration \lc{(or the beginning of a function body) why?} of a pointer,
if the poniter is an (NT-)array,
we first allocate two \emph{shadow variables}
to track the lower and upper bounds which are potentially changed for pointer arithmetic and NT-array bound widening.
Each $\cmode$-mode NT-array pointer variable is associated with its type information in a store.
Additionally, we place bounds and null-pointer checks, such as the line 6 and 7 in \Cref{fig:compilationexample1}.
In addition, in the formalism, before every use of a tainted pointer (\Cref{fig:compilationexample1} line 9 and 10), 
there is an inserted verification step similar to \Cref{fig:const-type},
which checks if a pointer is well defined in the heap (\code{not_null}) and the spatial safety.
Predicate \code{not_null} checks that every element in the pointer's range (\code{p_lo} and \code{p_hi}) is well defined in the heap.  
The modes in compiled deference (\code{*(mode(p) }$\wedge$\code{ m,p)})
 and assignment (\code{*(mode(q) }$\wedge$\code{ m,q)=1}) operations 
are computed based on the meet 
operation ($\wedge$) of the pointer mode (e.g. \code{mode(p)}) and the current context mode (\code{m}).

\myparagraph{Checked and Unchecked Blocks}
%
In the \systemname implementation,
$\euncheckedtext$ and $\echeckedtext$ blocks 
are compiled as context switching functions provided by the sandbox mechanism.
$\eunchecked{\overline{x}}{e}$ is compiled to 
$\texttt{sandbox\_call}(\overline{x},e)$, where we call the sandbox 
to execute expression $e$ with the arguments $\overline{x}$.
$\echecked{\overline{x}}{e}$ is compiled to 
$\texttt{callback}(\overline{x},e)$, where we perform 
a \texttt{callback} to a checked block code $e$ inside a sandbox.
In \systemname, we adopt an aggressive execution scheme that
directly learns pointer addresses from compiled assembly to make the $\texttt{callback}$ happen.
In the formalism, we rely on the type system to 
guarantee the context switching without creating the extra function calls for simplicity.

%Fig.~\ref{fig:compilationexample} shows how an invocation of
%\code{strlen} on a null-terminated string is compiled into C
%code. Each dereference of a checked pointer requires a null check
%(See \textsc{S-DefNull} in Fig.~\ref{fig:semantics}), which the
%compiler makes explicit: Line~$3$ of the generated code has the null
%check on pointer \code{p} due to the \code{strlen},
%  and a similar check happens
%  at line~$8$ due to the pointer arithmetic on \code{p}.
%Dereferences also require bounds checks: line~$2$ checks \code{p} is
%in bounds before computing \code{strlen(p)}, while line~$10$ does
%likewise before computing \code{*(p+1)}.

\myparagraph{Function Pointers and Calls}
%
Function pointers are managed similarly to normal pointers,
but we insert checks to check if the pointer address is not null in 
the function store instead of heap, and whether or not the type is correctly represented, 
for both $\cmode$ and $\tmode$ mode pointers 
\footnote{$\cmode$-mode pointers are checked once in the beginning and $\tmode$-mode pointers are checked every time when use}.
For example, in compiling the \code{stringsort} function in \Cref{fig:checkedc-example-1},
we place a check \code{verify_fun(cmp, not_null(c, p_lo, p_hi) && type_match)},
and we place a similar check before \Cref{fig:checkedc-example-3} line 7 to check the tainted \code{cmp} when it is used. 
The compilation of function calls (compiling to $\elcall{m}{e}{\overline{e}}$) 
is similar to the manipulation of pointer access operations in \Cref{fig:flagtable}.

For compiling dependent function calls,
\Cref{fig:compilationexample1} provides a hint.
Notice that the bounds for the array pointer \code{p} are not passed as
arguments. Instead, they are initialized according to \code{p}'s
type---see line~4 of the original \lang program at the top of the figure.
Line~$3$ of the generated code
sets the lower bound  to \code{0} and the
upper bound to \code{n}.

\subsection{Metatheory}
\label{sec:meta}

% \review{ 
% My interpretation of section IV.C is that the authors have a pen-and-paper
%   proof of Theorem 4, and that random testing using the Redex models has been
%   used to gain confidence in such a proof. Is this correct?}
% \liyi{Yes, this is correct.}
% \mwh{No, not correct: We have no pen-and-paper proof, just the
%   model. Clarify here}
% showing that
% extensive random testing fails to falsify the bisimilarity
% property. \mwh{Better way to state the previous?}

We formalize both the compilation procedure and the simulation
theorem in the PLT Redex model we developed for \lang (see Sec.~\ref{sec:syntax}),
and then attempt to falsify it via Redex's support for random
testing. Redex allows us
  to specify compilation as logical rules (an extension
  of typing), but then execute it algorithmically to
  automatically test whether simulation holds. This process revealed
  several bugs in compilation and the theorem statement.
%
  % us gain confidence that our original pen and paper proof of
  % simulation remains true with the addition of variable bounds. }
We ultimately plan to prove simulation in the Coq model.

%Turning to the simulation theorem: We first introduce notation
%used to specify the theorem.
We use the notation $\gg$ to
indicate the \emph{erasure} of stack and heap---the rhs is the same as
the lhs but with type annotations removed:
\begin{equation*}
  \begin{split}
    \heap  \gg & \dot \heap \\
    \varphi \gg & \dot \varphi
  \end{split}
\end{equation*}
In addition, when $\Gamma;\emptyset\vdash
\varphi$ and $\varphi$ is well-formed, we write $(\varphi,\heap,e) \gg_m (\dot \varphi, \dot \heap,
\dot e)$ to denote $\varphi \gg \dot \varphi$, $\heap \gg \dot \heap$
and $\Gamma;\Theta;\emptyset \vdash_m e \gg \dot e : \tau$ for some $\tau$ respectively. $\Gamma$ is omitted from the notation since the well-formedness of $\varphi$ and its consistency with respect to $\Gamma$ imply that $e$ must be closed under $\varphi$, allowing us to recover $\Gamma$ from $\varphi$.
Finally, we use $\xrightarrow{\cdot}^*$ to denote the transitive closure of the
reduction relation of $\elang$. Unlike the $\lang$, the semantics of
$\elang$ does not distinguish checked and unchecked regions.

Fig.~\ref{fig:checkedc-simulation-ref} gives an overview of 
the simulation theorem.\footnote{We ellide the  possibility of $\dot e_1$ evaluating to $\ebounds$ or $\enull$ in the diagram for readability.} The simulation theorem is specified in a way
that is similar to the one by~\citet{merigoux2021catala}.

An ordinary simulation property would
replace the middle and bottom parts of the figure with the
following: \[(\dot \varphi_0, \dot \heap_0, \dot e_0) 
  \xrightarrow{\cdot}^* (\dot \varphi_1, \dot \heap_1, \dot e_1)\]
Instead, we relate two erased configurations using the relation $\sim$,
which only requires that the two configurations will eventually reduce
to the same state.

\ignore{
 We formulate our simulation theorem differently
because the standard simulation theorem imposes a very strong
syntactic restriction to the compilation strategy. Very often, $(\dot
\varphi_0, \dot \heap_0, \dot e_0)$ reduces to a term that is
semantically equivalent to $(\dot \varphi_1, \dot \heap_1, \dot e_1)$,
but we are unable to syntactically equate the two configurations due
to the extra binders generated for dynamic checks and ANF
transformation. In earlier versions of the Redex model, we attempted
to change the compilation rules so the configurations could match
syntactically. However, the approach scaled poorly as we added
additional rules. 
This slight relaxation on the equivalence relation
between target configurations allows us to specify compilation more
naturally without having to worry about syntactic constraints.
}

% The two theorems are translation preservation and simulation. We donate $\xrightarrow{c}$ as the transition semantics of CLight.
\begin{thm}\label{simulation-thm}[Simulation ($\sim$)]
For \lang expressions $e_0$, stacks $\varphi_0$, $\varphi_1$, and heap snapshots $\heap_0$, $\heap_1$, 
if $\heap_0 \vdash \varphi_0$, $(\varphi_0,\heap_0,e_0)\gg_c (\dot \varphi_0,\dot \heap_0, \dot e_0)$,
and if there exists some $r_1$ such that $(\varphi_0, \heap_0, e_0)
\rightarrow_c (\varphi_1, \heap_1, r_1)$, then the following facts hold:

\begin{itemize}

\item if there exists $e_1$ such that $r=e_1$ and $(\varphi_1, \heap_1, e_1) \gg (\dot \varphi_1, \dot \heap_1, \dot e_1)$, then there exists some $\dot \varphi$,$\dot \heap$, $\dot e$, such that
$(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
\varphi,\dot \heap,\dot e)$ and $(\dot
\varphi_1,\dot \heap_1,\dot e_1) \xrightarrow{\cdot}^* (\dot \varphi,
\dot \heap,\dot e)$.

\item if $r_1 = \ebounds$ or $\enull$, then we have $(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
\dot \varphi_1,\dot \heap_1, r_1)$ where $\varphi_1 \gg \dot
\varphi_1$, $\heap_1 \gg \dot \heap_1$.

\end{itemize}
\end{thm}


% when $r_1 = e_1$ for
% some $e_1$ and
% $(\varphi_1, \heap_1, e_1) \gg (\dot \varphi_1, \dot \heap_1, \dot e_1)$, then
% there exists some $\dot \varphi$,$\dot \heap$, $\dot e$, such that
% $(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
% \varphi,\dot \heap,\dot e)$ and $(\dot
% \varphi_1,\dot \heap_1,\dot e_1) \xrightarrow{\cdot}^* (\dot \varphi,
% \dot \heap,\dot e)$. When $r_1 = \ebounds$ or $\enull$, we have $(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
% \dot \varphi_1,\dot \heap_1, r_1)$ where $\varphi_1 \gg \dot
% \varphi_1$, $\heap_1 \gg \dot \heap_1$.

% \begin{thm}[Simulation ($\sim$)]\label{simulation-thm}
% For \lang expressions $e_0$, stacks $\varphi_0$, $\varphi_1$, and heap snapshots $\heap_0$, $\heap_1$, 
% if $\emptyset;\emptyset;\emptyset \vdash_\cmode e_0 \gg \dot e_0 :\tau_0$,
% and if there exists some $r_1$ such that $(\varphi_0, \heap_0, e_0)
% \rightarrow_\cmode (\varphi_1, \heap_1, r_1)$, when $r_1 = e_1$ for
% some $e_1$ and
% $\emptyset;\emptyset;\emptyset \vdash_\cmode e_1 \gg \dot e_1 :\tau_1$ where $\tau_1 \sqsubseteq \tau_0$
% , then
% there exists some $\dot \varphi$,$\dot \heap$, $\dot e$, such that
% $(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
% \varphi,\dot \heap,\dot e)$ and $(\dot
% \varphi_1,\dot \heap_1,\dot e_1) \xrightarrow{\cdot}^* (\dot \varphi,
% \dot \heap,\dot e)$. When $r_1 = \ebounds$ or $\enull$, we have $(\dot \varphi_0, \dot \heap_0,\dot e_0) \xrightarrow{\cdot}^* (\dot
% \dot \varphi_1,\dot \heap_1, r_1)$ where $\varphi_1 \gg \dot
% \varphi_1$, $\heap_1 \gg \dot \heap_1$.
% \end{thm}

As our random generator never generates
$\euncheckedtext$ expressions (whose behavior could be undefined), we can only test a the simulation theorem 
as it relates to checked code. This limitation makes it
unnecessary to state the other direction of the simulation theorem
where $e_0$ is stuck, because Theorem~\ref{thm:progress} guarantees
that $e_0$ will never enter a stuck state if it is well-typed in
checked mode.

The current version of the Redex model has been tested against $23000$
expressions with depth less than $11$. Each expression can
reduce multiple steps, and we test simulation between every two
adjacent steps to cover a wider range of programs, particularly the
ones that have a non-empty heap.

\begin{figure}[t]
{\small
\[
\begin{array}{c}
\begin{tikzpicture}[
            > = stealth, % arrow head style
            shorten > = 1pt, % don't touch arrow head to node
            auto,
            node distance = 3cm
        ]

\begin{scope}[every node/.style={draw}]
    \node (A) at (0,1.5) {$\varphi_0,\heap_0, e_0$};
    \node (B) at (4,1.5) {$\varphi_1, \heap_1 ,e_1$};
    \node (C) at (0,0) {$\dot \varphi_0, \dot \heap_0 ,\dot e_0$};
    \node (D) at (4,0) {$\dot \varphi_1, \dot \heap_1, \dot e_1$};
    \node (E) at (2,-1.5) {$\dot \varphi,\dot \heap ,\dot e$};
\end{scope}
\begin{scope}[every edge/.style={draw=black}]

    \path [->] (A) edge node {$\longrightarrow_\cmode$} (B);
    \path [<->] (A) edge node {$\gg$} (C);
    \path [<->] (B) edge node {$\gg$} (D);
    \path [dashed,<->] (C) edge node {$\sim$} (D);
    \path [dashed,->] (C) edge node {$\xrightarrow{\cdot}^*$} (E);
    \path [dashed,->] (D) edge node[above] {$\xrightarrow{\cdot}^*$} (E);
\end{scope}

\end{tikzpicture}
\end{array}
\]
}
\caption{Simulation between \lang and \elang }
\label{fig:checkedc-simulation-ref}
\end{figure}

% \ignore
% {The two theorems can be best understood by the diagram in Fig.~\ref{fig:checkedc-simulation-ref}.
% % The diagram also indicates the simulation relation ($\sim$) among our formalization of the \checkedc Type System ($\vdash$), Semantics ($\longrightarrow$), Compilation ($\gg$), as well as the compiled C semantics ($\xrightarrow{c}$).
% On the top of the relation, we have type soundness theorem (Sec.~\ref{sec:theorem}) stating that every type-checked \lang program $e_0$ can transition via \lang semantics into a type-checked program $e_1$ by taking a checked step.
% The second line refers to that both $e_0$ and $e_1$ can be compiled to a C program $\dot e_0$ and $\dot e_1$, and such compilations always exist. The bottom two rewrites ($\xrightarrow{c}$) state that both $\dot e_0$ and $\dot e_1$ are transitioned finally to the same state $\dot e$. 

%  The simulation states that given any well-typed \lang expression $e_0$, its compiled C program as $\dot e_0$, if $e_0$ can transition one step to $e_1$, and there must exist the compiled C program $\dot e_1$, such that both $\dot e_0$ and $\dot e_1$ transition to the same final state $\dot e$ in C. The simulation relation $\sim$ is built on top of the "triangle" structure in Fig.~\ref{fig:checkedc-simulation-ref} stating that every \lang expression and its one step transitioned expression might be compiled to two different C program, but the C semantics always evaluates them to the same place.
% The translation preservation theorem is a support for the simulation theorem stating that for any well-typed \lang expression $e_0$,  its one step \checkedc transition expression $e_1$ must exist a compiled C program through the compilation process ($\gg$).

% A corollary of the simulation theorem states that for any \lang expression $e_0$ and its one step \lang transition expression $e_1$, such that $e_0 \longrightarrow e_1$, if $e_0$ contains a fault due to a unchecked block (the blame theorem tells us that if there is a fault in a \lang code, it must come from a unchecked block), and its compiled code $\dot e_0$ is evaluated to a fault state, the compiled code $\dot e_1$ for $e_1$ is always evaluated to the same fault state in C.
% This is an important property for a \lang compiler to preserve because any problematic program will be captured by running it long enough, so that enough random testing cases are able to capture all the bugs.
% In our formalization implementation, the type soundness theorem is proved through Coq, while the simulation theorem is validated through intensive random test case generation. We generate tens of thousands cases and cover all possible corner cases of the compilation. 
% }
% \ignore{
% \begin{figure*}[t]
%   \begin{subfigure}[b]{1\textwidth}
%     \begin{lstlisting}
% int deref_array (size_t n, nt_array_ptr<int> p : bounds(p, p + n)) {
%   return *p;
% }

% ...
% /* nt_array_ptr<int> p0 : bounds(p0, p0 + 5) */
% deref_array(5, p0);
%     \end{lstlisting}
%     \label{fig:chkcexamplederef}
%     \caption{\texttt{deref\_array} in \checkedc}
%   \end{subfigure}

%   \begin{subfigure}[b]{1\textwidth}
% \begin{lstlisting}
% int deref_array(size_t n, int *p) {
%   /* statically determine the definitions p_lo and p_hi */
%   int *p_lo = p;
%   int *p_hi = p + n;
%   /* runtime checks */
%   assert(p_lo <= p && p <= p_hi);
%   assert(p != NULL);
%   /* widening */
%   int p_derefed = *p;
%   if (p_derefed != '\0') {
%     if (p_hi == p) {
%       ++p_hi;
%     }
%   }
%   return p_derefed;
% }
% ...
% /* int *p0 */
% /* rho(p0) = p_lo, p_hi */
% deref_array(5, p0);
% \end{lstlisting}
% \caption{\texttt{deref\_array} in C}
%     \label{fig:cexamplederef}
%   \end{subfigure}

%   \begin{subfigure}[b]{\textwidth}
%     \begin{lstlisting}
% /* nt_array_ptr<int> p : bounds(e0, e1) */
% /* rho(p) = p_lo, p_hi */
% size_t x = strlen(p);
% if(x >= 1) {
%   *(p+1);
% }
%     \end{lstlisting}
%     \caption{\texttt{strlen} in \checkedc}
%     \label{fig:chkcexamplestrlen}
%   \end{subfigure}

%   \begin{subfigure}[b]{\textwidth}
%     \begin{lstlisting}
% /* nt_array_ptr<int> p : bounds(e0, e1) */
% /* rho(p) = p_lo, p_hi */
% /* runtime checks omitted */
% ...
% size_t x = strlen(p);
% int *p_hi_new = p + x;
% p_hi = max(p_hi, p_hi_new);
% if (x >= 1) {
%   /* null check for pointer arithmetic */
%   assert(p != NULL);
%   int *p_1 = p + 1;
%   /* null check for dereference */
%   assert(p_1 != NULL);
%   /* bounds check for dereference */
%   /* note how we are using p_hi rather than p + x */
%   assert(p_lo <= p_1 && p_1 <= p_hi);
%   ...
% }
%     \end{lstlisting}
%     \caption{\texttt{strlen} in C}
%     \label{fig:cexamplestrlen}
%   \end{subfigure}
% \caption{Compilation of null-terminated string dereference}
% \label{fig:compilationexample}
% \end{figure*}
% }

% \ignore{
% Fig.~\ref{fig:compilationexample} gives an example of how we compile the
% dereference of null-terminated strings by inserting explicit checks and
% bounds widening code. For readability, we present the example in real
% \checkedc and C syntax. At
% line 3-4 of Fig.~\ref{fig:cexamplederef}, we see how the upper and lower
% bounds are defined in terms of the arguments \code{p} and \code{n}
% according to the bounds annotations obtained during typechecking. This
% avoids the need to pass in bounds as extra arguments, thus maintaining
% compatibility with C code. When we call \code{deref_array} on
% \code{p0}, a string with size 5 (excluding the null character), there
% is no need to pass the bounds \code{p_lo} and \code{p_hi} stored on
% the stack. It is possible that \code{p_hi} has been widened
% before we reach line 21. The programmer will have to perform a
% \code{dynamic_bounds_cast} to recover the more precise bounds information. The if statement from line 10 to line 14
% attempts to widen the bound when the dereferenced result is not
% null. \todo[inline]{Show a full-fledged C program?} The widened upper bound will be available within the scope of
% \code{deref_array}, in contrast to the T-IfNT rule, which only
% remembers the widened bounds within the scope of the then branch of
% the if statement. 


% \todo[inline]{Widening can happen at every
%   dereference at runtime. Is that ok?} Fig.~\ref{fig:cexamplestrlen}
% shows how an invocation of \code{strlen} on null-termianted strings
% is compiled into C code. We perform the same runtime checks that
% happen during dereferencing. The widening code at line
% 8 updates \code{p}'s upper bound only if the result of
% \code{strlen} is larger than the value of the upper bound stored on
% the stack. This is another scenario where the runtime can be more precise
% than the statically determined bounds information.



% }



==> coq/Makefile <==
##########################################################################
##         #   The Coq Proof Assistant / The Coq Development Team       ##
##  v      #         Copyright INRIA, CNRS and contributors             ##
## <O___,, # (see version control and CREDITS file for authors & dates) ##
##   \VV/  ###############################################################
##    //   #    This file is distributed under the terms of the         ##
##         #     GNU Lesser General Public License Version 2.1          ##
##         #     (see LICENSE file for the text of the license)         ##
##########################################################################
## GNUMakefile for Coq 8.12.0

# For debugging purposes (must stay here, don't move below)
INITIAL_VARS := $(.VARIABLES)
# To implement recursion we save the name of the main Makefile
SELF := $(lastword $(MAKEFILE_LIST))
PARENT := $(firstword $(MAKEFILE_LIST))

# This file is generated by coq_makefile and contains many variable
# definitions, like the list of .v files or the path to Coq
include Makefile.conf

# Put in place old names
VFILES            := $(COQMF_VFILES)
MLIFILES          := $(COQMF_MLIFILES)
MLFILES           := $(COQMF_MLFILES)
MLGFILES          := $(COQMF_MLGFILES)
MLPACKFILES       := $(COQMF_MLPACKFILES)
MLLIBFILES        := $(COQMF_MLLIBFILES)
CMDLINE_VFILES    := $(COQMF_CMDLINE_VFILES)
INSTALLCOQDOCROOT := $(COQMF_INSTALLCOQDOCROOT)
OTHERFLAGS        := $(COQMF_OTHERFLAGS)
COQ_SRC_SUBDIRS   := $(COQMF_COQ_SRC_SUBDIRS)
OCAMLLIBS         := $(COQMF_OCAMLLIBS)
SRC_SUBDIRS       := $(COQMF_SRC_SUBDIRS)
COQLIBS           := $(COQMF_COQLIBS)
COQLIBS_NOML      := $(COQMF_COQLIBS_NOML)
CMDLINE_COQLIBS   := $(COQMF_CMDLINE_COQLIBS)
LOCAL             := $(COQMF_LOCAL)
COQLIB            := $(COQMF_COQLIB)
DOCDIR            := $(COQMF_DOCDIR)
OCAMLFIND         := $(COQMF_OCAMLFIND)
CAMLFLAGS         := $(COQMF_CAMLFLAGS)
HASNATDYNLINK     := $(COQMF_HASNATDYNLINK)
OCAMLWARN         := $(COQMF_WARN)

Makefile.conf: _CoqProject
	coq_makefile -f _CoqProject -o Makefile

# This file can be created by the user to hook into double colon rules or
# add any other Makefile code he may need
-include Makefile.local

# Parameters ##################################################################
#
# Parameters are make variable assignments.
# They can be passed to (each call to) make on the command line.
# They can also be put in Makefile.local once and for all.
# For retro-compatibility reasons they can be put in the _CoqProject, but this
# practice is discouraged since _CoqProject better not contain make specific
# code (be nice to user interfaces).

# Print shell commands (set to non empty)
VERBOSE ?=

# Time the Coq process (set to non empty), and how (see default value)
TIMED?=
TIMECMD?=
# Use command time on linux, gtime on Mac OS
TIMEFMT?="$@ (real: %e, user: %U, sys: %S, mem: %M ko)"
ifneq (,$(TIMED))
ifeq (0,$(shell command time -f "" true >/dev/null 2>/dev/null; echo $$?))
STDTIME?=command time -f $(TIMEFMT)
else
ifeq (0,$(shell gtime -f "" true >/dev/null 2>/dev/null; echo $$?))
STDTIME?=gtime -f $(TIMEFMT)
else
STDTIME?=command time
endif
endif
else
STDTIME?=command time -f $(TIMEFMT)
endif

ifneq (,$(COQBIN))
# add an ending /
COQBIN:=$(COQBIN)/
endif

# Coq binaries
COQC     ?= "$(COQBIN)coqc"
COQTOP   ?= "$(COQBIN)coqtop"
COQCHK   ?= "$(COQBIN)coqchk"
COQDEP   ?= "$(COQBIN)coqdep"
COQDOC   ?= "$(COQBIN)coqdoc"
COQPP    ?= "$(COQBIN)coqpp"
COQMKFILE ?= "$(COQBIN)coq_makefile"
OCAMLLIBDEP ?= "$(COQBIN)ocamllibdep"

# Timing scripts
COQMAKE_ONE_TIME_FILE ?= "$(COQLIB)/tools/make-one-time-file.py"
COQMAKE_BOTH_TIME_FILES ?= "$(COQLIB)/tools/make-both-time-files.py"
COQMAKE_BOTH_SINGLE_TIMING_FILES ?= "$(COQLIB)/tools/make-both-single-timing-files.py"
BEFORE ?=
AFTER ?=

# FIXME this should be generated by Coq (modules already linked by Coq)
CAMLDONTLINK=num,str,unix,dynlink,threads

# OCaml binaries
CAMLC       ?= "$(OCAMLFIND)" ocamlc   -c
CAMLOPTC    ?= "$(OCAMLFIND)" opt      -c
CAMLLINK    ?= "$(OCAMLFIND)" ocamlc   -linkpkg -dontlink $(CAMLDONTLINK)
CAMLOPTLINK ?= "$(OCAMLFIND)" opt      -linkpkg -dontlink $(CAMLDONTLINK)
CAMLDOC     ?= "$(OCAMLFIND)" ocamldoc
CAMLDEP     ?= "$(OCAMLFIND)" ocamldep -slash -ml-synonym .mlpack

# DESTDIR is prepended to all installation paths
DESTDIR ?=

# Debug builds, typically -g to OCaml, -debug to Coq.
CAMLDEBUG ?=
COQDEBUG ?=

# Extra packages to be linked in (as in findlib -package)
CAMLPKGS ?=

# Option for making timing files
TIMING?=
# Option for changing sorting of timing output file
TIMING_SORT_BY ?= auto
# Option for changing the fuzz parameter on the output file
TIMING_FUZZ ?= 0
# Option for changing whether to use real or user time for timing tables
TIMING_REAL?=
# Option for including the memory column(s)
TIMING_INCLUDE_MEM?=
# Option for sorting by the memory column
TIMING_SORT_BY_MEM?=
# Output file names for timed builds
TIME_OF_BUILD_FILE               ?= time-of-build.log
TIME_OF_BUILD_BEFORE_FILE        ?= time-of-build-before.log
TIME_OF_BUILD_AFTER_FILE         ?= time-of-build-after.log
TIME_OF_PRETTY_BUILD_FILE        ?= time-of-build-pretty.log
TIME_OF_PRETTY_BOTH_BUILD_FILE   ?= time-of-build-both.log
TIME_OF_PRETTY_BUILD_EXTRA_FILES ?= - # also output to the command line

TGTS ?=

########## End of parameters ##################################################
# What follows may be relevant to you only if you need to
# extend this Makefile.  If so, look for 'Extension point' here and
# put in Makefile.local double colon rules accordingly.
# E.g. to perform some work after the all target completes you can write
#
# post-all::
# 	echo "All done!"
#
# in Makefile.local
#
###############################################################################




# Flags #######################################################################
#
# We define a bunch of variables combining the parameters.
# To add additional flags to coq, coqchk or coqdoc, set the
# {COQ,COQCHK,COQDOC}EXTRAFLAGS variable to whatever you want to add.
# To overwrite the default choice and set your own flags entirely, set the
# {COQ,COQCHK,COQDOC}FLAGS variable.

SHOW := $(if $(VERBOSE),@true "",@echo "")
HIDE := $(if $(VERBOSE),,@)

TIMER=$(if $(TIMED), $(STDTIME), $(TIMECMD))

OPT?=

# The DYNOBJ and DYNLIB variables are used by "coqdep -dyndep var" in .v.d
ifeq '$(OPT)' '-byte'
USEBYTE:=true
DYNOBJ:=.cma
DYNLIB:=.cma
else
USEBYTE:=
DYNOBJ:=.cmxs
DYNLIB:=.cmxs
endif

# these variables are meant to be overridden if you want to add *extra* flags
COQEXTRAFLAGS?=
COQCHKEXTRAFLAGS?=
COQDOCEXTRAFLAGS?=

# these flags do NOT contain the libraries, to make them easier to overwrite
COQFLAGS?=-q $(OTHERFLAGS) $(COQEXTRAFLAGS)
COQCHKFLAGS?=-silent -o $(COQCHKEXTRAFLAGS)
COQDOCFLAGS?=-interpolate -utf8 $(COQDOCEXTRAFLAGS)

COQDOCLIBS?=$(COQLIBS_NOML)

# The version of Coq being run and the version of coq_makefile that
# generated this makefile
COQ_VERSION:=$(shell $(COQC) --print-version | cut -d " " -f 1)
COQMAKEFILE_VERSION:=8.12.0

COQSRCLIBS?= $(foreach d,$(COQ_SRC_SUBDIRS), -I "$(COQLIB)/$(d)")

CAMLFLAGS+=$(OCAMLLIBS) $(COQSRCLIBS)
# ocamldoc fails with unknown argument otherwise
CAMLDOCFLAGS:=$(filter-out -annot, $(filter-out -bin-annot, $(CAMLFLAGS)))
CAMLFLAGS+=$(OCAMLWARN)

ifneq (,$(TIMING))
TIMING_ARG=-time
ifeq (after,$(TIMING))
TIMING_EXT=after-timing
else
ifeq (before,$(TIMING))
TIMING_EXT=before-timing
else
TIMING_EXT=timing
endif
endif
else
TIMING_ARG=
endif

# Retro compatibility (DESTDIR is standard on Unix, DSTROOT is not)
ifdef DSTROOT
DESTDIR := $(DSTROOT)
endif

concat_path = $(if $(1),$(1)/$(if $(COQMF_WINDRIVE),$(subst $(COQMF_WINDRIVE),/,$(2)),$(2)),$(2))

COQLIBINSTALL = $(call concat_path,$(DESTDIR),$(COQLIB)/user-contrib)
COQDOCINSTALL = $(call concat_path,$(DESTDIR),$(DOCDIR)/user-contrib)
COQTOPINSTALL = $(call concat_path,$(DESTDIR),$(COQLIB)/toploop)

# Files #######################################################################
#
# We here define a bunch of variables about the files being part of the
# Coq project in order to ease the writing of build target and build rules

VDFILE := .Makefile.d

ALLSRCFILES := \
	$(MLGFILES) \
	$(MLFILES) \
	$(MLPACKFILES) \
	$(MLLIBFILES) \
	$(MLIFILES)

# helpers
vo_to_obj = $(addsuffix .o,\
  $(filter-out Warning: Error:,\
  $(shell $(COQTOP) -q -noinit -batch -quiet -print-mod-uid $(1))))
strip_dotslash = $(patsubst ./%,%,$(1))

# without this we get undefined variables in the expansion for the
# targets of the [deprecated,use-mllib-or-mlpack] rule
with_undef = $(if $(filter-out undefined, $(origin $(1))),$($(1)))

VO = vo
VOS = vos

VOFILES = $(VFILES:.v=.$(VO))
GLOBFILES = $(VFILES:.v=.glob)
HTMLFILES = $(VFILES:.v=.html)
GHTMLFILES = $(VFILES:.v=.g.html)
BEAUTYFILES = $(addsuffix .beautified,$(VFILES))
TEXFILES = $(VFILES:.v=.tex)
GTEXFILES = $(VFILES:.v=.g.tex)
CMOFILES = \
	$(MLGFILES:.mlg=.cmo) \
	$(MLFILES:.ml=.cmo) \
	$(MLPACKFILES:.mlpack=.cmo)
CMXFILES = $(CMOFILES:.cmo=.cmx)
OFILES = $(CMXFILES:.cmx=.o)
CMAFILES = $(MLLIBFILES:.mllib=.cma) $(MLPACKFILES:.mlpack=.cma)
CMXAFILES = $(CMAFILES:.cma=.cmxa)
CMIFILES = \
	$(CMOFILES:.cmo=.cmi) \
	$(MLIFILES:.mli=.cmi)
# the /if/ is because old _CoqProject did not list a .ml(pack|lib) but just
# a .mlg file
CMXSFILES = \
	$(MLPACKFILES:.mlpack=.cmxs) \
	$(CMXAFILES:.cmxa=.cmxs) \
	$(if $(MLPACKFILES)$(CMXAFILES),,\
		$(MLGFILES:.mlg=.cmxs) $(MLFILES:.ml=.cmxs))

# files that are packed into a plugin (no extension)
PACKEDFILES = \
	$(call strip_dotslash, \
	  $(foreach lib, \
	    $(call strip_dotslash, \
	       $(MLPACKFILES:.mlpack=_MLPACK_DEPENDENCIES)),$(call with_undef,$(lib))))
# files that are archived into a .cma (mllib)
LIBEDFILES = \
	$(call strip_dotslash, \
	  $(foreach lib, \
	    $(call strip_dotslash, \
	       $(MLLIBFILES:.mllib=_MLLIB_DEPENDENCIES)),$(call with_undef,$(lib))))
CMIFILESTOINSTALL = $(filter-out $(addsuffix .cmi,$(PACKEDFILES)),$(CMIFILES))
CMOFILESTOINSTALL = $(filter-out $(addsuffix .cmo,$(PACKEDFILES)),$(CMOFILES))
OBJFILES = $(call vo_to_obj,$(VOFILES))
ALLNATIVEFILES = \
	$(OBJFILES:.o=.cmi) \
	$(OBJFILES:.o=.cmx) \
	$(OBJFILES:.o=.cmxs)
# trick: wildcard filters out non-existing files, so that `install` doesn't show
# warnings and `clean` doesn't pass to rm a list of files that is too long for
# the shell.
NATIVEFILES = $(wildcard $(ALLNATIVEFILES))
FILESTOINSTALL = \
	$(VOFILES) \
	$(VFILES) \
	$(GLOBFILES) \
	$(NATIVEFILES) \
	$(CMIFILESTOINSTALL)
BYTEFILESTOINSTALL = \
	$(CMOFILESTOINSTALL) \
	$(CMAFILES)
ifeq '$(HASNATDYNLINK)' 'true'
DO_NATDYNLINK = yes
FILESTOINSTALL += $(CMXSFILES) $(CMXAFILES) $(CMOFILESTOINSTALL:.cmo=.cmx)
else
DO_NATDYNLINK =
endif

ALLDFILES = $(addsuffix .d,$(ALLSRCFILES)) $(VDFILE)

# Compilation targets #########################################################

all:
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" pre-all
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" real-all
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" post-all
.PHONY: all

all.timing.diff:
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" pre-all
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" real-all.timing.diff TIME_OF_PRETTY_BUILD_EXTRA_FILES=""
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" post-all
.PHONY: all.timing.diff

ifeq (0,$(TIMING_REAL))
TIMING_REAL_ARG :=
TIMING_USER_ARG := --user
else
ifeq (1,$(TIMING_REAL))
TIMING_REAL_ARG := --real
TIMING_USER_ARG :=
else
TIMING_REAL_ARG :=
TIMING_USER_ARG :=
endif
endif

ifeq (0,$(TIMING_INCLUDE_MEM))
TIMING_INCLUDE_MEM_ARG := --no-include-mem
else
TIMING_INCLUDE_MEM_ARG :=
endif

ifeq (1,$(TIMING_SORT_BY_MEM))
TIMING_SORT_BY_MEM_ARG := --sort-by-mem
else
TIMING_SORT_BY_MEM_ARG :=
endif

make-pretty-timed-before:: TIME_OF_BUILD_FILE=$(TIME_OF_BUILD_BEFORE_FILE)
make-pretty-timed-after:: TIME_OF_BUILD_FILE=$(TIME_OF_BUILD_AFTER_FILE)
make-pretty-timed make-pretty-timed-before make-pretty-timed-after::
	$(HIDE)rm -f pretty-timed-success.ok
	$(HIDE)($(MAKE) --no-print-directory -f "$(PARENT)" $(TGTS) TIMED=1 2>&1 && touch pretty-timed-success.ok) | tee -a $(TIME_OF_BUILD_FILE)
	$(HIDE)rm pretty-timed-success.ok # must not be -f; must fail if the touch failed
print-pretty-timed::
	$(HIDE)$(COQMAKE_ONE_TIME_FILE) $(TIMING_INCLUDE_MEM_ARG) $(TIMING_SORT_BY_MEM_ARG) $(TIMING_REAL_ARG) $(TIME_OF_BUILD_FILE) $(TIME_OF_PRETTY_BUILD_FILE) $(TIME_OF_PRETTY_BUILD_EXTRA_FILES)
print-pretty-timed-diff::
	$(HIDE)$(COQMAKE_BOTH_TIME_FILES) --sort-by=$(TIMING_SORT_BY) $(TIMING_INCLUDE_MEM_ARG) $(TIMING_SORT_BY_MEM_ARG) $(TIMING_REAL_ARG) $(TIME_OF_BUILD_AFTER_FILE) $(TIME_OF_BUILD_BEFORE_FILE) $(TIME_OF_PRETTY_BOTH_BUILD_FILE) $(TIME_OF_PRETTY_BUILD_EXTRA_FILES)
ifeq (,$(BEFORE))
print-pretty-single-time-diff::
	@echo 'Error: Usage: $(MAKE) print-pretty-single-time-diff AFTER=path/to/file.v.after-timing BEFORE=path/to/file.v.before-timing'
	$(HIDE)false
else
ifeq (,$(AFTER))
print-pretty-single-time-diff::
	@echo 'Error: Usage: $(MAKE) print-pretty-single-time-diff AFTER=path/to/file.v.after-timing BEFORE=path/to/file.v.before-timing'
	$(HIDE)false
else
print-pretty-single-time-diff::
	$(HIDE)$(COQMAKE_BOTH_SINGLE_TIMING_FILES) --fuzz=$(TIMING_FUZZ) --sort-by=$(TIMING_SORT_BY) $(TIMING_USER_ARG) $(AFTER) $(BEFORE) $(TIME_OF_PRETTY_BUILD_FILE) $(TIME_OF_PRETTY_BUILD_EXTRA_FILES)
endif
endif
pretty-timed:
	$(HIDE)$(MAKE) --no-print-directory -f "$(PARENT)" make-pretty-timed
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" print-pretty-timed
.PHONY: pretty-timed make-pretty-timed make-pretty-timed-before make-pretty-timed-after print-pretty-timed print-pretty-timed-diff print-pretty-single-time-diff

# Extension points for actions to be performed before/after the all target
pre-all::
	@# Extension point
	$(HIDE)if [ "$(COQMAKEFILE_VERSION)" != "$(COQ_VERSION)" ]; then\
	  echo "W: This Makefile was generated by Coq $(COQMAKEFILE_VERSION)";\
	  echo "W: while the current Coq version is $(COQ_VERSION)";\
	fi
.PHONY: pre-all

post-all::
	@# Extension point
.PHONY: post-all

real-all: $(VOFILES) $(if $(USEBYTE),bytefiles,optfiles)
.PHONY: real-all

real-all.timing.diff: $(VOFILES:.vo=.v.timing.diff)
.PHONY: real-all.timing.diff

bytefiles: $(CMOFILES) $(CMAFILES)
.PHONY: bytefiles

optfiles: $(if $(DO_NATDYNLINK),$(CMXSFILES))
.PHONY: optfiles

# FIXME, see Ralf's bugreport
# quick is deprecated, now renamed vio
vio: $(VOFILES:.vo=.vio)
.PHONY: vio
quick: vio
	$(warning "'make quick' is deprecated, use 'make vio' or consider using 'vos' files")
.PHONY: quick

vio2vo:
	$(TIMER) $(COQC) $(COQDEBUG) $(COQFLAGS) $(COQLIBS) \
		-schedule-vio2vo $(J) $(VOFILES:%.vo=%.vio)
.PHONY: vio2vo

# quick2vo is undocumented
quick2vo:
	$(HIDE)make -j $(J) vio
	$(HIDE)VIOFILES=$$(for vofile in $(VOFILES); do \
	  viofile="$$(echo "$$vofile" | sed "s/\.vo$$/.vio/")"; \
	  if [ "$$vofile" -ot "$$viofile" -o ! -e "$$vofile" ]; then printf "$$viofile "; fi; \
	done); \
	echo "VIO2VO: $$VIOFILES"; \
	if [ -n "$$VIOFILES" ]; then \
	  $(TIMER) $(COQC) $(COQDEBUG) $(COQFLAGS) $(COQLIBS) -schedule-vio2vo $(J) $$VIOFILES; \
	fi
.PHONY: quick2vo

checkproofs:
	$(TIMER) $(COQC) $(COQDEBUG) $(COQFLAGS) $(COQLIBS) \
		-schedule-vio-checking $(J) $(VOFILES:%.vo=%.vio)
.PHONY: checkproofs

vos: $(VOFILES:%.vo=%.vos)
.PHONY: vos

vok: $(VOFILES:%.vo=%.vok)
.PHONY: vok

validate: $(VOFILES)
	$(TIMER) $(COQCHK) $(COQCHKFLAGS) $(COQLIBS) $^
.PHONY: validate

only: $(TGTS)
.PHONY: only

# Documentation targets #######################################################

html: $(GLOBFILES) $(VFILES)
	$(SHOW)'COQDOC -d html $(GAL)'
	$(HIDE)mkdir -p html
	$(HIDE)$(COQDOC) \
		-toc $(COQDOCFLAGS) -html $(GAL) $(COQDOCLIBS) -d html $(VFILES)

mlihtml: $(MLIFILES:.mli=.cmi)
	$(SHOW)'CAMLDOC -d $@'
	$(HIDE)mkdir $@ || rm -rf $@/*
	$(HIDE)$(CAMLDOC) -html \
		-d $@ -m A $(CAMLDEBUG) $(CAMLDOCFLAGS) $(MLIFILES)

all-mli.tex: $(MLIFILES:.mli=.cmi)
	$(SHOW)'CAMLDOC -latex $@'
	$(HIDE)$(CAMLDOC) -latex \
		-o $@ -m A $(CAMLDEBUG) $(CAMLDOCFLAGS) $(MLIFILES)

all.ps: $(VFILES)
	$(SHOW)'COQDOC -ps $(GAL)'
	$(HIDE)$(COQDOC) \
		-toc $(COQDOCFLAGS) -ps $(GAL) $(COQDOCLIBS) \
		-o $@ `$(COQDEP) -sort $(VFILES)`

all.pdf: $(VFILES)
	$(SHOW)'COQDOC -pdf $(GAL)'
	$(HIDE)$(COQDOC) \
		-toc $(COQDOCFLAGS) -pdf $(GAL) $(COQDOCLIBS) \
		-o $@ `$(COQDEP) -sort $(VFILES)`

# FIXME: not quite right, since the output name is different
gallinahtml: GAL=-g
gallinahtml: html

all-gal.ps: GAL=-g
all-gal.ps: all.ps

all-gal.pdf: GAL=-g
all-gal.pdf: all.pdf

# ?
beautify: $(BEAUTYFILES)
	for file in $^; do mv $${file%.beautified} $${file%beautified}old && mv $${file} $${file%.beautified}; done
	@echo 'Do not do "make clean" until you are sure that everything went well!'
	@echo 'If there were a problem, execute "for file in $$(find . -name \*.v.old -print); do mv $${file} $${file%.old}; done" in your shell/'
.PHONY: beautify

# Installation targets ########################################################
#
# There rules can be extended in Makefile.local
# Extensions can't assume when they run.

install:
	$(HIDE)code=0; for f in $(FILESTOINSTALL); do\
	 if ! [ -f "$$f" ]; then >&2 echo $$f does not exist; code=1; fi \
	done; exit $$code
	$(HIDE)for f in $(FILESTOINSTALL); do\
	 df="`$(COQMKFILE) -destination-of "$$f" $(COQLIBS)`";\
	 if [ "$$?" != "0" -o -z "$$df" ]; then\
	   echo SKIP "$$f" since it has no logical path;\
	 else\
	   install -d "$(COQLIBINSTALL)/$$df" &&\
	   install -m 0644 "$$f" "$(COQLIBINSTALL)/$$df" &&\
	   echo INSTALL "$$f" "$(COQLIBINSTALL)/$$df";\
	 fi;\
	done
	$(HIDE)$(MAKE) install-extra -f "$(SELF)"
install-extra::
	@# Extension point
.PHONY: install install-extra

install-byte:
	$(HIDE)for f in $(BYTEFILESTOINSTALL); do\
	 df="`$(COQMKFILE) -destination-of "$$f" $(COQLIBS)`";\
	 if [ "$$?" != "0" -o -z "$$df" ]; then\
	   echo SKIP "$$f" since it has no logical path;\
	 else\
	   install -d "$(COQLIBINSTALL)/$$df" &&\
	   install -m 0644 "$$f" "$(COQLIBINSTALL)/$$df" &&\
	   echo INSTALL "$$f" "$(COQLIBINSTALL)/$$df";\
	 fi;\
	done

install-doc:: html mlihtml
	@# Extension point
	$(HIDE)install -d "$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/html"
	$(HIDE)for i in html/*; do \
	 dest="$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/$$i";\
	 install -m 0644 "$$i" "$$dest";\
	 echo INSTALL "$$i" "$$dest";\
	done
	$(HIDE)install -d \
		"$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/mlihtml"
	$(HIDE)for i in mlihtml/*; do \
	 dest="$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/$$i";\
	 install -m 0644 "$$i" "$$dest";\
	 echo INSTALL "$$i" "$$dest";\
	done
.PHONY: install-doc

uninstall::
	@# Extension point
	$(HIDE)for f in $(FILESTOINSTALL); do \
	 df="`$(COQMKFILE) -destination-of "$$f" $(COQLIBS)`" &&\
	 instf="$(COQLIBINSTALL)/$$df/`basename $$f`" &&\
	 rm -f "$$instf" &&\
	 echo RM "$$instf" &&\
	 (rmdir "$(call concat_path,,$(COQLIBINSTALL)/$$df/)" 2>/dev/null || true); \
	done
.PHONY: uninstall

uninstall-doc::
	@# Extension point
	$(SHOW)'RM $(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/html'
	$(HIDE)rm -rf "$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/html"
	$(SHOW)'RM $(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/mlihtml'
	$(HIDE)rm -rf "$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/mlihtml"
	$(HIDE) rmdir "$(COQDOCINSTALL)/$(INSTALLCOQDOCROOT)/" || true
.PHONY: uninstall-doc

# Cleaning ####################################################################
#
# There rules can be extended in Makefile.local
# Extensions can't assume when they run.

clean::
	@# Extension point
	$(SHOW)'CLEAN'
	$(HIDE)rm -f $(CMOFILES)
	$(HIDE)rm -f $(CMIFILES)
	$(HIDE)rm -f $(CMAFILES)
	$(HIDE)rm -f $(CMOFILES:.cmo=.cmx)
	$(HIDE)rm -f $(CMXAFILES)
	$(HIDE)rm -f $(CMXSFILES)
	$(HIDE)rm -f $(CMOFILES:.cmo=.o)
	$(HIDE)rm -f $(CMXAFILES:.cmxa=.a)
	$(HIDE)rm -f $(MLGFILES:.mlg=.ml)
	$(HIDE)rm -f $(ALLDFILES)
	$(HIDE)rm -f $(NATIVEFILES)
	$(HIDE)find . -name .coq-native -type d -empty -delete
	$(HIDE)rm -f $(VOFILES)
	$(HIDE)rm -f $(VOFILES:.vo=.vio)
	$(HIDE)rm -f $(VOFILES:.vo=.vos)
	$(HIDE)rm -f $(VOFILES:.vo=.vok)
	$(HIDE)rm -f $(BEAUTYFILES) $(VFILES:=.old)
	$(HIDE)rm -f all.ps all-gal.ps all.pdf all-gal.pdf all.glob all-mli.tex
	$(HIDE)rm -f $(VFILES:.v=.glob)
	$(HIDE)rm -f $(VFILES:.v=.tex)
	$(HIDE)rm -f $(VFILES:.v=.g.tex)
	$(HIDE)rm -f pretty-timed-success.ok
	$(HIDE)rm -rf html mlihtml
.PHONY: clean

cleanall:: clean
	@# Extension point
	$(SHOW)'CLEAN *.aux *.timing'
	$(HIDE)rm -f $(foreach f,$(VFILES:.v=),$(dir $(f)).$(notdir $(f)).aux)
	$(HIDE)rm -f $(TIME_OF_BUILD_FILE) $(TIME_OF_BUILD_BEFORE_FILE) $(TIME_OF_BUILD_AFTER_FILE) $(TIME_OF_PRETTY_BUILD_FILE) $(TIME_OF_PRETTY_BOTH_BUILD_FILE)
	$(HIDE)rm -f $(VOFILES:.vo=.v.timing)
	$(HIDE)rm -f $(VOFILES:.vo=.v.before-timing)
	$(HIDE)rm -f $(VOFILES:.vo=.v.after-timing)
	$(HIDE)rm -f $(VOFILES:.vo=.v.timing.diff)
	$(HIDE)rm -f .lia.cache .nia.cache
.PHONY: cleanall

archclean::
	@# Extension point
	$(SHOW)'CLEAN *.cmx *.o'
	$(HIDE)rm -f $(NATIVEFILES)
	$(HIDE)rm -f $(CMOFILES:%.cmo=%.cmx)
.PHONY: archclean


# Compilation rules ###########################################################

$(MLIFILES:.mli=.cmi): %.cmi: %.mli
	$(SHOW)'CAMLC -c $<'
	$(HIDE)$(TIMER) $(CAMLC) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) $<

$(MLGFILES:.mlg=.ml): %.ml: %.mlg
	$(SHOW)'COQPP $<'
	$(HIDE)$(COQPP) $<

# Stupid hack around a deficient syntax: we cannot concatenate two expansions
$(filter %.cmo, $(MLFILES:.ml=.cmo) $(MLGFILES:.mlg=.cmo)): %.cmo: %.ml
	$(SHOW)'CAMLC -c $<'
	$(HIDE)$(TIMER) $(CAMLC) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) $<

# Same hack
$(filter %.cmx, $(MLFILES:.ml=.cmx) $(MLGFILES:.mlg=.cmx)): %.cmx: %.ml
	$(SHOW)'CAMLOPT -c $(FOR_PACK) $<'
	$(HIDE)$(TIMER) $(CAMLOPTC) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) $(FOR_PACK) $<


$(MLLIBFILES:.mllib=.cmxs): %.cmxs: %.cmxa
	$(SHOW)'CAMLOPT -shared -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) \
		-linkall -shared -o $@ $<

$(MLLIBFILES:.mllib=.cma): %.cma: | %.mllib
	$(SHOW)'CAMLC -a -o $@'
	$(HIDE)$(TIMER) $(CAMLLINK) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) -a -o $@ $^

$(MLLIBFILES:.mllib=.cmxa): %.cmxa: | %.mllib
	$(SHOW)'CAMLOPT -a -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) -a -o $@ $^


$(MLPACKFILES:.mlpack=.cmxs): %.cmxs: %.cmxa
	$(SHOW)'CAMLOPT -shared -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) \
		-shared -linkall -o $@ $<

$(MLPACKFILES:.mlpack=.cmxa): %.cmxa: %.cmx
	$(SHOW)'CAMLOPT -a -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) -a -o $@ $<

$(MLPACKFILES:.mlpack=.cma): %.cma: %.cmo | %.mlpack
	$(SHOW)'CAMLC -a -o $@'
	$(HIDE)$(TIMER) $(CAMLLINK) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) -a -o $@ $^

$(MLPACKFILES:.mlpack=.cmo): %.cmo: | %.mlpack
	$(SHOW)'CAMLC -pack -o $@'
	$(HIDE)$(TIMER) $(CAMLLINK) $(CAMLDEBUG) $(CAMLFLAGS) -pack -o $@ $^

$(MLPACKFILES:.mlpack=.cmx): %.cmx: | %.mlpack
	$(SHOW)'CAMLOPT -pack -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) -pack -o $@ $^

# This rule is for _CoqProject with no .mllib nor .mlpack
$(filter-out $(MLLIBFILES:.mllib=.cmxs) $(MLPACKFILES:.mlpack=.cmxs) $(addsuffix .cmxs,$(PACKEDFILES)) $(addsuffix .cmxs,$(LIBEDFILES)),$(MLFILES:.ml=.cmxs) $(MLGFILES:.mlg=.cmxs)): %.cmxs: %.cmx
	$(SHOW)'[deprecated,use-mllib-or-mlpack] CAMLOPT -shared -o $@'
	$(HIDE)$(TIMER) $(CAMLOPTLINK) $(CAMLDEBUG) $(CAMLFLAGS) $(CAMLPKGS) \
		-shared -o $@ $<

ifneq (,$(TIMING))
TIMING_EXTRA = > $<.$(TIMING_EXT)
else
TIMING_EXTRA =
endif

$(VOFILES): %.vo: %.v
	$(SHOW)COQC $<
	$(HIDE)$(TIMER) $(COQC) $(COQDEBUG) $(TIMING_ARG) $(COQFLAGS) $(COQLIBS) $< $(TIMING_EXTRA)

# FIXME ?merge with .vo / .vio ?
$(GLOBFILES): %.glob: %.v
	$(TIMER) $(COQC) $(COQDEBUG) $(COQFLAGS) $(COQLIBS) $<

$(VFILES:.v=.vio): %.vio: %.v
	$(SHOW)COQC -vio $<
	$(HIDE)$(TIMER) $(COQC) -vio $(COQDEBUG) $(COQFLAGS) $(COQLIBS) $<

$(VFILES:.v=.vos): %.vos: %.v
	$(SHOW)COQC -vos $<
	$(HIDE)$(TIMER) $(COQC) -vos $(COQDEBUG) $(COQFLAGS) $(COQLIBS) $<

$(VFILES:.v=.vok): %.vok: %.v
	$(SHOW)COQC -vok $<
	$(HIDE)$(TIMER) $(COQC) -vok $(COQDEBUG) $(COQFLAGS) $(COQLIBS) $<

$(addsuffix .timing.diff,$(VFILES)): %.timing.diff : %.before-timing %.after-timing
	$(SHOW)PYTHON TIMING-DIFF $*.{before,after}-timing
	$(HIDE)$(MAKE) --no-print-directory -f "$(SELF)" print-pretty-single-time-diff BEFORE=$*.before-timing AFTER=$*.after-timing TIME_OF_PRETTY_BUILD_FILE="$@"

$(BEAUTYFILES): %.v.beautified: %.v
	$(SHOW)'BEAUTIFY $<'
	$(HIDE)$(TIMER) $(COQC) $(COQDEBUG) $(COQFLAGS) $(COQLIBS) -beautify $<

$(TEXFILES): %.tex: %.v
	$(SHOW)'COQDOC -latex $<'
	$(HIDE)$(COQDOC) $(COQDOCFLAGS) -latex $< -o $@

$(GTEXFILES): %.g.tex: %.v
	$(SHOW)'COQDOC -latex -g $<'
	$(HIDE)$(COQDOC) $(COQDOCFLAGS) -latex -g $< -o $@

$(HTMLFILES): %.html: %.v %.glob
	$(SHOW)'COQDOC -html $<'
	$(HIDE)$(COQDOC) $(COQDOCFLAGS) -html $< -o $@

$(GHTMLFILES): %.g.html: %.v %.glob
	$(SHOW)'COQDOC -html -g $<'
	$(HIDE)$(COQDOC) $(COQDOCFLAGS)  -html -g $< -o $@

# Dependency files ############################################################

ifndef MAKECMDGOALS
  -include $(ALLDFILES)
else
  ifneq ($(filter-out archclean clean cleanall printenv make-pretty-timed make-pretty-timed-before make-pretty-timed-after print-pretty-timed print-pretty-timed-diff print-pretty-single-time-diff,$(MAKECMDGOALS)),)
   -include $(ALLDFILES)
 endif
endif

.SECONDARY: $(ALLDFILES)

redir_if_ok = > "$@" || ( RV=$$?; rm -f "$@"; exit $$RV )

GENMLFILES:=$(MLGFILES:.mlg=.ml)
$(addsuffix .d,$(ALLSRCFILES)): $(GENMLFILES)

$(addsuffix .d,$(MLIFILES)): %.mli.d: %.mli
	$(SHOW)'CAMLDEP $<'
	$(HIDE)$(CAMLDEP) $(OCAMLLIBS) "$<" $(redir_if_ok)

$(addsuffix .d,$(MLGFILES)): %.mlg.d: %.ml
	$(SHOW)'CAMLDEP $<'
	$(HIDE)$(CAMLDEP) $(OCAMLLIBS) "$<" $(redir_if_ok)

$(addsuffix .d,$(MLFILES)): %.ml.d: %.ml
	$(SHOW)'CAMLDEP $<'
	$(HIDE)$(CAMLDEP) $(OCAMLLIBS) "$<" $(redir_if_ok)

$(addsuffix .d,$(MLLIBFILES)): %.mllib.d: %.mllib
	$(SHOW)'OCAMLLIBDEP $<'
	$(HIDE)$(OCAMLLIBDEP) -c $(OCAMLLIBS) "$<" $(redir_if_ok)

$(addsuffix .d,$(MLPACKFILES)): %.mlpack.d: %.mlpack
	$(SHOW)'OCAMLLIBDEP $<'
	$(HIDE)$(OCAMLLIBDEP) -c $(OCAMLLIBS) "$<" $(redir_if_ok)

# If this makefile is created using a _CoqProject we have coqdep get
# options from it. This avoids argument length limits for pathological
# projects. Note that extra options might be on the command line.
VDFILE_FLAGS:=$(if _CoqProject,-f _CoqProject,) $(CMDLINE_COQLIBS) $(CMDLINE_VFILES)

$(VDFILE): $(VFILES)
	$(SHOW)'COQDEP VFILES'
	$(HIDE)$(COQDEP) -vos -dyndep var $(VDFILE_FLAGS) $(redir_if_ok)

# Misc ########################################################################

byte:
	$(HIDE)$(MAKE) all "OPT:=-byte" -f "$(SELF)"
.PHONY: byte

opt:
	$(HIDE)$(MAKE) all "OPT:=-opt" -f "$(SELF)"
.PHONY:	opt

# This is deprecated.  To extend this makefile use
# extension points and Makefile.local
printenv::
	$(warning printenv is deprecated)
	$(warning write extensions in Makefile.local or include Makefile.conf)
	@echo 'LOCAL = $(LOCAL)'
	@echo 'COQLIB = $(COQLIB)'
	@echo 'DOCDIR = $(DOCDIR)'
	@echo 'OCAMLFIND = $(OCAMLFIND)'
	@echo 'HASNATDYNLINK = $(HASNATDYNLINK)'
	@echo 'SRC_SUBDIRS = $(SRC_SUBDIRS)'
	@echo 'COQ_SRC_SUBDIRS = $(COQ_SRC_SUBDIRS)'
	@echo 'OCAMLFIND = $(OCAMLFIND)'
	@echo 'PP = $(PP)'
	@echo 'COQFLAGS = $(COQFLAGS)'
	@echo 'COQLIB = $(COQLIBS)'
	@echo 'COQLIBINSTALL = $(COQLIBINSTALL)'
	@echo 'COQDOCINSTALL = $(COQDOCINSTALL)'
.PHONY:	printenv

# Generate a .merlin file.  If you need to append directives to this
# file you can extend the merlin-hook target in Makefile.local
.merlin:
	$(SHOW)'FILL .merlin'
	$(HIDE)echo 'FLG $(COQMF_CAMLFLAGS)' > .merlin
	$(HIDE)echo 'B $(COQLIB)' >> .merlin
	$(HIDE)echo 'S $(COQLIB)' >> .merlin
	$(HIDE)$(foreach d,$(COQ_SRC_SUBDIRS), \
		echo 'B $(COQLIB)$(d)' >> .merlin;)
	$(HIDE)$(foreach d,$(COQ_SRC_SUBDIRS), \
		echo 'S $(COQLIB)$(d)' >> .merlin;)
	$(HIDE)$(foreach d,$(SRC_SUBDIRS), echo 'B $(d)' >> .merlin;)
	$(HIDE)$(foreach d,$(SRC_SUBDIRS), echo 'S $(d)' >> .merlin;)
	$(HIDE)$(MAKE) merlin-hook -f "$(SELF)"
.PHONY: merlin

merlin-hook::
	@# Extension point
.PHONY: merlin-hook

# prints all variables
debug:
	$(foreach v,\
		$(sort $(filter-out $(INITIAL_VARS) INITIAL_VARS,\
	       		$(.VARIABLES))),\
	       	$(info $(v) = $($(v))))
.PHONY: debug

.DEFAULT_GOAL := all

# Local Variables:
# mode: makefile-gmake
# End:


==> coq/oldtext <==

(*
Lemma heapWArg :
  forall D S H H' env e t,
    well_typed_arg D S H env e t ->
    @heap_consistent D H' H ->
    well_typed_arg D S H' env e t.
Proof.
  intros D S H H' env es tvl WT HC.
  induction WT; intros; eauto.
  eapply ArgLit.
  assumption.
  unfold heap_consistent in HC.
  inv H1. econstructor. apply H4.
  apply HC. assumption.
  apply H2. assumption.
  eapply ArgVar.
  apply H0. apply H1. apply H2. assumption.
Qed.

Lemma heapWArgs :
  forall D S H H' env es tvl,
    well_typed_args D H S env es tvl ->
    @heap_consistent D H' H ->
    well_typed_args D H' S env es tvl.
Proof.
  intros D S H H' env es tvl WT HC.
  induction WT; intros; eauto.
  apply args_empty.
  eapply args_many.
  assumption. eapply heapWArg.
  apply H1. assumption.
  apply H2. assumption.
Qed.  

Lemma heapWF :
  forall D F S H H' env m e t,
    @well_typed D F S H env m e t ->
    @heap_consistent D H' H ->
    @well_typed D F S H' env m e t.
Proof.
  intros D F S H H' env m e t WT HC.
  induction WT; intros; eauto.
  apply TyLit.
  assumption.
  unfold heap_consistent in HC.
  inv H1. econstructor. apply H2.
  apply HC. assumption.
  eapply TyCall.
  apply H0.
  eapply heapWArgs.
  apply H1. assumption. apply H2. apply H3.
Qed.  

Hint Resolve heapWF : Preservation.

Lemma length_nth : forall {A} (l : list A) (k : nat),
    0 <= Z.of_nat(k) < Z.of_nat(length l) -> exists n, nth_error l k = Some n.
Proof.
  intros A l; induction l; intros k Hyp; simpl in *.
  - lia.
  - destruct k; simpl.
    + exists a; eauto.
    + assert (H: 0 <= Z.of_nat(k) < Z.of_nat(S k)). {split.
      *lia. 
      *zify. lia. }
     destruct H. assert (H2: Z.of_nat(k) < Z.of_nat (length l)). {zify. lia. }
     assert (H3: 0 <= Z.of_nat(k) < Z.of_nat (length l)). {split; assumption. }
     apply (IHl k H3).
Qed.      

Lemma nth_length : forall {A} (l : list A) (k : nat) n,
    nth_error l k = Some n -> 0 <= Z.of_nat(k) < Z.of_nat(length l).
Proof.
  intros A l; induction l; intros k n Hyp; simpl in *.
  - apply nth_error_In in Hyp; inv Hyp.
  - destruct k; simpl in *.
    +zify. lia.
    + edestruct IHl; eauto. zify.
      lia.
Qed.

Require Import Coq.Program.Equality.
  
Lemma heap_wf_maps_nonzero : forall D H n v, heap_wf D H -> Heap.MapsTo n v H -> n <> 0.
Proof.
  intros D H n v Hwf HMap.
  destruct (Hwf n) as [ _ HIn ]. 
  destruct n; eauto.
    -exfalso. destruct HIn; try eexists; eauto; 
     inversion H0.
    -zify. lia.
    -zify. lia.
Qed.

Lemma cardinal_not_in :
  forall D H, heap_wf D H -> ~ Heap.In (Z.of_nat(Heap.cardinal H) + 1) H.
Proof.
  intros D H Hwf Contra.
  destruct (Hwf (Z.of_nat(Heap.cardinal H) + 1)) as [H1 H2].
  specialize (H2 Contra).
  lia.
Qed.


Lemma well_typed_preserved : forall D H t, heap_wf D H ->
  @heap_consistent D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, t) H) H.
Proof.
  intros D H t0 Hwf n t HT.
  induction HT using well_typed_lit_ind'; pose proof (cardinal_not_in D H Hwf); eauto.
  eapply TyLitC; eauto.
  intros k HK.  
  destruct (H1 k HK) as [n' [t' [HNth [HMap HWT]]]].
  exists n'. exists t'.
  repeat split; eauto.
  + apply Heap.add_2; eauto.
    destruct (Hwf (n+k)) as [ _ HIn ].
    destruct HIn; try eexists; eauto.
    lia.
  + inv HWT; eauto.
Qed.


  
Lemma heap_add_preserves_wf : forall D H n v, heap_wf D H ->
  heap_wf D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (n, v) H).
Proof.
  intros D H n v Hwf.
  split; intros; simpl; eauto.
  * rewrite cardinal_plus_one in H0.
    - assert (Hyp: 0 < addr <= Z.of_nat(Heap.cardinal H) \/ addr = Z.of_nat(Heap.cardinal H) + 1). {zify. lia. } 
      inv Hyp.
      + destruct (Hwf addr) as [ HIn _ ].
        specialize (HIn H1).
        inv HIn. exists x.
        apply Heap.add_2; eauto.
        lia.
      + eexists; eapply Heap.add_1; eauto.
    - intros Contra.
      destruct (Hwf (Z.of_nat(Heap.cardinal H) + 1)) as [? ?].
      specialize (H2 Contra).
      lia.
  * apply HeapFacts.add_in_iff in H0.
    inv H0.
    - rewrite cardinal_plus_one; try (zify; lia).
      intro Contra.
      destruct (Hwf (Z.of_nat(Heap.cardinal H) + 1)) as [? ?].
      specialize (H1 Contra).
      lia.
    - rewrite cardinal_plus_one.
      + destruct (Hwf addr) as [_ H2]; specialize (H2 H1); zify; lia.
      + intro Contra.
        destruct (Hwf (Z.of_nat(Heap.cardinal H) + 1)) as [H2 H3].
        specialize (H3 Contra).
        lia.
Qed.

Lemma backwards_consistency :
  forall D H' H v,
    @heap_consistent D H' (Heap.add (Z.of_nat(Heap.cardinal H) + 1) v H) ->
    heap_wf D H ->
    @heap_consistent D H' H.
Proof.
  intros D H' H v HC Hwf.
  intros n t HWT.
  eapply HC; eauto.
  induction HWT using well_typed_lit_ind'; pose proof (cardinal_not_in D H Hwf); eauto.
  eapply TyLitC; eauto.
  intros k HK.
  destruct (H1 k HK) as [n' [t' [HN [HM HW]]]].
  exists n'. exists t'.
  repeat split; eauto.
  - apply Heap.add_2; eauto.
    intro Contra.
    destruct (Hwf (n + k)) as [ _ Hyp ].
    destruct Hyp; [eexists; eauto | lia].
  - inv HW; eauto.
Qed.
      
Lemma fold_preserves_consistency : forall l D H ptr, heap_wf D H ->
  let (_, H') :=
      fold_left
        (fun (acc : Z * heap) (t : type) =>
           let (sizeAcc, heapAcc) := acc in
           (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
        l
        (Z.of_nat(Heap.cardinal H), H) in
  Some ((Z.of_nat(Heap.cardinal H) + 1), H') = Some (ptr, H') ->
  @heap_consistent D H' H.
Proof.
  intro l; induction l; intros; simpl; eauto.
  assert (Hwf : heap_wf D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H))
    by (apply heap_add_preserves_wf; auto).
  specialize (IHl D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H) (ptr + 1) Hwf).
  remember (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H) as H1.

  
  Set Printing All.
  remember ((fun (acc : prod Z heap) (t : type) =>
             match acc return (prod Z heap) with
             | pair sizeAcc heapAcc =>
                 @pair Z (Heap.t (prod Z type)) (sizeAcc + 1)
                   (@Heap.add (prod Z type) (sizeAcc + 1) 
                      (@pair Z type 0 t) heapAcc)
             end)) as fold_fun.
  Unset Printing All.
  clear Heqfold_fun. 
  assert (Z.of_nat(Heap.cardinal H1) = (Z.of_nat(Heap.cardinal H) + 1)).
  {
    subst; apply cardinal_plus_one; eauto.
    intro Contra. 
    destruct (H0 (Z.of_nat(Heap.cardinal H) + 1)) as [H1 H2].
    specialize (H2 Contra).
    lia.
  } 
  rewrite H2 in IHl.

  assert (HEq:
      (  fold_left fold_fun l
            (@pair Z heap (Z.of_nat(Heap.cardinal H) + 1) H1) ) =
      (    @fold_left (prod Z heap) type fold_fun l
                      (@pair Z (Heap.t (prod Z type)) (Z.of_nat(Heap.cardinal H) + 1) H1))
    ). {zify. eauto. }


  rewrite HEq in IHl.


  match goal with
  | |- (match ?X with _ => _ end) => destruct X
  end.
  intro Hyp.
  inv Hyp.
   
  assert (Z.of_nat(Heap.cardinal H) + 1 + 1 = Z.of_nat((Heap.cardinal H + 1)) + 1) by (zify; lia).
  rewrite H1 in IHl.

  specialize (IHl eq_refl).


  eapply backwards_consistency; eauto.
Qed.


  
(* This could probably be merged with the previous one *)
Lemma fold_summary : forall l D H ptr,
  heap_wf D H ->
  let (_, H') :=
      fold_left
        (fun (acc : Z * heap) (t : type) =>
           let (sizeAcc, heapAcc) := acc in
           (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
        l
        (Z.of_nat(Heap.cardinal  H), H) in
  Some (Z.of_nat(Heap.cardinal  H)+ 1, H') = Some (ptr, H') ->
  heap_wf D H' /\
  ptr = Z.of_nat(Heap.cardinal  H) + 1 /\
  (Heap.cardinal  H') = ((Heap.cardinal H) + length l)%nat /\
  (forall (k : nat) v,
      (0 <= k < (length l))%nat -> nth_error l k = Some v ->
               Heap.MapsTo (Z.of_nat(Heap.cardinal  H) + 1 + Z.of_nat(k)) (0,v) H') /\
  forall x v, Heap.MapsTo x v H -> Heap.MapsTo x v H'.                                               
Proof.
  intro l; induction l; simpl; intros D H ptr Hwf.
  - intros Eq. inv Eq; repeat (split; eauto).
    intros k v Contra _.
    inv Contra.
    inv H1.
  - remember 
      (fun (acc : prod Z heap) (t : type) =>
         match acc return (prod Z heap) with
         | pair sizeAcc heapAcc =>
           @pair Z (Heap.t (prod Z type)) (sizeAcc + 1)
                 (@Heap.add (prod Z type) (sizeAcc + 1)
                            (@pair Z type 0 t) heapAcc)
         end) as fold_fun.
    clear Heqfold_fun.

    assert (Hwf' : heap_wf D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H))
      by (apply heap_add_preserves_wf; eauto).
    specialize (IHl D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H) (ptr + 1) Hwf').

    
    remember (Heap.add (Z.of_nat(Heap.cardinal H) +1) (0, a) H) as H1.

    assert (Z.of_nat(Heap.cardinal H1) = Z.of_nat(Heap.cardinal H) + 1).
    {
      subst; apply cardinal_plus_one; eauto.
      intro Contra.
      destruct (Hwf (Z.of_nat(Heap.cardinal H) + 1)) as [H1 H2].
      specialize (H2 Contra).
      lia.
    } 
    rewrite H0 in IHl.

    assert (HEq:
        (  @fold_left (prod Z heap) type fold_fun l
              (@pair Z heap ((Z.of_nat(@Heap.cardinal (prod Z type) H)) + 1) H1) ) =
        (    @fold_left (prod Z heap) type fold_fun l
                        (@pair Z (Heap.t (prod Z type)) (Z.of_nat(@Heap.cardinal (prod Z type) H) + 1) H1))
      ) by auto.
   
    rewrite HEq in IHl.

  Set Printing All.

  remember (
    @fold_left (prod Z heap) type fold_fun l
               (@pair Z (Heap.t (prod Z type)) ( Z.of_nat(@Heap.cardinal (prod Z type) H) + 1) H1)
    ) as fold_call.

  Unset Printing All.

  clear Heqfold_call.
  destruct fold_call.
  intro Hyp.
  inv Hyp.

  assert (Z.of_nat(Heap.cardinal H) + 1 + 1 = ((Z.of_nat(Heap.cardinal H)) + 1) + 1) by lia.
  (*rewrite H1 in IHl.*)
  destruct (IHl eq_refl) as [hwf [Card [Card' [HField HMap]]]].

  repeat (split; eauto).
  + lia.
  + intros k v Hk HF.
    destruct k.
    * simpl in *.
      inv HF.
      specialize (HMap (Z.of_nat(Heap.cardinal H) + 1) (0,v)).
      rewrite Z.add_0_r.
      eapply HMap.
      apply Heap.add_1; eauto.
    * simpl in *.
      assert (HS: (Z.of_nat(Heap.cardinal H) + 1 + Z.pos (Pos.of_succ_nat k)) = (Z.of_nat(Heap.cardinal H) + 1 + 1 + Z.of_nat(k))). {
      zify. lia. }
      rewrite HS.
      apply HField; eauto.
      lia.
  + intros x v HM.
    eapply HMap.
    apply Heap.add_2; eauto.
    intro Contra.
    destruct (Hwf x) as [_ Contra'].
    destruct Contra'; [eexists; eauto | ].
    lia.
Qed.

Print length_nth.

Lemma Zlength_nth : forall {A} (l : list A) (z : Z),
0 <= z < Z.of_nat(length l) -> exists n, nth_error l (Z.to_nat z) = Some n.
Proof.
intros. destruct z.
  -apply (length_nth l (Z.to_nat 0) H).
  -assert (H1: Z.of_nat (Z.to_nat (Z.pos p)) = (Z.pos p)).
    {destruct (Z.pos p) eqn:P; inv P.
      +simpl. rewrite positive_nat_Z. reflexivity. }
   rewrite <- H1 in H. apply (length_nth l (Z.to_nat (Z.pos p)) H).
  -exfalso. inv H. apply H0. simpl. reflexivity.
Qed.


(* allocation preservation. *)
Lemma alloc_correct : forall w D F S env H ptr H',
    simple_type w ->
    allocate D H w = Some (ptr, H') ->
    structdef_wf D ->
    heap_wf D H ->
    @heap_consistent D H' H /\
    @well_typed D F S H' env Checked (ELit ptr (TPtr Checked w)) (TPtr Checked w) /\
    heap_wf D H'.
Proof.
  intros w D F S env H ptr H' Wb Alloc HSd HWf.
  unfold allocate in *.
  unfold allocate_meta in *.
  unfold bind in *; simpl in *.
  destruct w; simpl in *; eauto; inv Alloc; simpl in *; eauto.
  - split; [| split].
    * apply well_typed_preserved; eauto.
    * apply TyLit; eauto.
      apply well_type_bound_in_ptr. apply well_type_bound_in_nat.
      eapply WTStack. apply cast_type_bound_ptr. apply cast_type_bound_nat.
      eapply TyLitC; simpl; eauto.
      intros k HK.
      simpl in HK.
      assert (k = 0) by lia; subst; clear HK.
      exists 0. exists TNat.
      repeat split; eauto.
      apply Heap.add_1; eauto. lia.
    * apply heap_add_preserves_wf; auto.
  - split; [ | split].
    * apply well_typed_preserved; eauto.
    * apply TyLit; eauto.
      apply (simple_type_well_bound env) in Wb.
      apply well_type_bound_in_ptr. assumption.
      eapply WTStack. apply cast_type_bound_ptr.
      apply (simple_type_means_cast_same). assumption.
      eapply TyLitC; simpl; eauto.
      intros k HK.
      simpl in HK.
      assert (k = 0) by lia; subst; clear HK.
      exists 0. exists (TPtr m w).
      repeat split; eauto.
      apply Heap.add_1; eauto. lia.
    * apply heap_add_preserves_wf; auto.
  - split.

    *unfold allocate in H1.
      unfold allocate_meta_no_bounds, allocate_meta in H1.
      destruct (StructDef.find s D) eqn:Find; simpl in *; try congruence.

      remember (Fields.elements f) as l.

      pose proof (fold_preserves_consistency (map snd l) D H ptr HWf).
      
      remember (fold_left
            (fun (acc : Z * heap) (t : type) =>
             let (sizeAcc, heapAcc) := acc in (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
            (map snd l) (Z.of_nat(Heap.cardinal H), H)) as p.
      
      destruct p.
      clear Heqp.      
      inv H1.
      eauto.
    
    * unfold allocate_meta_no_bounds, allocate_meta in H1.

      simpl in *.
      destruct (StructDef.find s D) eqn:Find; try congruence.

      pose proof (fold_summary (map snd (Fields.elements f)) D H ptr HWf) as Hyp.

      remember
        (fold_left
           (fun (acc : Z * heap) (t : type) =>
            let (sizeAcc, heapAcc) := acc in
            (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
           (map snd (Fields.elements (elt:=type) f))
           (Z.of_nat(Heap.cardinal H), H)) as p.
      destruct p as [z h].
      clear Heqp.
      inv H1.

      destruct Hyp as [H'wf  [Card1 [Card2 [HF HM]]]]; eauto.

      split; auto.
      constructor.
      apply (simple_type_well_bound env) in Wb.
      apply well_type_bound_in_ptr. assumption.
      eapply WTStack. apply cast_type_bound_ptr.
      apply cast_type_bound_struct.
      eapply TyLitC; simpl in *; eauto; [ rewrite Find | ]; eauto.
      intros k HK.
      apply StructDef.find_2 in Find.
      remember Find as Fwf; clear HeqFwf.
      apply HSd in Fwf.

      assert (HOrd: 0 < Z.of_nat(Heap.cardinal H) + 1 + k <= Z.of_nat(Heap.cardinal H')) by lia.
      pose proof (H'wf (Z.of_nat(Heap.cardinal H) + 1 + k)) as Hyp.
      apply Hyp in HOrd.
      destruct HOrd as [[n' t'] HM'].
      (*This bit is very annoying, quite a bit of converting back and forth
        between ints and nats. This could definately be more automated DP*)
      exists n'. exists t'.
      rewrite Z.sub_0_r in *.
      destruct (Zlength_nth (map snd (Fields.elements f)) k HK) as [x Hnth].
      assert (HK': (0 <= (Z.to_nat k) < (length (map snd (Fields.elements (elt:=type) f))))%nat). {
        destruct k.
          +zify. simpl. lia.
          +simpl. zify. lia.
          +exfalso. inv HK. apply H0. simpl. reflexivity. }
      specialize (HF (Z.to_nat k) x HK' Hnth).
      assert (K0 : k = Z.of_nat (Z.to_nat k)). {
      destruct k.
        +simpl. reflexivity.
        +simpl. zify. reflexivity.
        +inv HK. exfalso. apply H0. simpl. reflexivity. }
      rewrite <- K0 in HF.
      pose proof (HeapFacts.MapsTo_fun HM' HF) as Eq.
      inv Eq.
      repeat (split; eauto).
  - split.
    * destruct b. destruct b0.

      remember (Zreplicate (z0 - z) w) as l.
      pose proof (fold_preserves_consistency l D H ptr HWf) as H0.

      remember (fold_left
         (fun (acc : Z * heap) (t : type) =>
          let (sizeAcc, heapAcc) := acc in
          (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
         l
         (Z.of_nat (Heap.cardinal (elt:=Z * type) H), H)) as p.
      
      destruct p as (n1, h). (*n0 already used???*)
      clear Heqp.
      destruct z; inv H1.
      apply H0; eauto.
      inv Wb. inv Wb.
    * destruct b. destruct b0.

      remember (Zreplicate (z0 - z) w) as l.

      pose proof (fold_summary l D H ptr HWf) as Hyp.
      remember
        (fold_left
          (fun (acc : Z * heap) (t : type) =>
           let (sizeAcc, heapAcc) := acc in
           (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc)) l
          (Z.of_nat (Heap.cardinal (elt:=Z * type) H), H)) as p.
      destruct p.
      clear Heqp.
      inv H1.

      destruct z; inv H2; eauto.
      destruct Hyp as [H'wf  [Card1 [Card2 [HF HM]]]]; eauto.

      
      split; auto.
      constructor.
      apply (simple_type_well_bound env) in Wb.
      apply well_type_bound_in_ptr. assumption.
      eapply WTStack. apply cast_type_bound_ptr.
      apply (simple_type_means_cast_same). assumption.
      eapply TyLitC; simpl in *; eauto.
      intros k HK.
      simpl in *.
      pose proof (H'wf (Z.of_nat(Heap.cardinal H) + 1 + k)) as Hyp.
      rewrite Z.sub_0_r in *.

      remember (Heap.cardinal H ) as c.
      remember (Heap.cardinal H') as c'.
      
      assert (HOrd : 0 < Z.of_nat c + 1 + k <= Z.of_nat c')
        by (zify; lia).
      
      destruct Hyp as [HIn Useless].
      destruct (HIn HOrd) as [[n' t'] HM'].

      destruct HK as [HP1 HP2].

      destruct z0 as [ | p | ?]; simpl in *; [ lia | | lia].
      rewrite replicate_length in *.

      destruct (length_nth (replicate (Pos.to_nat p) w) (Z.to_nat k)) as [t Hnth].
      { rewrite replicate_length ; zify; split; try lia. }
       (* (*This should go through with omega but it doesn't*)
        assert (Hk : Z.of_nat (Z.to_nat k) = k). {
        destruct k; simpl.
          + reflexivity.
          + zify. omega.
          + exfalso. zify. apply HP1. simpl. reflexivity. }
        rewrite Hk. assumption.
      } *)

      rewrite Z.sub_0_r in *.
      
      rewrite Hnth.
      remember Hnth as Hyp; clear HeqHyp.
      apply replicate_nth in Hnth. rewrite Hnth in *; clear Hnth.
        
      exists n'; exists t.
      split; [ reflexivity | ].

      specialize (HF (Z.to_nat k) t).
      assert (HF1 : (0 <= Z.to_nat k < Pos.to_nat p)%nat). {
        split; zify; (try lia).
        (* destruct k; simpl; zify; lia.*)
      }

      specialize (HF HF1 Hyp).

      assert (HId: Z.of_nat (Z.to_nat k) = k). {
        destruct k; simpl.
          + reflexivity.
          + zify. lia.
          + exfalso. zify. lia. }
      rewrite HId in HF.
      
      pose proof (HeapFacts.MapsTo_fun HM' HF) as Eq.
      inv Eq.
      split; auto.
      inv Wb. inv Wb.
  - split.
    * destruct b. destruct b0.

      remember (Zreplicate (z0 - z + 1) w) as l.
      pose proof (fold_preserves_consistency l D H ptr HWf) as H0.

      remember (fold_left
         (fun (acc : Z * heap) (t : type) =>
          let (sizeAcc, heapAcc) := acc in
          (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
         l
         (Z.of_nat (Heap.cardinal (elt:=Z * type) H), H)) as p.
      
      destruct p as (n1, h). (*n0 already used???*)
      clear Heqp.
      destruct z; inv H1.
      apply H0; eauto.
      inv Wb. inv Wb.
    * destruct b. destruct b0.

      remember (Zreplicate (z0 - z + 1) w) as l.

      pose proof (fold_summary l D H ptr HWf) as Hyp.
      remember
        (fold_left
          (fun (acc : Z * heap) (t : type) =>
           let (sizeAcc, heapAcc) := acc in
           (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc)) l
          (Z.of_nat (Heap.cardinal (elt:=Z * type) H), H)) as p.
      destruct p.
      clear Heqp.
      inv H1.

      destruct z; inv H2; eauto.
      destruct Hyp as [H'wf  [Card1 [Card2 [HF HM]]]]; eauto.

      
      split; auto.
      constructor.
      apply (simple_type_well_bound env) in Wb.
      apply well_type_bound_in_ptr. assumption.
      eapply WTStack. apply cast_type_bound_ptr.
      apply (simple_type_means_cast_same). assumption.
      eapply TyLitC; simpl in *; eauto.
      intros k HK.
      simpl in *.
      pose proof (H'wf (Z.of_nat(Heap.cardinal H) + 1 + k)) as Hyp.
      rewrite Z.sub_0_r in *.

      remember (Heap.cardinal H ) as c.
      remember (Heap.cardinal H') as c'.
      
      assert (HOrd : 0 < Z.of_nat c + 1 + k <= Z.of_nat c')
        by (zify; lia).
      
      destruct Hyp as [HIn Useless].
      destruct (HIn HOrd) as [[n' t'] HM'].

      destruct HK as [HP1 HP2].

      destruct (z0+1) as [ | p | ?]; simpl in *; [ lia | | lia].
      rewrite replicate_length in *.

      destruct (length_nth (replicate (Pos.to_nat p) w) (Z.to_nat k)) as [t Hnth].
      { rewrite replicate_length ; zify; split; try lia. }
       (* (*This should go through with omega but it doesn't*)
        assert (Hk : Z.of_nat (Z.to_nat k) = k). {
        destruct k; simpl.
          + reflexivity.
          + zify. omega.
          + exfalso. zify. apply HP1. simpl. reflexivity. }
        rewrite Hk. assumption.
      } *)

      rewrite Z.sub_0_r in *.
      
      rewrite Hnth.
      remember Hnth as Hyp; clear HeqHyp.
      apply replicate_nth in Hnth. rewrite Hnth in *; clear Hnth.
        
      exists n'; exists t.
      split; [ reflexivity | ].

      specialize (HF (Z.to_nat k) t).
      assert (HF1 : (0 <= Z.to_nat k < Pos.to_nat p)%nat). {
        split; zify; (try lia).
        (* destruct k; simpl; zify; lia.*)
      }

      specialize (HF HF1 Hyp).

      assert (HId: Z.of_nat (Z.to_nat k) = k). {
        destruct k; simpl.
          + reflexivity.
          + zify. lia.
          + exfalso. zify. lia. }
      rewrite HId in HF.
      
      pose proof (HeapFacts.MapsTo_fun HM' HF) as Eq.
      inv Eq.
      split; auto.
      inv Wb. inv Wb.
Qed.



Definition env_wt (D : structdef) (env:env) := forall x t, Env.MapsTo x t env
            -> word_type t /\ type_wf D t. 

Lemma subtype_word_type_1 : forall D t t', subtype D t t' -> word_type t -> word_type t'.
Proof.
  intros.
  inv H. assumption.
  1-8:constructor.
Qed.

Lemma get_root_word_type : forall m t t', get_root (TPtr m t) t' -> word_type t -> word_type t'.
Proof.
  intros.
  inv H. assumption. inv H0. inv H0.
Qed.

Lemma get_root_type_wf : forall D m t t', get_root (TPtr m t) t' -> type_wf D t -> type_wf D t'.
Proof.
  intros.
  inv H. assumption. inv H0. assumption.
  inv H0. assumption.
Qed.

Lemma get_root_simple_type : forall m t t', get_root (TPtr m t) t' -> simple_type t -> simple_type t'.
Proof.
  intros.
  inv H. assumption. inv H0. assumption.
  inv H0. assumption.
Qed.



Lemma subtype_type_wf_1 : forall D t t', subtype D t t' -> type_wf D t' -> type_wf D t.
Proof.
  intros.
  inv H. assumption.
  inv H0. inv H4. constructor. assumption.
  inv H0.
  constructor. constructor.
  assumption. assumption.
  inv H0.
  constructor. constructor.
  assumption. assumption.
  inv H0. inv H3.
  constructor. constructor.
  1-2:assumption.
  inv H0. inv H3.
  constructor. constructor.
  assumption. assumption.
  inv H0. inv H3.
  constructor. constructor.
  assumption. assumption.
  constructor. constructor.
  exists fs. assumption.
  constructor. constructor.
  exists fs. assumption.
Qed.

Lemma type_eq_word_type_1 :  forall S t t', type_eq S t t' -> word_type t' -> word_type t.
Proof.
  intros.
  inv H. assumption.
  inv H0. inv H2. constructor.
  inv H2. constructor.
  inv H0. inv H2. constructor.
  inv H2. constructor.
Qed.

Lemma cast_word_type_1 : forall s t t', cast_type_bound s t t' -> word_type t' -> word_type t.
Proof.
  intros.
  induction H0. inv H. constructor.
  inv H. constructor.
Qed.


Lemma cast_type_wf_1 : forall D s t t', cast_type_bound s t t' -> type_wf D t' -> type_wf D t.
Proof.
 intros. generalize dependent t. induction t'.
 intros. inv H. constructor.
 intros. inv H. constructor. apply IHt'. inv H0. assumption.
 assumption.
 intros. inv H. constructor.
 inv H0. destruct H1. exists x. assumption.
 intros. inv H.
 constructor. inv H0. eapply cast_word_type_1. apply H7. assumption.
 apply IHt'. inv H0. assumption. assumption.
 intros. inv H.
 constructor. inv H0. eapply cast_word_type_1. apply H7. assumption.
 apply IHt'. inv H0. assumption. assumption.
Qed.

Lemma type_eq_type_wf : forall D S t t', type_eq S t t' -> type_wf D t' -> type_wf D t.
Proof.
  intros.
  inv H0.
  inv H. constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H. constructor. assumption.
  inv H2.
  constructor.
  eapply cast_type_wf.
  apply H5. assumption.
  inv H2.
  constructor.
  eapply cast_type_wf_1.
  apply H4.
  assumption.
  inv H.
  constructor.
  easy.
  inv H2.
  constructor.
  easy.
  inv H2.
  constructor.
  easy.
  inv H.
  constructor. easy. easy.
  inv H3.
  constructor.
  eapply cast_word_type. apply H9. assumption. 
  eapply cast_type_wf. apply H9. assumption.
  inv H3.
  constructor.
  eapply cast_word_type_1. apply H9. assumption. 
  eapply cast_type_wf_1. apply H9. assumption.
  inv H.
  constructor. assumption. assumption.
  inv H3. constructor.
  eapply cast_word_type. apply H9. assumption. 
  eapply cast_type_wf. apply H9. assumption.
  inv H3. constructor.
  eapply cast_word_type_1. apply H9. assumption. 
  eapply cast_type_wf_1. apply H9. assumption.
Qed.

Lemma type_eq_type_wf_1 : forall D S t t', type_eq S t t' -> type_wf D t -> type_wf D t'.
Proof.
  intros.
  inv H0.
  inv H. constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H. constructor. assumption.
  inv H2.
  constructor.
  eapply cast_type_wf_1.
  apply H4. assumption.
  inv H2.
  constructor.
  eapply cast_type_wf.
  apply H5.
  assumption.
  inv H.
  constructor.
  easy.
  inv H2.
  constructor.
  easy.
  inv H2.
  constructor.
  easy.
  inv H.
  constructor. easy. easy.
  inv H3.
  constructor.
  eapply cast_word_type_1. apply H9. assumption. 
  eapply cast_type_wf_1. apply H9. assumption.
  inv H3.
  constructor.
  eapply cast_word_type. apply H9. assumption. 
  eapply cast_type_wf. apply H9. assumption.
  inv H.
  constructor. assumption. assumption.
  inv H3. constructor.
  eapply cast_word_type_1. apply H9. assumption. 
  eapply cast_type_wf_1. apply H9. assumption.
  inv H3. constructor.
  eapply cast_word_type. apply H9. assumption. 
  eapply cast_type_wf. apply H9. assumption.
Qed.

Lemma meet_type_word_type_1 : forall D s t t1 t2, meet_type D s t t1 t2 -> word_type t -> word_type t2.
Proof.
  intros. inv H0. inv H.
  inv H0. constructor.
  inv H0. inv H2. inv H1. constructor.
  inv H0. constructor.
  inv H0. inv H2. inv H1.
  constructor.
  inv H. inv H0.
  1 - 9: constructor.
  inv H0. inv H2. inv H1.
  constructor.
  inv H1.
  constructor.
  inv H1.
  constructor.
  inv H1.
  constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H1. constructor.
  inv H0. 1 - 9 : constructor.
  inv H0.
  apply ptr_subtype_equiv in H2.
  destruct H2. subst.
  inv H1. constructor.
Qed.

Lemma meet_type_type_wf : forall D s t t1 t2, meet_type D s t t1 t2 
                                -> type_wf D t -> type_wf D t1 -> type_wf D t2.
Proof.
  intros. inv H. assumption.
  assumption.
  assumption.
  assumption.
Qed.

Lemma subtype_well_type : forall D H env t t' n,
@well_typed_lit D H env n t ->
subtype D t t' ->
@well_typed_lit D H env n t'.
Proof.
  intros. induction H0. 
  - inv H1. eauto.
  - assert (exists t, t' = (TPtr Unchecked t)) by (inv H1; eauto).
    destruct H0. rewrite H0. eauto.
  - eauto.
  - specialize (subtype_trans D t t' Checked w H2 H1) as eq1.

    assert (exists t0, t' = (TPtr Checked t0)) by (inv H1; eauto).
    destruct H3. rewrite H3 in *.
    eapply TyLitRec; eauto.
  - assert (exists t0, t' = (TPtr Checked t0)) by (inv H1; eauto).
    unfold allocate_meta in H0.
    induction w.
    * inv H1.
      ++ eapply TyLitC; eauto. 
      ++ inv H7. inv H9. eapply TyLitC; eauto.
      unfold allocate_meta. eauto.
      intros.
      assert (l - h0 <= 0 \/ l - h0 = 1) by lia.
      destruct H5.
      assert ((Zreplicate (l - h0) TNat) = []).
      unfold Zreplicate. 
      destruct (l - h0). easy.
      specialize (Pos2Z.is_pos p) as eq1. contradiction. easy.
      rewrite H8 in H1. simpl in H1. lia.

      rewrite H5 in *.
      unfold Zreplicate in *. simpl in *.
      assert (k = h0) by lia. subst. simpl.
      inv H0. simpl in *.
      destruct (H2 0). lia.
      destruct H0. 
      destruct H0. destruct H8.
      assert (l = 1) by lia.
      assert (h0 = 0) by lia.
      subst.
      exists x. exists x0.
      split. easy. split. easy.
      inv H0. apply TyLitInt.
    * inv H1. 
      ++ eapply TyLitC; eauto.
      ++ inv H7. inv H9. eapply TyLitC; eauto. 
      unfold allocate_meta. eauto.
      intros.
      assert (l - h0 <= 0 \/ l - h0 = 1) by lia.
      destruct H5.
      assert ((Zreplicate (l - h0) (TPtr m w)) = []).
      unfold Zreplicate. 
      destruct (l - h0). easy.
      specialize (Pos2Z.is_pos p) as eq1. contradiction. easy.
      rewrite H8 in H1. simpl in H1. lia.
      rewrite H5 in *.
      unfold Zreplicate in *. simpl in *.
      assert (k = h0) by lia. subst. simpl.
      inv H0. simpl in *.
      destruct (H2 0). lia.
      destruct H0. 
      destruct H0. destruct H8.
      assert (l = 1) by lia.
      assert (h0 = 0) by lia.
      subst.
      exists x. exists x0.
      split. easy. split. easy.
      inv H0.
      destruct (Z.eq_dec x n).
      subst.
      destruct m.
      eapply TyLitRec.
      apply set_add_intro2. reflexivity.
      apply SubTyOne.
      inv H9. apply TyLitU.
      apply TyLitZero.
      eapply (TyLitRec).

    * inv H1. eapply TyLitC; eauto.
     
      eapply TyLitC; eauto.
      unfold allocate_meta; eauto.
      simpl in H0. destruct (StructDef.find (elt:=fields) s D) eqn:Hf.
      + inv H0. rewrite map_length in H2.
        assert (StructDef.MapsTo s f D) by (eapply find_implies_mapsto; eauto).
        assert (f = fs) by (eapply StructDefFacts.MapsTo_fun; eauto). 
        rewrite H1 in *.
        assert (((length (Fields.elements (elt:=type) fs)) >= 1)%nat) by (eapply fields_implies_length; eauto).
        intros. simpl in H5.
        destruct (H2 k). zify. lia.
        exists x. exists TNat.
        assert (k = 0) by (destruct k; inv H5; eauto; exfalso; zify; lia).
        rewrite H9 in *. simpl. split; eauto.
        destruct H7. destruct H7.
        simpl in H7. 
        rewrite <- (element_implies_element s fs D TNat H0 H8) in H7.
        inv H7. destruct H10.
        split. assumption. eauto.
      + inv H0. 
    * clear IHw. inv H0.
    * 
      inv H1. clear H3. 
        + eapply TyLitC; eauto.
        + clear H3.
          eapply TyLitC.


          unfold allocate_meta; eauto.
          intros. 
          assert (Hmin : (h' - l') > 0).
          {
                destruct (h' - l'); zify; (try omega); simpl in *; inv H0;
                exfalso; rewrite Z.add_0_r in *; omega.
          }
          assert (Hpos : exists p, h' - l' = Z.pos p).
          {
           destruct (h' - l'); zify; (try omega).
           exists p; eauto.
          }
          assert ((z0 - z) >= (h' - l')) by omega.
          assert ((length (Zreplicate (z0 - z) w) >= (length (Zreplicate (h' - l') w)))%nat).
          {
            destruct (z0 - z).
            * simpl. destruct (h' - l'); simpl; eauto. exfalso. zify; omega.
            * simpl. rewrite replicate_length. destruct (h' - l');
              simpl; eauto; (try omega). rewrite replicate_length; zify; omega.
            * exfalso; zify; omega.
          }
          destruct (H2 k).
          split. 
            ** omega.
            ** (* relies on the fact that h' - l' must be greater than 0*)
              destruct Hpos as [p Hpos].
              assert (h' > l') by omega.
              assert (psuc : exists n, Pos.to_nat p = S n) by (eapply pos_succ; eauto).
              (*very convoluted*)
              destruct (z0 - z)eqn:Hz.
              ++ exfalso; omega.
              ++ rewrite Hpos in *. simpl in *.
                 rewrite replicate_length in *.
                 assert (Hp : Z.of_nat (Pos.to_nat p) = Z.pos p).
                 {
                  destruct psuc as [n0 psuc]. rewrite psuc.
                  zify; omega.
                 } clear psuc.
                 assert (psuc: exists n, Pos.to_nat p0 = S n) by eapply pos_succ; eauto.
                 assert (Hp0 : Z.of_nat (Pos.to_nat p0) = Z.pos p0).
                 {
                  destruct psuc as [n0 psuc]. rewrite psuc.
                  zify; omega.
                 }
                 rewrite Hp0. rewrite <- Hz. 
                 assert (z + (z0 - z) = z0) by omega.
                 rewrite H5. rewrite Hp in H0.
                 rewrite <- Hpos in H0.
                 assert (l' + (h' - l') = h') by omega.
                 rewrite H6 in H0. omega.
              ++ exfalso; zify; omega.
          ** exists x. exists w.
             split.
             ++ destruct Hpos as [p Hpos]. rewrite Hpos.
                simpl. 
                assert (exists n, Pos.to_nat p = S n) by (eapply pos_succ; eauto).
                destruct H5. rewrite H5. simpl.
                destruct (k - l')eqn:Hk; simpl; eauto.
               -- Search nth_error.
             ++ destruct H4.
                destruct H4 as [? [? ?]].
                rewrite H7 in *. 
                split; eauto. 
                assert (well_typed_lit D H
               (set_add eq_dec_nt (n, TPtr Checked (TArray l' h' w))
               (set_add eq_dec_nt
               (n, TPtr Checked (TArray z z0 w))
                s)) x w) by (eapply scope_weakening; eauto).
                assert (set_equal (set_add eq_dec_nt (n, TPtr Checked (TArray l' h' w))
          (set_add eq_dec_nt (n, TPtr Checked (TArray z z0 w)) s))
              (set_add eq_dec_nt (n, TPtr Checked (TArray z z0 w))
               (set_add eq_dec_nt
               (n, TPtr Checked (TArray l' h' w))
                s))).
                { eapply set_equal_add_add; eauto. instantiate (1:=s). unfold set_equal.
                  intros; split; intros; assumption. } 
                assert (well_typed_lit D H
               (set_add eq_dec_nt (n, TPtr Checked (TArray z z0 w))
               (set_add eq_dec_nt
               (n, TPtr Checked (TArray l' h' w))
                s)) x w). 
               { eapply scope_replacement; eauto. } 
Qed.

(* If a term is typed checked, then its returned expression has a word type. *)
Lemma well_typed_word_type_wf :
   forall D F S H env m e t,
          structdef_wf D ->
          expr_wf D F e -> 
         env_wt D env ->
         fun_typed D F S H ->
         @well_typed D F S H env m e t  -> word_type t /\ type_wf D t.
Proof.
  intros.
  induction H4; eauto.
  inv H1. easy.
  apply H3 in H4.
  destruct H4. destruct H8.
  split.
  apply subtype_word_type_1 in H7. eapply type_eq_word_type_1.
  apply H6. assumption. assumption.
  apply subtype_type_wf in H7.
  eapply type_eq_type_wf. apply H6.
  assumption. assumption.
  split. constructor. constructor.
  inv H1.
  specialize (IHwell_typed1 H6 H2) as eq1.
  assert (env_wt D (Env.add x t1 env0)).
  unfold env_wt in *.
  intros.
  destruct (Nat.eq_dec x0 x).
  subst.
  apply Env.mapsto_add1 in H1.
  subst. assumption.
  apply Env.add_3 in H1.
  specialize (H2 x0 t0 H1) as eq2.
  easy. lia.
  specialize (IHwell_typed2 H8 H1) as eq2. easy.
  split. constructor. constructor.
  inv H1.
  split. constructor. constructor.
  unfold structdef_wf in H0.
  apply H0 in H5.
  unfold fields_wf in H5.
  apply H5 in H6.
  easy.
  inv H1.
  split. constructor. constructor. easy.
  apply IHwell_typed.
  inv H1. assumption. assumption.
  inv H1. easy.
  inv H1.
  easy.
  inv H1.
  split. easy. easy.
  inv H1.
  split. easy.
  constructor. constructor.
  inv H11. inv H8.
  easy.
  inv H11. inv H8. easy.
  inv H1. easy.
  inv H1.
  specialize (IHwell_typed H9 H2).
  destruct H6.
  destruct IHwell_typed.
  destruct H1. subst.
  split. easy.
  assert (type_wf D (TPtr m' t')).
  eapply subtype_type_wf. apply H5.
  assumption. inv H10. assumption.
  destruct H1.
  destruct H1. subst.
  easy.
  destruct H1. subst.
  easy.
  split.
  eapply type_eq_word_type. apply H6.
  assumption.
  inv H1.
  specialize (IHwell_typed1 H10 H2) as eq1.
  destruct eq1. inv H8.
  eapply type_eq_type_wf_1.
  apply H6. assumption. 
  split.
  eapply type_eq_word_type. apply H6.
  assumption.
  inv H1.
  specialize (IHwell_typed1 H11 H2) as eq1.
  destruct eq1. inv H9. inv H13.
  eapply type_eq_type_wf_1.
  apply H6. assumption. 
  split.
  eapply type_eq_word_type. apply H6.
  assumption.
  inv H1.
  specialize (IHwell_typed1 H11 H2) as eq1.
  destruct eq1. inv H9. inv H13.
  eapply type_eq_type_wf_1.
  apply H6. assumption. 
  split. 
  eapply subtype_word_type_1.
  apply H7. assumption.
  eapply subtype_type_wf.
  apply H7. assumption.
  split. 
  eapply subtype_word_type_1.
  apply H7. assumption.
  eapply subtype_type_wf.
  apply H7. assumption.
  inv H1.
  specialize (IHwell_typed1 H11 H2) as eq1.
  specialize (IHwell_typed2 H13 H2) as eq2.
  destruct eq1. destruct eq2.
  split.
  eapply meet_type_word_type_1. apply H7.
  assumption.
  eapply meet_type_type_wf.
  apply H7.
  assumption. assumption.
Qed.

Lemma in_map_snd : forall (l : list (Fields.key*type)) t,
                In t (map snd l) -> (exists x, In (x,t) l).
Proof.
  intros.
  induction l. inv H.
  simpl in *.
  destruct H.
  destruct a. exists k. simpl in H. subst. left. easy.
  apply IHl in H.
  destruct H.
  exists x. right. easy.
Qed.

Axiom field_eq : Equivalence (Fields.eq_key_elt (elt:=type)).

Lemma replicate_in : forall n (w t:type), In t (replicate n w) -> t = w.
Proof.
 induction n.
 simpl. intros. inv H.
 simpl. intros. destruct H. easy.
 apply IHn in H. easy.
Qed.

Lemma allocate_meta_wt : forall D w n tl, 
          structdef_wf D -> type_wf D w -> simple_type w 
            -> allocate_meta D w = Some (n, tl) ->
                      (forall t, In t tl -> word_type t /\ type_wf D t /\ simple_type t).
Proof.
   intros. unfold allocate_meta in H2.
   destruct w. inv H2.
   inv H3.
   split. easy. split. easy. easy.
   inv H2.
   inv H2. inv H3.
   split. easy. split. constructor. inv H0. easy. easy.
   inv H2.
   destruct ((StructDef.find (elt:=fields) s D)) eqn:eq1.
   inv H2.
   apply in_map_snd in H3.
   destruct H3.
   apply (@In_InA (Fields.key*type) (Fields.eq_key_elt (elt:=type))) in H2.
   apply Fields.elements_2 in H2.
   unfold structdef_wf in H.
   apply StructDef.find_2 in eq1.
   apply H in eq1.
   apply eq1 in H2. easy.
   apply field_eq.
   inv H2. inv H1.
   inv H2.
   unfold Zreplicate in H3.
   destruct (h - n). inv H3.
   apply replicate_in in H3.
   subst.
   inv H0. easy.
   inv H3.
   inv H1.
   inv H2.
   unfold Zreplicate in H3.
   destruct (h - n + 1). inv H3.
   apply replicate_in in H3.
   subst.
   inv H0. easy.
   inv H3.
Qed.

Lemma heap_add_preserves_wt : forall D H n v, heap_wt D H ->
  word_type v -> type_wf D v -> simple_type v ->
  heap_wt D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (n, v) H).
Proof.
  intros D H n v WT Twf ST Hwf.
  unfold heap_wt in *.
  intros.
  destruct (Z.eq_dec x (Z.of_nat (Heap.cardinal (elt:=Z * type) H) + 1)).
  subst.
  apply Heap.mapsto_add1 in H0. inv H0.
  easy.
  apply Heap.add_3 in H0. apply WT in H0.
  easy. lia.
Qed.


Lemma allocate_wt_aux : forall l D H ptr, 
   heap_wf D H -> 
   heap_wt D H ->
   (forall t, In t l -> word_type t /\ type_wf D t /\ simple_type t) ->
  let (_, H') :=
      fold_left
        (fun (acc : Z * heap) (t : type) =>
           let (sizeAcc, heapAcc) := acc in
           (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc))
        l
        (Z.of_nat(Heap.cardinal H), H) in
  Some ((Z.of_nat(Heap.cardinal H) + 1), H') = Some (ptr, H') ->
  heap_wt D H'.
Proof.
  intro l; induction l; intros; simpl; eauto.
  assert (Hwt : heap_wt D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H)).
  specialize (H2 a). assert (a = a \/ In a l). left. easy.
  apply H2 in H3.
  apply heap_add_preserves_wt. assumption. 1-3:easy.
  assert (Hwf : heap_wf D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H))
     by (apply heap_add_preserves_wf; eauto).
  assert ((forall t : type,
       In t l -> word_type t /\ type_wf D t /\ simple_type t)).
  intros. simpl in H2.
  assert (a = t \/ In t l). right. assumption. apply H2 in H4. easy.
  specialize (IHl D (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H) (ptr + 1) Hwf Hwt H3).
  remember (Heap.add (Z.of_nat(Heap.cardinal H) + 1) (0, a) H) as H5.

  Set Printing All.
  remember ((fun (acc : prod Z heap) (t : type) =>
             match acc return (prod Z heap) with
             | pair sizeAcc heapAcc =>
                 @pair Z (Heap.t (prod Z type)) (sizeAcc + 1)
                   (@Heap.add (prod Z type) (sizeAcc + 1) 
                      (@pair Z type 0 t) heapAcc)
             end)) as fold_fun.
  Unset Printing All.
  clear Heqfold_fun. 

  assert (Z.of_nat(Heap.cardinal H5) = (Z.of_nat(Heap.cardinal H) + 1)).
  {
    subst; apply cardinal_plus_one; eauto.
    intro Contra. 
    destruct (H0 (Z.of_nat(Heap.cardinal H) + 1)) as [H7 H8].
    specialize (H8 Contra).
    lia.
  } 
  rewrite H4 in IHl.

  assert (HEq:
      (  fold_left fold_fun l
            (@pair Z heap (Z.of_nat(Heap.cardinal H) + 1) H5) ) =
      (    @fold_left (prod Z heap) type fold_fun l
                      (@pair Z (Heap.t (prod Z type)) (Z.of_nat(Heap.cardinal H) + 1) H5))
    ). {zify. eauto. }


  rewrite HEq in IHl.


  match goal with
  | |- (match ?X with _ => _ end) => destruct X
  end.
  intro Hyp.
  inv Hyp.
   
  assert (Z.of_nat(Heap.cardinal H) + 1 + 1 = Z.of_nat((Heap.cardinal H + 1)) + 1) by (zify; lia).
  rewrite H5 in IHl.

  specialize (IHl eq_refl).
  assumption.
Qed.

Lemma allocate_wt : forall D H w n H',    
         heap_wf D H -> 
         heap_wt D H -> 
          structdef_wf D -> type_wf D w -> simple_type w ->
                 allocate D H w = Some (n, H') -> heap_wt D H'.
Proof.
 intros. unfold allocate in H5.
 destruct (allocate_meta D w) eqn:eq1.
 destruct p.
 specialize (allocate_meta_wt D w z l H2 H3 H4 eq1) as eq2.
 destruct z.
 clear eq1.
 Check allocate_wt_aux.
 
 pose proof (allocate_wt_aux l D H n H0 H1 eq2).

 remember (fold_left
         (fun (acc : Z * heap) (t : type) =>
          let (sizeAcc, heapAcc) := acc in
          (sizeAcc + 1, Heap.add (sizeAcc + 1) (0, t) heapAcc)) l
         (Z.of_nat (Heap.cardinal (elt:=Z * type) H), H)) as p.
      
 destruct p.
 clear Heqp.      
 inv H5.
 eauto. inv H5. inv H5. inv H5.
Qed.

Lemma heapWT : forall D F S S' H H' env m e t r,
     heap_wf D H -> 
     structdef_wf D ->
     expr_wf D F e -> 
     env_wt D env ->
     fun_typed D F S H ->
    @well_typed D F S H env m e t ->
     heap_wt D H -> step D F S H e S' H' r -> heap_wt D H'.
Proof.
  intros D F S S' H H' env m e t r Hwf Wsd Wexp Wenv Wfun WT Hwt HS.
  induction HS; eauto.
  unfold heap_wt in *.
  subst.
  intros.
  destruct (Z.eq_dec x n).
  subst.
  apply Heap.mapsto_add1 in H5.
  inv H5.
  inv WT.
  inv Wexp.
  specialize (well_typed_word_type_wf D F s H env m 
               (ELit n t0) (TPtr m' t2) Wsd H11 Wenv Wfun H10) as eq1.
  inv H10. 
  inv H1.
  assert (word_type t').
  eapply cast_word_type. apply H14. assumption.
  assert (type_wf D t').
  eapply cast_type_wf.
  apply H14.
  destruct eq1. inv H6. assumption.
  assert (simple_type t').
  apply cast_means_simple_type in H14. assumption.
  split. eapply get_root_word_type. apply H4. assumption.
  split. eapply get_root_type_wf. apply H4. assumption.
  eapply get_root_simple_type. apply H4. assumption.
  inv Wexp.
  specialize (well_typed_word_type_wf D F s H env m 
               (ELit n t0) (TPtr m' (TArray l h t2)) Wsd H12 Wenv Wfun H11) as eq1.
  inv H11. 
  inv H1. inv H15.
  assert (word_type t'1).
  eapply cast_word_type. apply H21. assumption.
  assert (type_wf D t'1).
  eapply cast_type_wf.
  apply H21.
  destruct eq1. inv H6. inv H17. assumption.
  assert (simple_type t'1).
  apply cast_means_simple_type in H21. assumption.
  split. inv H4. inv H23. assumption.
  split. inv H4. inv H23. assumption.
  inv H4. inv H23. assumption.
  inv Wexp.
  specialize (well_typed_word_type_wf D F s H env m 
               (ELit n t0) (TPtr m' (TNTArray l h t2)) Wsd H12 Wenv Wfun H11) as eq1.
  inv H11. 
  inv H1. inv H15.
  assert (word_type t'1).
  eapply cast_word_type. apply H21. assumption.
  assert (type_wf D t'1).
  eapply cast_type_wf.
  apply H21.
  destruct eq1. inv H6. inv H17. assumption.
  assert (simple_type t'1).
  apply cast_means_simple_type in H21. assumption.
  split. inv H4. inv H23. assumption.
  split. inv H4. inv H23. assumption.
  inv H4. inv H23. assumption.
  apply Heap.add_3 in H5.
  apply Hwt in H5. easy. lia.
  inv Wexp.
  assert (type_wf D w'). 
  eapply cast_type_wf. apply H0. assumption.
  assert (simple_type w').
  eapply cast_means_simple_type. apply H0. 
  apply (allocate_wt D H w' n1 H' Hwf Hwt Wsd H3 H5 H2).
Qed.  

Hint Resolve heapWT : Preservation.



Ltac maps_to_fun :=
  match goal with
  | [ H1 : Heap.MapsTo ?X (?V1, ?T1) ?H 
    , H2 : Heap.MapsTo ?X (?V2, ?T2) ?H
      |- _ ] =>
    let H := fresh "Eq" in     
    assert (H : (V1,T1) = (V2, T2)) by (eapply HeapFacts.MapsTo_fun; eauto);
    inv H
  | _ => idtac
  end.

Ltac solve_map :=
  match goal with
  | [ |- Heap.MapsTo ?x ?T (Heap.add ?x ?T _) ] => apply Heap.add_1; auto
  | _ => idtac
  end.



Lemma HeapUpd:
  Suppose H(i) = n^T and G |- n'^T' : T' under heap H.
  If H' = H[i |--> k^T] and G |- k^T : T under H' then G |- n'^T' under heap H'
  (In short: H' |- H)
Proof.
  The proof is by induction on G |- n'^T' : T' under H.
  Case T-Int and T-VConst apply as before
  Case T-PtrC
    G |- n'^(ptr^c W) under H
    where
      types(D,W) = T0,...,T(j-1)
      G,n'^(ptr^c W) |-m H(n'+x) : Tx for 0 <= x < j under H
    We want to prove
      G,n'^(ptr^c W) |-m H'(n'+x) : Tx for 0 <= x < j under H'
    Two cases
      n'+x == i: So H'(i) = k^T and we are given G |- k^T under H'. Follows by weakening
      n'+x != i. So H'(i) = H(i) and the result follows by induction.


Definition set_equal (s1 s2 : scope) :=
  forall x, set_In x s1 <-> set_In x s2.

Lemma set_equal_add (s1 s2 : scope) (v : Z * type) :
  set_equal s1 s2 -> 
  set_equal (set_add eq_dec_nt v s1) (set_add eq_dec_nt v s2).
Proof.  
  intros Eq x.
  split; intros.
  - destruct (eq_dec_nt x v).
    + subst; apply set_add_intro2; auto.
    + apply set_add_intro1; auto.
      apply set_add_elim2 in H; eauto.
      apply Eq; auto.
  - destruct (eq_dec_nt x v).
    + subst; apply set_add_intro2; auto.
    + apply set_add_intro1; auto.
      apply set_add_elim2 in H; eauto.
      apply Eq; auto.
Qed.      

Lemma scope_replacement :
  forall D H s n t,
    @well_typed_lit D H s n t ->
  (forall s', 
    set_equal s s' ->
    @well_typed_lit D H s' n t).
Proof.
  intros D H ss n t HWT.
  induction HWT using well_typed_lit_ind'; eauto.
  - (* Replacement, TyRec *)
    intros s' HEq.
    econstructor; eauto; eapply HEq; eauto.
  - (* Replacement, TyLitC *)
    intros s' Heq.
    eapply TyLitC; eauto.
    intros k Hk.
    destruct (H1 k Hk) as [n' [t' [HNth [HMap [HWt1 HRepl]]]]].
    exists n'. exists t'.
    repeat (split; eauto).
    eapply HRepl; eauto.
    apply set_equal_add; auto.
Qed.

Lemma set_equal_add_add (s1 s2 : scope) (v1 v2 : Z * type) :
  set_equal s1 s2 -> 
  set_equal (set_add eq_dec_nt v1 (set_add eq_dec_nt v2 s1))
            (set_add eq_dec_nt v2 (set_add eq_dec_nt v1 s1)).
Proof.  
  intros Eq x.
  split; intros;
    destruct (eq_dec_nt x v1); destruct (eq_dec_nt x v2); subst;
      try solve [apply set_add_intro2; auto];
      try solve [apply set_add_intro1; auto;
                 apply set_add_intro2; auto];
    (do 2 (apply set_add_intro1; auto);
     do 2 (apply set_add_elim2 in H; auto)).
Qed.

Lemma set_equal_refl (s : scope) : set_equal s s.
  intros x; split; auto.
Qed.

Lemma scope_weakening :
  forall D H s n t,
    @well_typed_lit D H s n t ->
  forall x,
    @well_typed_lit D H (set_add eq_dec_nt x s) n t.
Proof.
  intros D H ss n t HWT.
  induction HWT using well_typed_lit_ind'; eauto.
  - (* Weakening, TyRec *)
    intros x.
    econstructor.
    apply set_add_intro1; eauto.
  - (* Weakening, TyLitC *)
    intros x.
    eapply TyLitC; eauto.
    intros k Hk.
    destruct (H1 k Hk) as [n' [t' [HNth [HMap [HWt1 HWeak]]]]].
    exists n'. exists t'.
    repeat (split; eauto).
    eapply scope_replacement; [eapply HWeak; eauto |].
    eapply set_equal_add_add; eauto.
    eapply set_equal_refl; eauto.
Qed.

Lemma set_equal_add_cons :
  forall x y s,
      set_equal (x :: set_add eq_dec_nt y s)
                (set_add eq_dec_nt y (x :: s)).
Proof.
  intros x y s z; split; intros H;
  destruct (eq_dec_nt z y); destruct (eq_dec_nt z x);
    subst; try congruence.
  - apply set_add_intro2; auto.
  - apply set_add_intro2; auto.
  - apply set_add_intro1; left; auto.
  - inv H; try congruence.
    apply set_add_elim in H0.
    inv H0; try congruence.
    apply set_add_intro1; auto.
    right; auto.
  - left; auto. 
  - right; apply set_add_intro2; auto.
  - left; auto.
  - apply set_add_elim in H.
    inv H; try congruence.
    inv H0; try congruence.
    right; apply set_add_intro1; auto.
Qed.

Lemma scope_weakening_cons :
  forall D H n t s,
    @well_typed_lit D H s n t ->
  forall x, @well_typed_lit D H (x :: s) n t.
Proof.
  intros D H n t s HWT.
  induction HWT using well_typed_lit_ind'; eauto; intros x.
  - econstructor.
    right; eauto.
  - eapply TyLitC; eauto.
    intros k Hk.
    destruct (H1 k Hk) as [n' [t' [HNth [HMap [HWt1 HWeak]]]]].
    exists n'. exists t'.
    repeat (split; eauto).
    eapply scope_replacement; [eapply (HWeak x); eauto |].
    apply set_equal_add_cons.
Qed.

Corollary scope_weakening' :
  forall D H n t,
    @well_typed_lit D H empty_scope n t ->
  forall s, @well_typed_lit D H s n t.
Proof.  
  intros D H n t HWT s.
  induction s; auto.
  apply scope_weakening_cons; auto.
Qed.  
  
  (*
Lemma scope_wf_heap_consistent_weakening :
  forall s D H x v T v',
    Heap.MapsTo x (v,T) H ->
    scope_wf D H s -> scope_wf D (Heap.add x (v',T) H) s.
Proof.
  intros s D H x v T v' HMap HSwf.
  intros x' t' HS.
  destruct (HSwf x' t'); eauto.
  destruct (Nat.eq_dec x x').
  - subst; maps_to_fun.
    exists v'.
    eapply Heap.add_1; eauto.
  - exists x0.
    eapply Heap.add_2; eauto.
Qed.

Hint Resolve scope_wf_heap_consistent_weakening.
 *)
     
Lemma HeapUpd : forall D i n T H k,
  Heap.MapsTo i (n,T) H ->
  @well_typed_lit D (Heap.add i (k,T) H) empty_scope k T ->
  @heap_consistent D (Heap.add i (k,T) H) H.
Proof.
  intros D i n T H k HMap Hwtk n' t' HWT.
  induction HWT using well_typed_lit_ind'; eauto.
  (* T-PtrC *)
  eapply TyLitC; eauto.
  intros x Hx.
  destruct (H1 x Hx) as [n' [t' [HNth [HMap' [HWt1 HWt2]]]]].
  destruct (Z.eq_dec (n0+x) i).
  - exists k. exists t'.
    subst. maps_to_fun.
    repeat (split; eauto).
    + apply Heap.add_1; eauto.
    + apply scope_weakening; eauto.
  - exists n'. exists t'.
    repeat (split; eauto).
      + apply Heap.add_2; eauto.
      + eapply HWt2.
        eapply scope_weakening; eauto.
Qed.

Hint Constructors value.

Lemma types_are_not_infinite :
  forall w, TPtr Checked w = w -> False.
Proof.
  induction w; intros; try congruence.
Qed.

(* Custom remove to avoid NoDup? *)
Fixpoint set_remove_all v (x : scope) := 
    match x with
    | nil => empty_scope
    | v' :: vs => if eq_dec_nt v v' then
                    set_remove_all v vs
                  else
                    v' :: set_remove_all v vs
    end.

Lemma set_remove_all_intro : forall a b l,
    set_In a l -> a <> b -> set_In a (set_remove_all b l).
Proof.
  intros a b l.
  induction l; intros; simpl.
  - inv H.
  - destruct (eq_dec_nt b a0).
    + subst.
      inv H; try congruence.
      eapply IHl; eauto.
    + destruct (eq_dec_nt a a0).
      * subst; left; auto.
      * inv H; try congruence.
        simpl.
        right.
        eauto.
Qed.

Lemma set_remove_all_elim1:
  forall a b l, set_In a (set_remove_all b l) -> a <> b.
Proof.  
  intros; induction l.
  - inv H.
  - intro Contra; subst.
    simpl in H.
    destruct (eq_dec_nt b a0).
    + subst.
      apply IHl; eauto.
    + simpl in *.
      inv H; try congruence.
      eapply IHl; eauto.
Qed.

Lemma set_remove_all_elim2:
  forall a b l, set_In a (set_remove_all b l) -> set_In a l.
Proof.
  intros; induction l.
  - inv H.
  - simpl in H.
    destruct (eq_dec_nt b a0).
    + subst.
      right; apply IHl; eauto.
    + simpl in *.
      inv H.
      * left; auto.
      * right; eapply IHl; eauto.
Qed.
  
Lemma set_equal_add_remove (s : scope) (v1 v2 : Z * type) :
  v1 <> v2 ->
  set_equal (set_add eq_dec_nt v1 (set_remove_all v2 s))
            (set_remove_all v2 (set_add eq_dec_nt v1 s)).
Proof.
  intros H x.
  split; intro In.
  * destruct (eq_dec_nt x v1); destruct (eq_dec_nt x v2); try congruence; subst;
      unfold not in *.
    - apply set_remove_all_intro; eauto.
      apply set_add_intro2; auto.
    - apply set_add_elim in In; destruct In; try congruence.
      eapply set_remove_all_elim1 in H0.
      congruence.
    - apply set_remove_all_intro; eauto.
      apply set_add_elim in In; destruct In; try congruence.
      apply set_remove_all_elim2 in H0.
      apply set_add_intro1; auto.
  * destruct (eq_dec_nt x v1); destruct (eq_dec_nt x v2); try congruence; subst.
    - apply set_add_intro2; auto.
    - apply set_remove_all_elim1 in In.
      try congruence.
    - apply set_remove_all_elim2 in In.
      apply set_add_elim in In.
      inv In; try congruence.
      apply set_add_intro1; auto.
      apply set_remove_all_intro; eauto.
Qed.      

Lemma set_remove_add :
  forall x s, set_equal (set_remove_all x (set_add eq_dec_nt x s)) (set_remove_all x s).
Proof.
  intros x s y; split; intros H; destruct (eq_dec_nt x y); subst; eauto.
  - apply set_remove_all_elim1 in H; congruence.
  - apply set_remove_all_elim2 in H.
    apply set_add_elim in H.
    inv H; try congruence.
    apply set_remove_all_intro; auto.
  - apply set_remove_all_elim1 in H; congruence.
  - apply set_remove_all_intro; auto.
    apply set_remove_all_elim2 in H.
    apply set_add_intro1; auto.
Qed.

Lemma set_equal_symmetry : forall (s1 s2 : scope),
    set_equal s1 s2 -> set_equal s2 s1.
Proof.  
  intros s1 s2 Eq x; split; intro H;
  apply Eq; auto.
Qed.  
  
Lemma scope_swap :
  forall D H x y s N T,
    @well_typed_lit D H (set_remove_all x (set_add eq_dec_nt y s)) N T ->
    @well_typed_lit D H (set_add eq_dec_nt y (set_remove_all x s)) N T.
Proof.
  intros D H x y s N T HWT.
  destruct (eq_dec_nt x y).
  - subst.
    pose proof (set_remove_add y s).
    apply scope_replacement with (s' := set_remove_all y s) in HWT; auto.
    apply scope_weakening; auto.
  - assert (Neq: y <> x) by auto.
    pose proof (set_equal_add_remove s y x Neq) as Hyp.
    eapply scope_replacement.
    + eapply HWT.
    + apply set_equal_symmetry.
      auto.
Qed.




Lemma scope_strengthening :
  forall D H n tn s,
    @well_typed_lit D H s n tn ->
    heap_wf D H ->
    forall m tm,
      @well_typed_lit D H empty_scope m tm ->
      @well_typed_lit D H (set_remove_all (m, tm) s) n tn.
Proof.
  intros D H n' t s HWT.
  remember HWT as Backup; clear HeqBackup.
  induction HWT using well_typed_lit_ind';
  (* intros HHwf m HMap HSetIn HWT; eauto. *)
    intros HHwf m tm Hwt; eauto.
  - destruct (Z.eq_dec n m).
    + subst.
      destruct (type_eq_dec tm (TPtr Checked w)).
      * subst. 
        apply scope_weakening'; eauto.
      * econstructor; eauto.
        apply set_remove_all_intro; eauto.
        intro Contra; inv Contra. eauto.
    + econstructor.
      apply set_remove_all_intro; eauto.
      congruence.
  - eapply TyLitC; eauto.
    intros k Hk.
    destruct (H1 k Hk) as [N [T [HNth [HMap' [Hwt' IH]]]]].

    exists N; exists T; eauto.
    repeat (split; eauto).

    specialize (IH Hwt' HHwf m tm Hwt).
    apply scope_swap; auto.
Qed.


Lemma preservation_fieldaddr : forall (D : structdef) H n T (fs : fields),
  @well_typed_lit D H empty_scope n (TPtr Checked (TStruct T)) ->
  forall i fi ti,
  n <> 0 ->
  StructDef.MapsTo T fs D ->
  Fields.MapsTo fi ti fs ->
  nth_error (Fields.this fs) i = Some (fi, ti) ->
  heap_wf D H ->
  structdef_wf D ->
  fields_wf D fs ->
  word_type ti ->
  @well_typed_lit D H empty_scope (n + (Z.of_nat i)) (TPtr Checked ti).
Proof.
  intros D H n T fs HWT.
  inversion HWT;
  intros i fi ti Hn HS HF Hnth Hhwf HDwf Hfwf Hwt; eauto.
  - exfalso ; eauto.
  - destruct (H4  (Z.of_nat i)) as [N' [T' [HNth [HMap HWT']]]]; subst.
    + inv H1.
      simpl in H2.
      destruct (StructDef.find T D) eqn:Find; try congruence.
      inv H2.
      rewrite map_length.
      apply StructDef.find_2 in Find.
      assert (f = fs).
      { eapply StructDefFacts.MapsTo_fun; eauto. }
      subst.
      apply nth_length in Hnth.
      rewrite <- Fields.cardinal_1.
      eauto.
    + inv H1.
      simpl in *.
      destruct (@StructDef.find _ T D) eqn:Find; try congruence.
      inv H2.

      apply StructDef.find_2 in Find.
      assert (f = fs).
      { eapply StructDefFacts.MapsTo_fun; eauto. }
      subst.

      eapply map_nth_error with (f := snd) in Hnth.
      assert (Hyp: Fields.this fs = Fields.elements fs) by auto.
      rewrite Hyp in Hnth.

      (* I hate these types... *)
      assert (
          Hnth' : @eq (option type)
                      (@nth_error type
              (@map (prod Fields.key type) type (@snd Fields.key type)
                 (@Fields.elements type fs)) i)
           (@Some type (@snd nat type (@pair Fields.key type fi ti)))
        ) by auto.
      assert (Hi : (Z.to_nat (Z.of_nat i)) = i). {
        destruct i.
          +simpl. reflexivity.
          +simpl. zify. lia. }
      simpl in *.
      rewrite Z.sub_0_r in *. rewrite Hi in HNth.
      rewrite <- HNth in Hnth'.
      inv Hnth'.
      inv Hwt.
      * eapply TyLitC; simpl in *; eauto.
        intros k Hk; simpl in *.
        assert (k = 0) by lia; subst.
        exists N'. exists TNat.
        repeat (split; eauto).
        rewrite Z.add_0_r; eauto.
      * unfold fields_wf in Hfwf.
        apply Hfwf in HF. destruct HF. destruct H1.
        eapply TyLitC; simpl in *; eauto.
        intros k Hk; simpl in *.
        assert (k = 0) by lia; subst.
        exists N'. exists (TPtr m w).
        repeat (split; eauto).
        rewrite Z.add_0_r; eauto.

        assert (HEmpty : empty_scope = set_remove_all (n, TPtr Checked (TStruct T))
                                             ((n, TPtr Checked (TStruct T)) :: nil)).
        { unfold set_remove_all.
          destruct (eq_dec_nt (n, TPtr Checked (TStruct T)) (n, TPtr Checked (TStruct T))); auto.
          congruence.
        }

        eapply scope_strengthening in HWT'; eauto.
        rewrite <- HEmpty in HWT'.
        apply scope_weakening_cons.
        auto.

Qed.

(*

Def: H' |- H iff for all i
  H(i) = n^T such that . |- n^T : T under H implies
  H'(i) = n'^T such that . |- n'^T : T under H'.

Lemma PtrUpdA:
  Suppose H(i) = n^T and G |- n'^T' : T' under heap H.
  Then H' = H[i |--> k^T] implies that G,k^T |- n'^T' under heap H'
    when T = ptr^c W (i.e., it's a checked pointer type)
Proof
  Proof by induction on G |- n'^T' : T' under heap H.
  Case T-Int: Then T'=int and G,k^T |- n'^int under heap H' by T-Int
  Case T-VConst: Then G,k^T |- n'^T' under heap H' by T-VConst as well (since n'^T' \in G)
  Case T-PtrC: Three cases:
    n'^T' = k^T. Follows from T-VConst
    Otherwise
      T' = ptr^c W'
      types(D,W') = T0,...,T(j-1)
      G,n'^(ptr^c W') |-m H(n'+x) : Tx for 0 <= x < j under H
    We want to show
      G,n'^(ptr^c W'),k^T |-m H(n'+x) : Tx for 0 <= x < j under H'
    When n'+x != i then the result follows from T-Int, T-VConst, or T-PtrC and induction.
    When n'+x = i it follows by H-Visited, since H'(i) = k^T and k^T \in G,k^T
      (and H(i) = n^T --- that is the old and new value had the same annotation)
*)

Lemma PtrUpdA :
  forall D H s n' T',
    @well_typed_lit D H s n' T' ->
    forall i k m w,
      Heap.MapsTo i (m,TPtr Checked w) H ->
      @well_typed_lit D (Heap.add i (k,TPtr Checked w) H) (set_add eq_dec_nt (k,TPtr Checked w) s) n' T'.
Proof.
  intros D H s n' T' HWT'.
  remember HWT' as Backup; clear HeqBackup.
  induction HWT' using well_typed_lit_ind'; eauto;
    intros i k m T HMap.
  - econstructor.
    apply set_add_intro; eauto.
  - eapply TyLitC; eauto.
    intros x Hx.
    destruct (H1 x Hx) as [N' [T' [HNth [HMap' [HWT'' IH]]]]].
    destruct (Z.eq_dec (n + x) i).
    + subst.
      maps_to_fun.
      exists k; exists (TPtr Checked T); eauto.
      repeat (split; eauto).
      * apply Heap.add_1; eauto.
      * eapply TyLitRec; auto.
        apply set_add_intro1;
        apply set_add_intro2; auto. 
    + exists N'; exists T'; eauto.
      repeat (split; eauto).
      * apply Heap.add_2; auto.
      * eapply scope_replacement; eauto.
        eapply set_equal_add_add; eauto.
        eapply set_equal_refl.
Qed.
        (*
Lemma A: If G |- n^T : T where T = Ptr^c W such that W is an array
or word type, then G |- H(n) : T' where types(D,W) = T',...
Proof by induction on G |- n^T.
We have G,n^T |- H(n) : T' by inversion on H-PtrC. Consider the
derivation of this, and let k^T' = H(n).
  H-Int: Then G |- k^Int : Int as well
  H-Visited: There are two cases:
   k^T' \in G: In that case G |- k^T' : T' by H-Visited
   k^T' = n^T: In this case we can simply reuse the derivation we were
   given, i.e., G |- n^T : T.
 H-PtrC: Holds by induction.



Corollary PtrUpd:
  Suppose H(i) = n^T and G |- n'^T : T under heap H.
  Then H' = H[i |--> n'^T] implies that G |- n'^T under heap H'
Proof.
  If T is not a checked pointer it follows directly (same logic is PtrUpdA)
  Else by inversion we have
      T = ptr^c W 
      types(D,W) = T0,...,T(j-1)
      G,n'^(ptr^c W) |-m H(n'+k) : Tk for 0 <= k < j under H
    We want to prove
      G,n'^(ptr^c W) |-m H'(n'+k) : Tk for 0 <= k < j under H'
    Two cases
      n'+k == i. Then H'(i) = n'^T. The result follows from T-VConst.
      n'+k != i. Then H'(n'+k) = H(n'+k) = n''^Tk.
        By Lemma A we have G |-m H(n'+k) : Tk for 0 <= k < j under H
        By PtrUpdA we have G, n'^(ptr^c W) |-m H'(n'+k) : Tk for 0 <= k < j under H'

 *)




Lemma PtrUpd : forall i n T H D n',
    heap_wf D H ->
    simple_type T ->
    Heap.MapsTo i (n, T) H ->
    @well_typed_lit D H empty_scope n' T ->
    @well_typed_lit D (Heap.add i (n',T) H) empty_scope n' T.
Proof.
  intros i n T H D n' Hwf HSimple HMap HWT.
  remember HWT as Backup; clear HeqBackup.
  inv HWT; eauto.
  eapply TyLitC; eauto.
  intros x Hx.
  destruct (H1 x Hx) as [x' [Tx [HNth [HMap' HWt1]]]].

  destruct (Z.eq_dec (n'+x) i).
  - subst.
    maps_to_fun.
    exists n'. exists (TPtr Checked w).
    repeat (split; eauto).
    + solve_map.
    + eapply TyLitRec; eauto.
      apply set_add_intro2; auto. 
  - exists x'. exists Tx.
    repeat (split; eauto).
    + eapply Heap.add_2; eauto.
    + eapply PtrUpdA; eauto.

      assert (HEmpty : empty_scope = set_remove_all (n', TPtr Checked w)
                                                    ((n', TPtr Checked w) :: nil)).
      {
        unfold set_remove_all.
        destruct (eq_dec_nt (n', TPtr Checked w) (n', TPtr Checked w)); auto.
        congruence.
      } 

      rewrite HEmpty.
      eapply scope_strengthening; eauto.
Qed.

Lemma well_typed_heap_in : forall n D H w,
  heap_wf D H ->
  Heap.In n H ->
  word_type w ->
  @well_typed_lit D H empty_scope n (TPtr Checked w) ->
  exists x, Heap.MapsTo n (x, w) H.
Proof.
  intros n D H w Hwf HIn Hwt HWT.
  inv HWT.
  - destruct (Hwf 0) as [_ Contra].
    apply Contra in HIn.
    lia.
  - inv H3. 
  - inv Hwt; simpl in *; inv H1.
    + destruct (H4 0) as [n' [t' [HNth [HMap HWT]]]]; auto.
      *simpl. lia.
      *
      rewrite Z.add_0_r in HMap.
      inv HNth.
      exists n'; eauto.
    + destruct (H4 0) as [n' [t' [HNth [HMap HWT]]]]; auto.
      *simpl. lia.
      *rewrite Z.add_0_r in HMap.
       inv HNth.
       exists n'; eauto.
Qed.

Lemma well_typed_heap_in_array : forall n D H l h w,
  heap_wf D H ->
  Heap.In n H ->
  h > 0 ->
  l <= 0 ->
  @well_typed_lit D H empty_scope n (TPtr Checked (TArray (Num l) (Num h) w)) ->
  exists x, Heap.MapsTo n (x, w) H.
Proof.
  intros n D H l h w Hwf HIn Hl Hh HWT.
  inv HWT.
  - destruct (Hwf 0) as [_ Contra].
    apply Contra in HIn.
    lia.
  - inv H3.
  - inv H1.
    destruct l.
    + destruct (H4 0) as [n' [t' [HNth [HMap HWT]]]]; auto.
      * simpl. destruct h; inv Hl. simpl.
        assert (Hyp : exists s, Pos.to_nat(p) = S s).
        { apply pos_succ. }
        inv Hyp.
        rewrite replicate_length.
        simpl. lia.
      * rewrite Z.sub_0_r in *.
        inv HNth.
        exists n'; eauto.
        assert (H3 : t' = w). {
          destruct h; inv Hl. inv H1. 
          assert (HP: exists s, Pos.to_nat(p) = S s) by apply pos_succ.
          inv HP.
          rewrite H0 in H2. simpl in H2. inv H2. reflexivity.
        }
        rewrite <- H3. rewrite Z.add_0_r in *. assumption.
    + zify; lia.
    + assert (H1: (h - (Z.neg p)) > 0) by (zify; lia).
      assert (H2: exists n, (h - (Z.neg p)) = Z.pos n). {
        destruct (h - (Z.neg p)); inv H1. exists p0. reflexivity.
      }
      destruct H2 as [pos Hpos].
      assert (Hpos': exists n, Pos.to_nat pos = S n) by apply pos_succ.
      destruct Hpos' as [N HN].
      destruct (H4 0) as [n' [t' [HNth [HMap HWT]]]]; auto.
      rewrite Hpos. simpl. rewrite HN.
      rewrite replicate_length.
      simpl. split.
        * zify. lia.
        * rewrite Z.pos_sub_gt. 
          { zify. lia. }
          { zify. lia. }
        * rewrite Z.add_0_r in HMap.
          rewrite Hpos in HNth. simpl in HNth.
          rewrite HN in HNth. 
          assert (w = t').
              {
                eapply replicate_nth; eauto.
              }
              subst w.
          exists n'. assumption.
Qed.

Lemma add_one_not_change :
   forall x0 s,
      (forall x v t, Stack.MapsTo x (v,t) (add_nt_one s x0) -> simple_type t)
     -> (forall x v t, Stack.MapsTo x (v,t) s -> simple_type t).
Proof.
  intros.
  destruct (var_eq_dec x x0). subst.
  destruct t. apply SPTNat.
  destruct t. apply SPTPtr. apply SPTNat.
  apply (H x0 v (TPtr m (TPtr m0 t))).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v,TPtr m (TPtr m0 t)) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s). destruct p.
  inv eq1. assumption. inv eq1.
  apply SPTPtr. apply SPTStruct.
  apply (H x0 v (TPtr m (TArray b b0 t))).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v, TPtr m (TArray b b0 t)) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s). destruct p.
  inv eq1. assumption. inv eq1.
  destruct b0.
  assert (Stack.MapsTo x0
        (v, TPtr m (TNTArray b (Num (z + 1)) t))
        (add_nt_one s x0)).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v, TPtr m (TNTArray b (Num z) t)) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s).
  inv eq1.
  apply Stack.add_1. reflexivity. inv eq1.
  apply H in H1.
  inv H1. inv H3.
  apply SPTPtr. apply SPTNTArray. assumption.
  assert (Stack.MapsTo x0
        (v, TPtr m (TNTArray b (Var v0 (z + 1)) t))
        (add_nt_one s x0)).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v, TPtr m (TNTArray b (Var v0 z) t)) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s).
  inv eq1.
  apply Stack.add_1. reflexivity. inv eq1.
  apply H in H1.
  inv H1. inv H3.
  apply SPTStruct.
  apply (H x0 v (TArray b b0 t)).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v, TArray b b0 t) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s).
  inv eq1. assumption. inv eq1.
  apply (H x0 v (TNTArray b b0 t)).
  unfold add_nt_one.
  specialize (@Stack.find_1 (Z * type)s x0 (v, TNTArray b b0 t) H0) as eq1.
  destruct (Stack.find (elt:=Z * type) x0 s).
  inv eq1. assumption. inv eq1.
  apply (H x v t).
  unfold add_nt_one.
  destruct (Stack.find (elt:=Z * type) x0 s). destruct p.
  destruct t0.
  assumption.
  destruct t0. 1 - 4 : assumption.
  destruct b0.
  apply Stack.add_2. lia. assumption.
  apply Stack.add_2. lia. assumption.
  1 - 4 : assumption.
Qed.

(*
Lemma simple_type_step : forall D H s e s' H' r, (forall x v t, Stack.MapsTo x (v,t) s -> simple_type t)
                                    -> step D s H e s' H' r -> (forall x v t, Stack.MapsTo x (v,t) s' -> simple_type t).
Proof.
  intros. induction H1; eauto.
  destruct (var_eq_dec x x0).
  rewrite e0 in H2.
  apply Stack.mapsto_add1 in H2.
  injection H2. intros.
  subst.
  apply cast_means_simple_type in H1. assumption.
  apply Stack.add_3 in H2.
  apply (H0 x v). assumption. lia.
  specialize (add_one_not_change x0 s H0 x v t) as eq1.
  apply eq1. assumption.
Qed.
*)

Lemma well_bound_grow_env :
    forall env x v b, well_bound_in env b -> well_bound_in (Env.add x v env) b.
Proof.
   intros. induction b.
   apply well_bound_in_num.
   apply well_bound_in_var.
   inv H. inv H2.
   destruct (var_eq_dec x v0).
   unfold Env.In,Env.Raw.PX.In.
   exists v. apply Env.add_1. assumption.
   unfold Env.In,Env.Raw.PX.In.
   exists x0.
   apply Env.add_2. assumption. assumption.
Qed.

Lemma well_type_bound_grow_env :
    forall env x v t, well_type_bound_in env t -> well_type_bound_in (Env.add x v env) t.
Proof.
   intros. induction t.
   apply well_type_bound_in_nat.
   apply well_type_bound_in_ptr.
   apply IHt. inv H. assumption.
   apply well_type_bound_in_struct.
   apply well_type_bound_in_array.
   apply well_bound_grow_env. inv H. assumption.
   apply well_bound_grow_env. inv H. assumption.
   inv H. apply IHt. assumption.
   apply well_type_bound_in_ntarray.
   apply well_bound_grow_env. inv H. assumption.
   apply well_bound_grow_env. inv H. assumption.
   inv H. apply IHt. assumption.
Qed.

Lemma cast_bound_well_type : forall D F S H m env v t t', cast_type_bound S t t'
                 -> @well_typed D F S H env m (ELit v t) t -> @well_typed D F S H env m (ELit v t') t'.
Proof.
  intros. inv H1. apply TyLit.
  apply cast_means_simple_type in H0.
  apply (simple_type_well_bound env0) in H0.
  assumption. remember empty_scope as scope.
  eapply WTStack. apply (simple_type_means_cast_same).
  apply cast_means_simple_type in H0. assumption.
  inv H8.
  apply (cast_type_bound_same S t t' t'0) in H0.
  subst. apply cast_means_simple_type in H1.
  remember empty_scope as sc.
  induction H2 using well_typed_lit_ind'.
  apply TyLitInt.
  apply TyLitU.
  apply TyLitZero.
  subst. inv H0.
  eapply TyLitC;eauto.
    intros k Hk.
    destruct (H2 k Hk) as [N [T [HNth [HMap' [Hwt' IH]]]]].
    exists N. exists T.
    easy.
  assumption.
Qed.

   
Inductive env_consistent : env -> env -> Prop :=
  |Env_refl : forall e,
      env_consistent e e
  |Env_add : forall e x t,
      ~ Env.In x e ->
      env_consistent (Env.add x t e) e.

Definition ty_ssa_stack (S:stack) (e:expression) 
            := exists l, (forall x,  Stack.In x S -> In x l) /\ (exists l', ty_ssa l e l').

Definition stack_grow (D: structdef) (S S' : stack) :=
     (forall x v t, Stack.MapsTo x (v,t) S
              -> (exists t', (subtype D t' t) /\ Stack.MapsTo x (v,t') S')).


Lemma stack_grow_prop : forall D F S H S' H' e e', 
           ty_ssa_stack S e
          -> step D F S H e S' H' (RExpr e') -> stack_grow D S S'.
Proof.
 intros.
 specialize (ty_ssa_preserve' D S H S' H' e e' H0 H1) as eq1.
 remember (RExpr e') as e1.
 unfold stack_grow. intros.
 induction H1.
 exists t. split. constructor. easy.
 unfold change_strlen_stack in *.
 destruct ( n' - n <=? h) eqn:eq2.
 exists t. split. constructor. easy.
 assert (~ (n' - n <= h)).
 specialize (Z.leb_le (n' - n) h) as eq3.
 apply not_true_iff_false in eq2.
 intros R.
 apply eq3 in R. rewrite R in eq2. contradiction.
 assert (h < n' - n) by lia.
 destruct (Nat.eq_dec x x0).
 subst.
 apply Stack.find_1 in H2. rewrite H1 in H2. inv H2.
 exists (TPtr m (TNTArray l (Num (n' - v)) t0)).
 split. 
 apply SubTyNtSubsume.
 destruct l.
 constructor. lia. constructor. lia.
 constructor. lia.
 apply Stack.add_1. lia.
 exists t.
 split. constructor.
 apply Stack.add_2. lia. assumption.
 1 - 36 : exists t; split; try constructor; try easy.
 unfold ty_ssa_stack in H0.
 destruct H0. destruct H0.
 destruct H3.
 inv H3.
 destruct (Nat.eq_dec x x0).
 subst.
 assert (In x0 x1).
 apply H0.
 unfold Stack.In,Stack.Raw.PX.In.
 exists (v,t). assumption.
 contradiction.
 exists t. split. constructor.
 apply Stack.add_2. lia. assumption.
 1 - 5 : exists t; split; try constructor; try easy.
Qed.

Lemma stack_grow_cast_same : forall D S S' b b', stack_grow D S S' ->
              cast_bound S b = Some b' -> cast_bound S' b = Some b'.
Proof.
  intros. unfold cast_bound in *.
  destruct b. assumption.
  destruct (Stack.find (elt:=Z * type) v S) eqn:eq1. destruct p.
  unfold stack_grow in H.
  apply Stack.find_2 in eq1. apply H in eq1.
  destruct eq1. destruct H1.
  apply Stack.find_1 in H2.
  destruct (Stack.find (elt:=Z * type) v S') eqn:eq2. destruct p.
  inv H2. assumption. inv H2. inv H0.
Qed.

Lemma stack_grow_cast_type_same : forall D S S' t t', stack_grow D S S' ->
              cast_type_bound S t t' -> cast_type_bound S' t t'.
Proof.
  intros.
  induction H0. apply cast_type_bound_nat.
  apply cast_type_bound_ptr. apply IHcast_type_bound.
  apply cast_type_bound_array.
  apply (stack_grow_cast_same D S). assumption.
  assumption.
  apply (stack_grow_cast_same D S). assumption.
  assumption.
  assumption.
  apply cast_type_bound_ntarray.
  apply (stack_grow_cast_same D S). assumption.
  assumption.
  apply (stack_grow_cast_same D S). assumption.
  assumption.
  assumption.
  apply cast_type_bound_struct.
Qed.

Lemma cast_type_well_typed_lit :
    forall D s H v t t', cast_type_bound s t t' -> 
      well_type_lit_stack D s H empty_scope v t -> 
       well_type_lit_stack D s H empty_scope v t'.
Proof. 
 intros. 
 inv H1.
 apply (cast_type_bound_same s t t' t'0) in H0.
 subst. eapply WTStack. apply (simple_type_means_cast_same).
 apply (cast_means_simple_type) in H2. assumption.
 assumption. assumption.
Qed.

Lemma stack_grow_well_typed_lit :
    forall D s s' H v t,
     stack_grow D s s' -> 
      well_type_lit_stack D s H empty_scope v t -> 
       well_type_lit_stack D s' H empty_scope v t.
Proof. 
 intros D s s' H v t Hgrow HWT.
 inv HWT.
 eapply WTStack.
 apply (stack_grow_cast_type_same D s).
 assumption. apply H0.
 assumption.
Qed.

Lemma stack_grow_type_eq :
   forall D s s' t t', stack_grow D s s' -> 
         type_eq s t t' -> type_eq s' t t'.
Proof.
 intros.
 induction H0.
 constructor.
 apply type_eq_left. apply H0.
 apply (stack_grow_cast_type_same D s). assumption. assumption.
 apply type_eq_right. apply H0.
 apply (stack_grow_cast_type_same D s). assumption. assumption.
Qed.

Lemma stack_grow_meet_type :
  forall D s s' t t1 t2, stack_grow D s s' 
         -> meet_type D s t t1 t2 -> meet_type D s' t t1 t2.    
Proof.
  intros. 
  induction H0; eauto.
  apply meet_type_front_1. assumption.
  eapply meet_type_front_2.
  apply (stack_grow_cast_type_same D s s').
  assumption. apply H0.
  apply (stack_grow_cast_type_same D s s').
  assumption. apply H1.
  apply H2.
  apply meet_type_end_1. assumption.
  eapply meet_type_end_2.
  apply (stack_grow_cast_type_same D s s').
  assumption. apply H0.
  apply (stack_grow_cast_type_same D s s').
  assumption. apply H1.
  apply H2.
Qed.

Lemma stack_grow_well_typed :
    forall D F s s' H env m e t,
     stack_grow D s s' -> 
      @well_typed D F s H env m e t -> 
       @well_typed D F s' H env m e t.
Proof. 
 intros D F s s' H env m e t Hgrow Hwf.
 induction Hwf;eauto.
 constructor. assumption.
 apply (stack_grow_well_typed_lit D s s').
 assumption. assumption.
 eapply TyCall. apply H0.
 eapply TyCast2. 
 apply (stack_grow_type_eq D s s') in H0.
 apply H0. assumption.
 assumption.
 apply IHHwf.
 eapply TyCast3. 
 apply (stack_grow_type_eq D s s') in H0.
 apply H0. assumption.
 assumption.
 apply IHHwf.
 eapply TyCast4. 
 apply (stack_grow_type_eq D s s') in H0.
 apply H0. assumption.
 assumption.
 apply IHHwf.
 eapply TyAssign1.
 apply H0. assumption.
 apply (stack_grow_type_eq D s s'). assumption.
 assumption. apply IHHwf1.
 apply IHHwf2.
 assumption.
 eapply TyAssign2.
 apply H0. assumption. 
 apply (stack_grow_type_eq D s s'); assumption.
 apply IHHwf1.
 apply IHHwf2.
 assumption.
 eapply TyAssign3.
 apply H0. assumption. 
 apply (stack_grow_type_eq D s s'); assumption.
 apply IHHwf1.
 apply IHHwf2.
 assumption.
 eapply TyIndexAssign1. assumption. assumption.
 apply IHHwf1.
 apply (stack_grow_type_eq D s s'); assumption.
 apply IHHwf2. apply IHHwf3. assumption.
 eapply TyIndexAssign2. assumption. assumption.
 apply IHHwf1.
 apply (stack_grow_type_eq D s s'); assumption.
 apply IHHwf2. apply IHHwf3. assumption.
 eapply TyIf.
 apply H0. apply H1. easy.
 apply IHHwf1. apply IHHwf2.
 apply (stack_grow_meet_type D s s'); assumption.
 assumption.
Qed.

Lemma subtype_simple : forall D t t', subtype D t t'
                 -> simple_type t' -> simple_type t.
Proof.
  intros. 
  induction H. assumption.
  inv H0. inv H4.
  constructor. assumption.
  inv H1. inv H2. constructor. constructor. inv H0. assumption.
  inv H1. inv H2. constructor. constructor. inv H0. assumption.
  inv H0. inv H3. inv H. inv H1. constructor. apply SPTArray. assumption.
  inv H0. inv H3. inv H. inv H1. constructor. apply SPTNTArray. assumption.
  inv H0. inv H3. inv H. inv H1. constructor. apply SPTNTArray. assumption.
  constructor. constructor.
  constructor. constructor.
Qed.


Lemma env_sym : forall env env', @Env.Equal type env env' -> @Env.Equal type env' env.
Proof.
 intros. unfold Env.Equal in *.
 intros.  rewrite H. reflexivity.
Qed.

Lemma well_typed_grow : forall D F S H env m e t x t',
    ~ Env.In x env ->
    @well_typed D F S H env m e t ->
    @well_typed D F S H (Env.add x t' env) m e t.
Proof.
  intros.
  induction H1; eauto 20.
  apply weakening.
  eauto.
  apply TyVar. apply weakening_type_bound. assumption.
  destruct (Nat.eq_dec x0 x).
  subst.
  unfold Env.In,Env.Raw.PX.In in H0.
  destruct H0.
  exists t. assumption.
  apply Env.add_2. lia. assumption.
  eapply TyCall. apply H1.
  eapply TyStrlen.
  apply weakening_type_bound.
  apply H1.
  destruct (Nat.eq_dec x0 x).
  subst.
  unfold Env.In,Env.Raw.PX.In in H0.
  destruct H0.
  exists (TPtr m (TNTArray h l t)). assumption.
  apply Env.add_2. lia. assumption.
  eapply TyLet.
  apply IHwell_typed1. assumption.
  destruct (Nat.eq_dec x0 x).
  subst.
  eapply equiv_env_wt.
  assert (Env.Equal (Env.add x t1 (Env.add x t' env0)) (Env.add x t1 env0)).
  apply env_shadow. apply env_sym in H1. apply H1.
  assumption.
  eapply equiv_env_wt.
  assert (Env.Equal (Env.add x t' (Env.add x0 t1 env0)) (Env.add x0 t1 (Env.add x t' env0))).
  apply env_neq_commute.
  unfold Env.E.eq. lia. apply H1.
  apply IHwell_typed2.
  unfold Env.In,Env.Raw.PX.In in *.
  intros R. destruct R.
  apply Env.add_3 in H1.
  destruct H0.
  exists x1. assumption.
  lia.
  eapply TyMalloc.
  apply weakening_type_bound. assumption.
  eapply TyCast1; eauto.
  apply weakening_type_bound. assumption.
  eapply TyCast2; eauto.
  apply weakening_type_bound. assumption.
  eapply TyCast3; eauto.
  apply weakening_type_bound. assumption.
  eapply TyCast4; eauto.
  apply weakening_type_bound. assumption.
  eapply TyIf; eauto.
  destruct (Nat.eq_dec x x0).
  subst.
  unfold Env.In,Env.Raw.PX.In in *.
  destruct H0.
  exists t.
  assumption.
  apply Env.add_2.
  lia.
  assumption.
Qed.


Lemma well_bound_in_subst : forall env x t1 t2 b,
                          well_bound_in (Env.add x t1 env) b
                                -> well_bound_in (Env.add x t2 env) b.
Proof.
 intros. remember (Env.add x t1 env0) as env1.
 remember (Env.add x t2 env0) as env2.
 induction H;subst;eauto.
 apply well_bound_in_num.
 apply well_bound_in_var.
 unfold Env.In,Env.Raw.PX.In in *.
 destruct (Nat.eq_dec x x0).
 subst.
 exists t2.
 apply Env.add_1. reflexivity.
 destruct H.
 apply Env.add_3 in H.
 exists x1.
 apply Env.add_2. lia.
 assumption. lia.
Qed.

Definition ty_ssa_env (S:env) (e:expression) 
            := exists l, (forall x,  Env.In x S -> In x l) /\ (exists l', ty_ssa l e l').

Lemma well_type_bound_in_subst : forall env x t1 t2 t,
                          well_type_bound_in (Env.add x t1 env) t
                                -> well_type_bound_in (Env.add x t2 env) t.
Proof.
  intros. remember (Env.add x t1 env0) as env1.
  remember (Env.add x t2 env0) as env2.
  induction H;subst;eauto.
  apply well_type_bound_in_nat.
  apply well_type_bound_in_ptr.
  apply IHwell_type_bound_in. reflexivity.
  apply well_type_bound_in_struct.
  apply well_type_bound_in_array.
  eapply well_bound_in_subst. apply H.
  eapply well_bound_in_subst. apply H0.
  apply IHwell_type_bound_in. reflexivity.
  apply well_type_bound_in_ntarray.
  eapply well_bound_in_subst. apply H.
  eapply well_bound_in_subst. apply H0.
  apply IHwell_type_bound_in. reflexivity.
Qed.

Lemma ty_ssa_env_let_r : forall s x e e1 t,
         ty_ssa_env s (ELet x e e1) -> ty_ssa_env (Env.add x t s) e1.
Proof.
  intros. unfold ty_ssa_env in *.
  destruct H. destruct H.
  destruct H0.
  inv H0.
  exists S'.
  specialize (ty_ssa_grow (x::x0) e S' H7) as eq1.
  unfold list_subset in eq1.
  split. intros.
  destruct (Nat.eq_dec x2 x).
  subst.
  assert (In x (x::x0)) by apply in_eq.
  apply eq1 in H1. assumption.
  unfold Env.In,Env.Raw.PX.In in H0.
  destruct H0.
  apply Env.add_3 in H0.
  assert (Env.In x2 s).
  unfold Env.In,Env.Raw.PX.In. exists x3. assumption.
  apply H in H1.
  assert (In x2 (x::x0)). apply in_cons. assumption.
  apply eq1 in H2. assumption. lia.
  exists x1. assumption.
Qed.

Lemma ty_ssa_env_eq : forall s1 s2 e,
        Env.Equal s1 s2 -> ty_ssa_env s1 e -> ty_ssa_env s2 e.
Proof.
  intros. 
  unfold ty_ssa_env in *.
  destruct H0.
  unfold Env.Equal in H.
  exists x.
  split. intros.
  unfold Env.In,Env.Raw.PX.In in H1.
  destruct H1.
  apply Env.find_1 in H1.
  rewrite <- H in H1.
  apply Env.find_2 in H1.
  destruct H0. apply H0.
  unfold Env.In,Env.Raw.PX.In.
  exists x1. assumption.
  destruct H0.
  destruct H1.
  exists x0. assumption.
Qed.

Definition env_match D S (env env' : env) : Prop :=
   (forall x t, (Env.MapsTo x t env -> (Env.MapsTo x t env'
                   \/ (exists t' t'', cast_type_bound S t t' /\ subtype D t'' t' /\ Env.MapsTo x t'' env'))))
   /\ (forall x, Env.In x env' -> Env.In x env).

Lemma env_match_refl : forall D S env, env_match D S env env.
Proof.
  intros. unfold env_match.
  intros. split. intros. left. assumption.
  intros. assumption.
Qed.

Lemma env_match_ty_ssa : forall D S env1 env2 e,
        env_match D S env1 env2 -> ty_ssa_env env1 e -> ty_ssa_env env2 e.
Proof.
  intros. 
  unfold ty_ssa_env in *.
  unfold env_match in H.
  destruct H0. destruct H0.
  destruct H1.
  destruct H.
  assert (forall x0 : Env.key, Env.In (elt:=type) x0 env2 -> In x0 x).
  intros.
  apply H0.
  apply H2. assumption.
  exists x.
  split.
  easy.
  exists x0. assumption.
Qed.

Lemma env_match_grow : forall D S env env' x t, env_match D S env env' -> 
               env_match D S (Env.add x t env) (Env.add x t env').
Proof.
  unfold env_match in *.
  split. intros.
  destruct (Nat.eq_dec x0 x).
  subst.
  apply Env.mapsto_add1 in H0.
  subst.
  left. apply Env.add_1. reflexivity.
  apply Env.add_3 in H0.
  apply H in H0.
  destruct H0.
  left. apply Env.add_2.
  lia. assumption.
  destruct H0.
  destruct H0.
  right.
  exists x1. exists x2.
  split. destruct H0. eauto.
  split. destruct H0. destruct H1. assumption.
  apply Env.add_2. lia.
  destruct H0. destruct H1.
  assumption. lia.
  intros.
  destruct H.
  unfold Env.In,Env.Raw.PX.In in *.
  destruct (Nat.eq_dec x0 x).
  subst.
  exists t. apply Env.add_1. reflexivity.
  destruct H0.
  apply Env.add_3 in H0.
  specialize (H1 x0) as eq1.
  assert ((exists e : type, Env.Raw.PX.MapsTo x0 e (Env.this env'))).
  exists x1. assumption.
  apply eq1 in H2.
  destruct H2.
  exists x2.
  apply Env.add_2.
  lia. assumption. lia.
Qed.

Lemma env_match_grow_1 : forall D S env env' x t t' t'', env_match D S env env' -> 
              cast_type_bound S t t' -> subtype D t'' t' ->
               env_match D S (Env.add x t env) (Env.add x t'' env').
Proof.
  unfold env_match in *.
  split. intros.
  destruct (Nat.eq_dec x0 x).
  subst.
  apply Env.mapsto_add1 in H2.
  subst.
  right.
  exists t'. exists t''.
  split. assumption.
  split. assumption.
  apply Env.add_1. reflexivity.
  apply Env.add_3 in H2.
  destruct H.
  apply H in H2.
  destruct H2.
  left. apply Env.add_2. lia. assumption.
  destruct H2. destruct H2. destruct H2. destruct H4.
  right.
  exists x1. exists x2.
  split. assumption. split. assumption. 
  apply Env.add_2. lia. assumption. lia.
  intros.
  destruct H.
  unfold Env.In,Env.Raw.PX.In in *.
  destruct (Nat.eq_dec x0 x).
  subst.
  exists t. apply Env.add_1. reflexivity.
  destruct H2.
  apply Env.add_3 in H2.
  specialize (H3 x0) as eq1.
  assert ((exists e : type, Env.Raw.PX.MapsTo x0 e (Env.this env'))).
  exists x1. assumption.
  apply eq1 in H4.
  destruct H4.
  exists x2.
  apply Env.add_2.
  lia. assumption. lia.
Qed.

Lemma well_bound_match : forall D S env env' b, 
    env_match D S env env' ->
    well_bound_in env b -> well_bound_in env' b.
Proof.
  intros. induction H0.
  apply well_bound_in_num.
  apply well_bound_in_var.
  unfold env_match in *.
  destruct H.
  unfold Env.In,Env.Raw.PX.In in *.
  destruct H0.
  apply H in H0.
  destruct H0.
  exists x0. assumption.
  destruct H0. destruct H0.
  destruct H0. destruct H2.
  exists x2. assumption.
Qed.

Lemma well_type_bound_match : forall D S env env' t,
     env_match D S env env' ->
    well_type_bound_in env t -> well_type_bound_in env' t.
Proof.
 intros.
 induction H0;eauto.
 apply well_type_bound_in_nat.
 apply well_type_bound_in_ptr.
 apply IHwell_type_bound_in.
 assumption.
 apply well_type_bound_in_struct.
 apply well_type_bound_in_array.
 apply (well_bound_match D S env0). assumption.
 assumption.
 apply (well_bound_match D S env0). assumption.
 assumption.
 apply IHwell_type_bound_in. assumption.
 apply well_type_bound_in_ntarray.
 apply (well_bound_match D S env0). assumption.
 assumption.
 apply (well_bound_match D S env0). assumption.
 assumption.
 apply IHwell_type_bound_in. assumption.
Qed.

Lemma well_typed_match : forall D F S H env env' m e t,
    (env_match D S env env') -> 
     @well_typed D F S H env m e t ->
     ( @well_typed D F S H env' m e t \/ (exists t' t'' , cast_type_bound S t t'
          /\ subtype D t'' t' /\ @well_typed D F S H env' m e t'')).
Proof.
  intros.
  generalize dependent env'.
  induction H1;eauto.
  intros.
  - left. apply TyLit.
  apply (well_type_bound_match D S env0). assumption. assumption.
  assumption.
  - intros.
  unfold env_match in H2.
  destruct H2.
  apply H2 in H1.
  destruct H1.
  left. apply TyVar.
  apply (well_type_bound_match D S env0).
  unfold env_match. eauto.
  assumption.
  assumption.
  right.
  destruct H1. destruct H1.
  exists x0. exists x1.
  destruct H1. destruct H4.
  split. assumption. split. assumption.
  apply TyVar.
  apply cast_means_simple_type in H1.
  apply subtype_simple in H4.
  apply simple_type_well_bound. assumption.
  assumption. assumption.
  - auto.
  - intros. 
  assert (eq1 := H2).
  unfold env_match in H2.
  destruct H2.
  apply H2 in H1.
  destruct H1.
  left.
  eapply TyStrlen.
  apply (well_type_bound_match D S env0).
  assumption.
  apply H0.
  apply H1.
  destruct H1. destruct H1. destruct H1. destruct H4.
  left.
  specialize (cast_means_simple_type S (TPtr m (TNTArray h l t)) x0 H1) as eq2.
  inv H1. inv H9.
  specialize (subtype_ntarray D x1 m l' h' t'0 H4) as eq3.
  destruct eq3.  destruct H1. subst.
  apply subtype_simple_left in H4.
  eapply TyStrlen.
  apply (simple_type_well_bound env') in H4.
  apply H4.
  apply H5. assumption.
  - intros.
  assert (eq1 := H0).
  apply IHwell_typed1 in H0.
  destruct H0.
  assert (env_match D S (Env.add x t1 env0) (Env.add x t1 env')).
  apply env_match_grow. assumption.
  apply IHwell_typed2 in H1.
  destruct H1.
  left. eapply TyLet.
  apply H0. apply H1.
  destruct H1. destruct H1. destruct H1.
  destruct H2.
  right. 
  exists x0. exists x1.
  split. assumption. split. assumption.
  eapply TyLet.
  apply H0.
  apply H3.
  destruct H0. destruct H0. destruct H0.
  destruct H1.
  assert (env_match D S (Env.add x t1 env0) (Env.add x x1 env')).
  eapply env_match_grow_1. apply eq1.
  apply H0. apply H1.
  apply IHwell_typed2 in H3.
  destruct H3.
  left. eapply TyLet.
  apply H2.
  apply H3.
  destruct H3. destruct H3. destruct H3. destruct H4.
  right. exists x2. exists x3.
  split. assumption. split. assumption.
  eapply TyLet.
  apply H2.
  assumption.
  - intros.
  assert (eq1:= H0).
  apply IHwell_typed1 in H0.
  apply IHwell_typed2 in eq1.
  destruct H0.
  destruct eq1.
  left. apply TyPlus. assumption. assumption.
  destruct H1. destruct H1. destruct H1. destruct H2.
  inv H1. inv H2.
  left. apply TyPlus. assumption. assumption.
  destruct H0. destruct H0. destruct H0. destruct H1.
  destruct eq1. 
  inv H0. inv H1.
  left. apply TyPlus. assumption. assumption.
  destruct H3. destruct H3. destruct H3. destruct H4.
  inv H0. inv H1. inv H3. inv H4.
  left. apply TyPlus. assumption. assumption.
  - intros. 
  apply IHwell_typed in H4.
  destruct H4.
  left. eapply TyFieldAddr.
  apply H4. apply H0. apply H2.
  apply H3.
  destruct H4. destruct H4. destruct H4. destruct H5.
  inv H4. inv H10. inv H5.
  left. eapply TyFieldAddr.
  apply H6. apply H0. apply H2.
  apply H3.
  - intros.
  left.
  apply TyMalloc.
  eapply well_type_bound_match. apply H1.
  assumption.
  - intros. 
  apply IHwell_typed in H0.
  destruct H0.
  left. apply TyUnchecked.
  assumption.
  destruct H0. destruct H0. destruct H0.
  destruct H2.
  right.
  exists x. exists x0.
  split. assumption. split. assumption.
  apply TyUnchecked.
  assumption.
  - intros.
  assert (eq1 := H3).
  apply IHwell_typed in H3.
  destruct H3.
  left. eapply TyCast1.
  eapply well_type_bound_match. apply eq1.
  apply H0.
  assumption.
  apply H3.
  destruct H3. destruct H3. destruct H3.
  destruct H4.
  left.
  eapply TyCast1.
  eapply well_type_bound_match. apply eq1.
  assumption.
  assumption.
  apply H5.
  - intros.
  assert (eq1 := H3).
  apply IHwell_typed in H3.
  destruct H3.
  left.
  eapply TyCast2. apply H0.
  eapply well_type_bound_match. apply eq1.
  assumption.
  apply H3.
  destruct H3. destruct H3. destruct H3.
  destruct H4.
  specialize (cast_means_simple_type S (TPtr Checked (TArray u v t')) x0 H3) as eq2.
  inv H3.
  inv H9.
  specialize (subtype_array D x1 Checked l' h' t'1 H4) as eq3.
  destruct eq3. destruct H3. subst.
  apply subtype_simple_left in H4.
  left.
  eapply TyCast2.
  assert (type_eq S t t'1).
  inv H0.
  apply type_eq_right.
  apply (cast_means_simple_type S t'). assumption. assumption.
  apply (cast_type_bound_same S t' t t'1) in H12.
  subst. apply type_eq_refl. assumption.
  specialize (simple_type_means_cast_same S t' H3) as eq3.
  apply (cast_type_bound_same S t' t' t'1) in H12.
  subst.
  apply type_eq_right.
  assumption. assumption. assumption.
  apply H3.
  eapply well_type_bound_match.
  apply eq1. assumption. apply H5.
  assumption.
  - intros.
  assert (eq1 := H3).
  apply IHwell_typed in H3.
  destruct H3.
  left.
  eapply TyCast3. apply H0.
  eapply well_type_bound_match. apply eq1.
  assumption.
  apply H3.
  destruct H3. destruct H3. destruct H3.
  destruct H4.
  specialize (cast_means_simple_type S (TPtr Checked (TNTArray u v t')) x0 H3) as eq2.
  inv H3.
  inv H9.
  specialize (subtype_ntarray D x1 Checked l' h' t'1 H4) as eq3.
  destruct eq3. destruct H3. subst.
  apply subtype_simple_left in H4.
  left.
  eapply TyCast3.
  assert (type_eq S t t'1).
  inv H0.
  apply type_eq_right.
  apply (cast_means_simple_type S t'). assumption. assumption.
  apply (cast_type_bound_same S t' t t'1) in H12.
  subst. apply type_eq_refl. assumption.
  specialize (simple_type_means_cast_same S t' H3) as eq3.
  apply (cast_type_bound_same S t' t' t'1) in H12.
  subst.
  apply type_eq_right.
  assumption. assumption. assumption.
  apply H3.
  eapply well_type_bound_match.
  apply eq1. assumption. apply H5.
  assumption.
  - intros.
  assert (eq1 := H3).
  apply IHwell_typed in H3.
  destruct H3.
  left.
  eapply TyCast4. apply H0.
  eapply well_type_bound_match. apply eq1.
  assumption.
  apply H3.
  destruct H3. destruct H3. destruct H3.
  destruct H4.
  specialize (cast_means_simple_type S (TPtr Checked (TNTArray u v t')) x0 H3) as eq2.
  inv H3.
  inv H9.
  specialize (subtype_ntarray D x1 Checked l' h' t'1 H4) as eq3.
  destruct eq3. destruct H3. subst.
  apply subtype_simple_left in H4.
  left.
  eapply TyCast4.
  assert (type_eq S t t'1).
  inv H0.
  apply type_eq_right.
  apply (cast_means_simple_type S t'). assumption. assumption.
  apply (cast_type_bound_same S t' t t'1) in H12.
  subst. apply type_eq_refl. assumption.
  specialize (simple_type_means_cast_same S t' H3) as eq3.
  apply (cast_type_bound_same S t' t' t'1) in H12.
  subst.
  apply type_eq_right.
  assumption. assumption. assumption.
  apply H3.
  eapply well_type_bound_match.
  apply eq1. assumption. apply H5.
  assumption.
  - intros. 
  assert (eq1 := H4).
  apply IHwell_typed in H4.
  destruct H4.
  left. eapply TyDeref.
  apply H4.
  apply H0.
  eauto.
  apply H3.
  destruct H4. destruct H4. destruct H4.
  destruct H5.
  destruct H2. destruct H2.
  inv H0. inv H4. inv H5.
  right. exists t'0. exists t'0.
  split. assumption.
  split. constructor.
  eapply TyDeref.
  apply H6.
  apply SubTyRefl.
  left. split. eapply cast_word_type.
  apply H9. apply H2. reflexivity. assumption.
  inv H9. inv H2. inv H9. inv H2.
  inv H9.
  left. 
  eapply TyDeref.
  apply H6.
  eapply SubTyStructArrayField.
  apply H8. assumption.
  left. easy. assumption.
  inv H2. inv H2.
  inv H4. inv H9. inv H5.
  left. eapply TyDeref.
  apply H6.
  eapply SubTyStructArrayField.
  apply H11. assumption.
  left. easy. assumption.
  destruct H2. destruct H2. destruct H7.
  inv H0.
  inv H4. inv H10.
  inv H5.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. left.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H13. assumption.
  eapply cast_type_wf. apply H13. assumption.
  assumption.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. left.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H13. assumption.
  eapply cast_type_wf. apply H13. assumption.
  assumption.
  inv H4.
  inv H11. inv H5. inv H10.
  right. 
  exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. left.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H16. assumption.
  eapply cast_type_wf. apply H16. assumption.
  assumption.
  inv H10.
  right. 
  exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. left.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H16. assumption.
  eapply cast_type_wf. apply H16. assumption.
  assumption. inv H10. inv H10.
  destruct H2. destruct H7. subst.
  inv H0.
  inv H4. inv H10.
  inv H5.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. right.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H13. assumption.
  eapply cast_type_wf. apply H13. assumption.
  assumption.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. right.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H13. assumption.
  eapply cast_type_wf. apply H13. assumption.
  assumption.
  inv H4.
  inv H10. inv H5.
  right. 
  exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. right.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H15. assumption.
  eapply cast_type_wf. apply H15. assumption.
  assumption.
  right. 
  exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyDeref. apply H6.
  apply SubTyRefl.
  right. right.
  split. reflexivity.
  split. eapply cast_word_type.
  apply H15. assumption.
  eapply cast_type_wf. apply H15. assumption.
  assumption.
  - intros.
  assert (eq1 := H4).
  assert (eq2 := H4).
  apply IHwell_typed1 in H4.
  apply IHwell_typed2 in eq1.
  destruct H4.
  destruct eq1.
  left. eapply TyIndex1.
  assumption. assumption.
  apply H4. apply H2.
  apply H5. assumption.
  destruct H5. destruct H5.
  destruct H5. destruct H6.
  inv H5. inv H6.
  left. eapply TyIndex1.
  assumption. assumption.
  apply H4. reflexivity.
  assumption. assumption.
  destruct H4. destruct H4. destruct H4.
  destruct H5. subst.
  inv H4. inv H9.
  specialize (cast_means_simple_type S t' t'1 H12) as eqa.
  inv H5.
  destruct eq1.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex1.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H2. assumption.
  destruct H2. destruct H2. 
  destruct H2. destruct H4.
  inv H2. inv H4.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex1.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  destruct eq1.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex1.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H2. assumption.
  destruct H2. destruct H2. 
  destruct H2. destruct H4.
  inv H2. inv H4.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex1.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  - intros.
  assert (eq1 := H4).
  assert (eq2 := H4).
  apply IHwell_typed1 in H4.
  apply IHwell_typed2 in eq1.
  destruct H4.
  destruct eq1.
  left. eapply TyIndex2.
  assumption. assumption.
  apply H4. apply H2.
  apply H5. assumption.
  destruct H5. destruct H5.
  destruct H5. destruct H6.
  inv H5. inv H6.
  left. eapply TyIndex2.
  assumption. assumption.
  apply H4. reflexivity.
  assumption. assumption.
  destruct H4. destruct H4. destruct H4.
  destruct H5. subst.
  inv H4. inv H9.
  specialize (cast_means_simple_type S t' t'1 H12) as eqa.
  inv H5.
  destruct eq1.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H2. assumption.
  destruct H2. destruct H2. 
  destruct H2. destruct H4.
  inv H2. inv H4.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  destruct eq1.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H2. assumption.
  destruct H2. destruct H2. 
  destruct H2. destruct H4.
  inv H2. inv H4.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  - intros. 
  assert (eq1 := H4).
  assert (eq2 := H4).
  apply IHwell_typed1 in H4.
  apply IHwell_typed2 in eq1.
  destruct H4. destruct eq1.
  left. 
  eapply TyAssign1.
  apply H0.
  apply H1.
  apply H2.
  assumption. assumption. assumption.
  destruct H5. destruct H5.
  destruct H5. destruct H6.
  inv H1. apply type_eq_tnat in H2. subst.
  inv H5. inv H6.
  left. eapply TyAssign1.
  apply H0. constructor. constructor.
  assumption. assumption. assumption.
  assert (eq3 := H2).
  inv H2. inv H5.
  inv H6.
  inv H0.
  subst.
  right. 
  exists (TPtr m0 t').
  exists (TPtr m0 x).
  split. constructor. assumption.
  split. apply H6.
  inv H0.
  assert (
  eapply TyAssign1.
  apply H0. constructor.
  apply type_eq_right.
  constructor. apply (cast_means_simple_type S w).
  assumption. constructor.
  assumption.
  assumption.
  assumption.
  assumption.
  constructor.
  apply H3. apply H4.
  apply H0. apply H1.
  assumption.
  destruct H4. destruct H4.
  destruct H4. destruct H5.


  intros.
  assert (eq1 := H5).
  apply IHwell_typed1 in H5.
  apply IHwell_typed2 in eq1.
  destruct H5.
  destruct eq1.
  left. eapply TyIf.
  apply H1. eauto.
  apply H5. apply H6. apply H3.
  assumption.
  destruct H6. destruct H6. destruct H6.
  destruct H7.
Qed.


Lemma well_typed_subtype : forall D F S H env m e t x t1 t2 t3,
    @well_typed D F S H (Env.add x t1 env) m e t ->
     cast_type_bound S t1 t2 ->
     subtype D t3 t2 ->
    (exists env', env_match D S env env' /\
    (@well_typed D F S H (Env.add x t3 env') m e t \/ 
       (exists t' t'' , cast_type_bound S t t'
          /\ subtype D t'' t' /\ @well_typed D F S H (Env.add x t3 env') m e t''))).
Proof.
  intros.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  destruct eq1.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H2. assumption.
  destruct H2. destruct H2. 
  destruct H2. destruct H4.
  inv H2. inv H4.
  right. exists t'1. exists t'1.
  split. assumption. split. constructor.
  eapply TyIndex2.
  eapply cast_word_type. apply H12. assumption.
  eapply cast_type_wf. apply H12. assumption.
  apply H6. reflexivity. apply H5. assumption.
  - intros. 
  assert (eq1 := H4).
  assert (eq2 := H4).
  apply IHwell_typed1 in H4.
  apply IHwell_typed2 in eq1.
  destruct H4. destruct eq1.
  left. 
  eapply TyAssign1.
  apply H0.
  apply H1.
  apply H2.
  assumption. assumption. assumption.
  destruct H5. destruct H5.
  destruct H5. destruct H6.
  inv H1. apply type_eq_tnat in H2. subst.
  inv H5. inv H6.
  left. eapply TyAssign1.
  apply H0. constructor. constructor.
  assumption. assumption. assumption.
  assert (eq3 := H2).
  inv H2. inv H5.
  inv H6.
  inv H0.
  subst.
  right. 
  exists (TPtr m0 t').
  exists (TPtr m0 x).
  split. constructor. assumption.
  split. apply H6.
  inv H0.
  assert (
  eapply TyAssign1.
  apply H0. constructor.
  apply type_eq_right.
  constructor. apply (cast_means_simple_type S w).
  assumption. constructor.
  assumption.
  assumption.
  assumption.
  assumption.
  constructor.
  apply H3. apply H4.
  apply H0. apply H1.
  assumption.
  destruct H4. destruct H4.
  destruct H4. destruct H5.
  intros.
  assert (eq1 := H5).
  apply IHwell_typed1 in H5.
  apply IHwell_typed2 in eq1.
  destruct H5.
  destruct eq1.
  left. eapply TyIf.
  apply H1. eauto.
  apply H5. apply H6. apply H3.
  assumption.
  destruct H6. destruct H6. destruct H6.
  destruct H7.
Qed.

(* ty_ssa properties. *)
Lemma ty_ssa_stack_small_let : forall s e x e1,
         ty_ssa_stack s (ELet x e e1) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  inv H0.
  exists ((x :: x0)).
  split. intros.
  apply H in H0.
  apply in_cons. assumption.
  exists S'. assumption.
Qed.

Lemma ty_ssa_stack_small_plus_l : forall s e e1,
         ty_ssa_stack s (EPlus e e1) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  inv H0.
  exists x.
  split. intros.
  apply H in H0. assumption.
  exists S'. assumption.
Qed.

Lemma ty_ssa_stack_small_plus_r : forall s v t e,
         ty_ssa_stack s (EPlus (ELit v t) e) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  inv H0. inv H4.
  exists S'. eauto.
Qed.

Lemma ty_ssa_stack_small_efield : forall s e f,
         ty_ssa_stack s (EFieldAddr e f) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  exists x.
  split. intros.
  apply H in H1. assumption.
  exists x0. inv H0. assumption.
Qed.

Lemma ty_ssa_stack_small_cast : forall s t e,
         ty_ssa_stack s (ECast t e) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  exists x.
  split. intros.
  apply H in H1. assumption.
  exists x0. inv H0. assumption.
Qed.

Lemma ty_ssa_stack_small_deref : forall s e,
         ty_ssa_stack s (EDeref e) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  exists x.
  split. intros.
  apply H in H1. assumption.
  exists x0. inv H0. assumption.
Qed.

Lemma ty_ssa_stack_small_assign_l : forall s e e1,
         ty_ssa_stack s (EAssign e e1) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  exists x.
  split. intros.
  apply H in H1. assumption.
  inv H0.
  exists S'. assumption.
Qed.

Lemma ty_ssa_stack_small_assign_r : forall s v t e,
         ty_ssa_stack s (EAssign (ELit v t) e) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0. inv H0. inv H4.
  exists S'.
  split. intros. apply H.
  assumption.
  exists x0. assumption.
Qed.

Lemma ty_ssa_stack_small_unchecked : forall s e,
         ty_ssa_stack s (EUnchecked e) -> ty_ssa_stack s e.
Proof.
  intros. unfold ty_ssa_stack in *.
  destruct H. destruct H.
  destruct H0.
  exists x.
  split. intros.
  apply H in H1. assumption.
  exists x0. inv H0. assumption.
Qed.
*)


==> extended.tex <==
\newif\iftr\trtrue
\trtrue
\input{main}


==> figures/existingmem.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.75]
%\node[text width=3cm] at (1.5,-0.5) 
%    {some text spanning three};
%\draw[step=5cm,gray,very thin] (0,0) grid (5,5);
\fill[red!50!white] (2.5,2.5) rectangle (5,5);
\fill[red!20!white] (0,2.5) rectangle (2.5,5);
\fill[red!20!white] (2.5,0) rectangle (5,2.5);
\fill[green!40!white] (0,0) rectangle (2.5,2.5);

\Text[x=3.8cm,y=4.7cm,fontsize=\tiny]{Managed}
\Text[x=3.8cm,y=4.5cm,fontsize=\tiny]{Languages.}
\Text[x=3.8cm,y=4.3cm,fontsize=\tiny]{(Java, Python,}
\Text[x=3.8cm,y=4.1cm,fontsize=\tiny]{C\#, etc)}

\Text[x=1.2cm,y=4.7cm,fontsize=\tiny]{High Performant}
\Text[x=1.2cm,y=4.5cm,fontsize=\tiny]{Safe Languages.}
\Text[x=1.2cm,y=4.3cm,fontsize=\tiny]{(Rust, Go, etc)}

\Text[x=1.3cm,y=1.3cm,fontsize=\tiny]{\bf Checked C}


\Text[x=3.8cm,y=2.1cm,fontsize=\tiny]{Retrofitting}
\Text[x=3.8cm,y=1.8cm,fontsize=\tiny]{Techniques.}
\Text[x=3.8cm,y=1.5cm,fontsize=\tiny]{(ASAN, CCured,}
\Text[x=3.8cm,y=1.3cm,fontsize=\tiny]{etc)}

%\Text[x=0.9cm,y=0.6cm,fontsize=\tiny]{\bf \faFlagCheckered}

%\Text[x=2.0cm,y=1.4cm,fontsize=\tiny]{\bf \footnotesize iC3C}

%\draw [{Implies}-,double,line width=1pt] (1.0,0.8) -- (1.9,2.1);


\draw[-Stealth,thick] (0,0) -- (5.1,0) node[anchor=north west] {\bf \tiny high};
\Text[x=0cm,y=-0.2cm,fontsize=\tiny]{\bf least}
\Text[x=2.6cm,y=-0.2cm,fontsize=\footnotesize]{Performance Overhead}
\Text[x=-0.2,y=2.6,rotation=90,fontsize=\footnotesize]{Developer effort}
\draw[-Stealth,thick] (0,0) -- (0,5.1) node[anchor=south east] {\bf \tiny high};
\end{tikzpicture}
\caption{Existing approaches to handle memory corruptions vulnerabilities in C programs along with Checked C.}
\label{fig:memprotections}
\end{center}
\end{figure}

==> figures/memoryoverhead.tex <==
\begin{figure}
\pgfplotsset{every x tick label/.append style={font=\tiny, rotate=30}}
\pgfplotsset{every y tick label/.append style={font=\tiny}}
\begin{tikzpicture}  
  
\begin{axis}  
[  
    ybar,  
    ymin=-200, ymax=+200,
    enlargelimits=0.04,  
    ylabel={Memory Overhead (KiB)}, % the ylabel must precede a # symbol.  
    %xlabel={Programs},  
    symbolic x coords={ProFTPD, TinyBigNum, UFTPD, MicroHTTPD, png2pnm, pnm2png, Parsons}, % these are the specification of coordinates on the x-axis.  
    xtick=data,  
    bar width=10pt,
    width=7cm,
    x tick label/.append style={font=\tiny, rotate=30},
    y tick label/.append style={font=\tiny},
    axis background/.style={fill=gray!10},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north, font=\footnotesize},
    xlabel={Programs},
    ylabel style={font=\footnotesize},
     nodes near coords, % this command is used to mention the y-axis points on the top of the particular bar.  
    nodes near coords align={vertical},  
    ]  
\addplot coordinates {(ProFTPD,82.1) (TinyBigNum,81.1) (UFTPD, 86.3) (MicroHTTPD,82.3) (png2pnm, -102.5) (pnm2png, -51000) (Parsons, 9.8)};  
  
\end{axis}  
\end{tikzpicture} 
\caption{Memory Overhead of Partioned Programs.}
\label{fig:memoryoverhead}
\end{figure}


==> tables/conversioneffort.tex <==
{
\tiny
\begin{table}[]
\begin{tabular}{c|c|c|c|r|c}
\toprule
\textbf{Program} & \textbf{\begin{tabular}[c]{@{}c@{}}Partition\\ Methodology\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Pointers\\ Annotated\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Lines in\\ \ucregion \\ (Sandbox)\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Time\\ Taken\\ (hours)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}CVEs\\ Prevented\end{tabular}} \\ 
\midrule
\rowcolor{black!15} ProFTPD          &     $TP$                                                                     &       6                                                                &                                                                     N/A &                                                                                      1        & CVE-2010-4221 (\vulprevented{})                                                           \\ %\hline
png2pnm          & \multirow{2}{*}{$TP$}                                                        & \multirow{2}{*}{248}                                                     & \multirow{2}{*}{N/A}                                                    & \multirow{2}{*}{}                                                                            & \multirow{2}{*}{CVE-2018-144550 (\vulprevented{})}                                             \\ %\cline{1-1}
pnm2png          &                                                                          &                                                                       &                                                                      &                                                     8                                         &                                                                   \\ %\hline
\rowcolor{black!15} MicroHTTPD       &     $TP$                                                                     &          139                                                             &                                                                     450 &                                                                                       3       &                    N/A                                               \\ %\hline
UFTPD             &        $T_{Pr}$                                                                  &  146                                                                     &                                                                     90 &                                                           3                                   & \begin{tabular}[c]{@{}c@{}}CVE-2020-14149 (\vulprevented{}) \\ CVE-2020-5204 (\vulisolated{})\end{tabular}             \\ %\hline
\rowcolor{black!15} TinyBigNum       &      $CTP$                                                                    &   69                                                                    &                                                                     30 &                                                                                        2      &                             N/A                                      \\ %\hline
Parsons          &     $CTP$                                                                     &      364                                                                 &                                                                     800 &                                                      5                                        &                                                  N/A                 \\ 
\bottomrule
\end{tabular}
\caption{Summary of Conversion Efforts \& Security Impact.}
\label{table:conversioneffort}
\end{table}
}


==> typesystem.tex <==
\section{\systemname Type System and Formalism}
\label{sec:checkcboxtypesystem}
\subsection{Typing}
--EXPLAIN CHECKED C BOX TYPE SYSTEM
\subsection{Semantics}
BRIEF OVERVIEW of Semantics
